Modern Data Pricing Models: Taxonomy and Comprehensive Survey

Data play an increasingly important role in smart data analytics, which facilitate many data-driven applications. The goal of various data markets aims to alleviate the issue of isolated data islands, so as to benefit data circulation. The problem of data pricing is indispensable yet challenging in data trade. In this paper, we conduct a comprehensive survey on the modern data pricing solutions. We divide the data pricing solutions into three major strategies and thirteen models, including query pricing strategy, feature-based data pricing strategy, and pricing strategy in machine learning. It is so far the first attempt to classify so many existing data pricing models. Moreover, we not only elaborate the thirteen specific pricing models within each pricing strategy, but also make in-depth analyses among these models. We also conclude five research directions for the data pricing field, and put forward some novel and interesting data pricing topics. This paper aims at gaining better insights, and directing the future research towards practical and sophisticated pricing mechanisms for better data trade and share.

==> application.tex <==


\section{Applications}
 \label{sec:applicaiton}


 %\subsection{Related Fields}
 %\label{subsec:concpet}

\textcolor[rgb]{0.00,0.00,1.00}{In this section, we introduce two real-life application scenarios with data pricing issues, including pricing for mobile crowd sensing data markets and data trade with blockchain.}





\subsection{Pricing for Mobile Crowd Sensing Data Markets}


In recent years, electronic items like smartphones become more and more intelligent, which possess many kinds of sensors,  such as camera, compass, gyroscope, and global positioning system (GPS).
With a smartphone, individuals are capable of collecting all kinds of  data around them.  GPSs in mobile phones can be utilized to collect traffic information and help users estimate the travel time; phone sensors can help track the individual behaviors to evaluate the impact on the environment pollution; and phone-embedded microphones can help create noisy maps in different areas.
%
%


Using the crowd power to acquire large-scale sensing tasks is called \emph{mobile crowd sensing} (MCS).
The key to MCS is to use the embedded sensors in smartphones,
instead of the traditional paradigm relying on wireless sensor networks, like satellites, \textcolor[rgb]{0.00,0.00,1.00}{which significantly lowers the cost.
While the trading of structured and relational data have been studies, as we mentioned before, pricing mobile crowd-sensed data also attracts more attention due to the universality of data.
Recent studies \cite{zheng2017online,zheng2019arete} have made efforts in this field.}

\textcolor[rgb]{0.00,0.00,1.00}{Zheng et al.~\cite{zheng2017online} first identify the pricing problem in mobile crowd sensing data markets.
They introduce three challenges of this problem, including data uncertainty, economic-robustness (arbitrage-freeness in particular), revenue maximization.
For the first problem, they adopt a powerful regression technique \emph{Gaussian process}, which has been widely used as to model numerical sensing data, to model the data uncertainty.
Moreover, they provide three query types, i.e., single-data query, multi-data query, and range query, so that the data consumers can obtain required information.
Furthermore, they propose a pricing shceme \textsc{Arete}, which consists of two parts, namely, versioning mechanism and an online pricing mechanism.
They prove that \textsc{Arete} achieves both arbitrage-freeness and a
constant competitive ratio in terms of revenue maximization.}


\textcolor[rgb]{0.00,0.00,1.00}{Then Zheng et al.~\cite{zheng2019arete} further study the reward sharing in above data markets, and propose \textsc{Arete-sh} framework.
In particular, they model the problem as a coalitional game.
First of all, \textsc{Arete-sh} defined the qualified basic \emph{coalition} by using versioning algorithm, in order to reduce the number of coalitions.
Observing the basic \emph{coalition} is substitutable, they use a compact representation scheme, i.e., marginal contribution networks, to capture this feature.
Specifically, marginal contribution networks can represent coalitional game by a set of rules with specific forms.
After that, they employ Shapley value to fair share the reward in different coalitions.
The proposed \textsc{Arete-sh} can compute shapley value in polynomial time, achieving the four fairness axioms.}
%The MCS system consists of smartphone users to be data providers and platforms that require data.
%It can be viewed as an \emph{auction based process} where users bid tasks and the platform chooses the winner. While the difference is that, users in MCS systems need to \emph{lower} their bids to win the auction.
%
%The tasks (or saying the requesters publishing the tasks) act as the buyers of mobile resources, and the mobile devices owning the resources act as the sellers. The smartphone users may not be interested to share their sensors with the platform unless they receive satisfying rewards, which compensate their consumed resources, such as battery.
%A series of works attempt to solve the problem of setting the price in MCS. Table \ref{tab:MCS} overviews several algorithms on the objectives and pricing models.
%
%
%%Meanwhile, it has a critical payment to ensure the basic profit which will be defined later in the text.
%
%  %The above discussion can be stated: \\
%  %\emph{Payment Scheme Problem}: \emph{Payment Scheme Problem is to determine the least bids to win the auction and get maximum profits under the auction constraints.}\\
%  %\emph{Truthfulness}: \emph{The bid submitted by each mobile device should be truthful, i.e.} $b_h=c_h$
%
%  %Where $b_h$ and $c_h$ is the bid made by user $r_h$ and the true cost of taking the task the platform ask.\\
%  %\emph{Computational efficiency}: \emph{The algorithm should be solved in polynomial time, which is important to a practical system. }\\
%  %\emph{Individual rationality}: \emph{It means the utility of each mobile device should be nonnegative, i.e., $u_h\ge0$ for $\forall r_h$, which is a basic condition to stimulate the mobile devices participating in task execution.}
%
% %\cite{yang2012crowdsourcing} is a user-centric model even at the cost of sacrificing the platform utility. \cite{wen2014quality} concentrate on the reliability of data and the Wi-Fi fingerprint-based indoor localization realization.
%
%
%
%
%Specicially, ProMoT \cite{shah2015profit} provides incentives to the users to share the capabilities of their smartphones with the platform, and so that the platform's profit can be maximized.
%ProMot is composed of \emph{two} major components, denoted by the pair $(\mathcal{A},\mathcal{P})$, i.e., a \emph{winner determination algorithm} $\mathcal{A}$ and a \emph{payment scheme} $\mathcal{P}$, which calculates the payment.
%The winner determination algorithm  $\mathcal{A}$ converts the problem into a linear programming (LP) problem.
%A novel greedy mechanism is proposed, which selects those users who are most likely to increase the profit of the platform by using the solution of LP problem.
%The component of payment scheme  $\mathcal{P}$ is based on auction theory, and  aims to ensure truthful bidding of smartphone users. %The critical payments motivate the bidders to reveal their bid truthfully. The concept of critical payments is introduced to propose the payment scheme.
%Each bidder is paid an amount of rewards, which is the highest bid that the bidder can submit to win the auction. %Let $\mathcal{M}_{-j}$ denote the set of smartphone users excluding user $j$. %We execute the winner determination algorithm $\mathcal{A}$ with $\mathcal{M}_{-j}$ as input to find the winner set $\mathcal{W}_{-j}$.
%The critical value of bidder $j$ is the highest value of $b_j$, such that it can still win the auction and contribute to the profit of the platform,  which motivate the bidders to reveal their bid truthfully. The truthful auction mechanism ProMot considerably increases the profit of the platform in comparison with other mechanisms and is able to motive users to bid.

%\begin{table*}[t]\footnotesize
%  	\centering	
%  \setlength{\tabcolsep}{2pt}
%  	\caption{Overview of Mobile Crowd Sensing Mechanisms}
%  	\begin{tabular}
%     	{lll}
%  		\toprule[0.7pt]
%  		\textbf{Algorithm}&\textbf{Pricing Model}&\textbf{Objective} \\
%  		\midrule[0.5pt]
%  		ProMoT \cite{shah2015profit}&auction based model & maximizing the platform's profit \\
%  		HTM \cite{wang2017towards}&auction based model & maximizing each user's utility \\
%  		MS \cite{yang2012crowdsourcing}&game theory \& auction based  model & considering both platform
%and user centric situations  \\
%  		\bottomrule[0.7pt]
%  	\end{tabular}
%  	\label{tab:MCS}
%  \end{table*}


%In contrast, an auction based mechanism, i.e., heterogeneous task model (HTM) \cite{wang2017towards}, is proposed to allocate tasks in MCS and to determine the rewards given to users. HTM aims to maximize the utility for every single user.
%The main idea is to convert the winning bid determination problem into finding a minimum weight bipartite matching, based on which, a VCG-based auction mechanism is designed to decide the payments of the winning bids. Results show that, HTM achieves computational efficiency and maximizes the user utility.





%Therefore, the critical payment $p_j$ is the maximum value of $b_j$ such that the following inequality holds
  %\begin{equation}
  %v(\mathcal{W})-\sum_{i\in{\mathcal{W}}/j}b_i-b_j \ge %v(\mathcal{W}_{-j})-\sum_{i\in \mathcal{W}_{-j}}b_i
  %\end{equation}

  %It can be proved that the algorithm fits all the constraints well.\\



  %Similar to the previous model, the first part of Heterogeneous Task Model\cite{wang2017towards} is called \emph{\textbf{ Greedy Winning Bids Determination Scheme}}.

  %For each bid submitted by the mobile devices, e.g. $b_i$, we first define a parameter $\beta_{i}$ , named cost per unit resource, as follows:
 % \begin{equation}
  %\beta_{i}=\frac{b_i}{res_i}
  %\end{equation}

  %Where $b_i$ and $res_i$ represents the bid of user $P_i$ and the resource it take for $P_i$ to finish the task.



  %It can be proved that the algorithm fits all the constraints well.\\
  %\noindent \textbf{(3) Mobile Sensing Pricing}

%The ultimate goal in mobile sensing pricing is to design an incentive mechanism that motivates smartphone users to participate in mobile phone sensing while preventing any user from rigging its bid to manipulate the market.
%It needs to settle for a tradeoff between utility maximization and truthfulness. %Our highest priority is to design an incentive mechanism that satisfies all of the four desirable properties, even at the cost of sacrificing the platform utility.
%The MS model \cite{yang2012crowdsourcing} considers both platform-centric and user-centric situations.
%The first one uses a game to reach \emph{equilibrium} between users and platform, where the platform is the leader while the users are the followers.
%For the user-centric situation, an auction-based incentive mechanism is designed, which essentially sorts the users according to the difference of their marginal values, and bids by following a greedy approach.
%The results show that, the platform-centric model enables the platform to maximize its utility, while no user can improve its utility by deviating from the current strategy unilaterally.
%The user-centric model reaches linear computational complexity and maximized user profit.
%Then in the sorting, one computes the maximum price that user $i$ can bid such that $i$ can be selected instead of user at $j$-th place. It repeats this until the position of the first loser and we compute the payment $p_i$ for each winner $i$.
  %MSensing auction mechanism consists of two phases: the winner selection phase and the payment determination phase.

  %\emph{The winner selection phase} follows a greedy approach: Users are essentially sorted according to the difference of their marginal values and bids. Given the selected users $\mathcal{S}$, the marginal value of user $i$ is $v_i(\mathcal{S})$ = $v(\mathcal{S} \cup {i}) -$ $v(\mathcal{S})$.
  %In this sorting the $(i + 1)$-th user is the user $j$ such that $v_j(\mathcal{S}_i) - bj$ is maximized over $\mathcal{U} \setminus \mathcal{S}_i$, where $\mathcal{S}_i = {1, 2, \cdots, i}$ and $S_0 = \varnothing$.
  %We use $v_i$ instead of $v_i(\mathcal{S}_{i-1})$ to simplify the notation. Considering the submodularity of $v$, this sorting implies that
  %\begin{equation}
  %v_1-b_1 \ge v_2-b_2\ge...\ge v_n-b_n
  %\end{equation}


  %The set of winners are $\mathcal{S}_L = {1, 2, ... , L}$, where $L \leq n$ is the largest index such that $v_L - b_L > 0$.

  %In the payment determination phase, we compute the payment $p_i$ for each winner $i \in \mathcal{S}$. To compute the payment for user $i$, we sort the users in $\mathcal{U} \setminus {i}$ similarly,
  %\begin{equation}
 % v_{i_1}'-b_{i_1}' \ge v_{i_2}'-b_{i_2}'\ge...\ge v_{i_{n-1}}-b_{i_{n-1}}
 % \end{equation}\\
  %where $v_{i_j}' = v(\mathcal{T}_{j-1} \cup {i_j}) - v(\mathcal{T}_{j-1}) $denotes the marginal value of the $j$ th user and $\mathcal{T}_j$ denotes the first $j$ users according to this sorting over $\mathcal{U} \setminus {i}$ and $\mathcal{T}_0 = \varnothing $. The marginal value of user $i$ at position $j$ is $v_{i(j)} = v(\mathcal{T}_{j-1} \cup {i}) - v(\mathcal{T}_{j-1})$. Let $K$ denote the position of the last user $i_j \in \mathcal{U} \setminus {i}$, such that $b_{i_j} < v_{i_j}$. For each position $j$ in the sorting, we compute the maximum price that user $i$ can bid such that $i$ can
  %be selected instead of user at $j$ th place. We repeat this until the position of the first loser. In the end we set the value of $p_i$ to the maximum of these $K + 1$ prices.\\
  %\noindent \textbf{(4) Quality-Driven Auction}

  %\cite{wen2014quality} presents the algorithm of determining the winner data set for a specific type of task for the convenience of presentation. %The process of determining the entire submitted data set is similar and thus omitted here.

 %The algorithm first randomly chooses a value $G$, which separates all line segments into three classes. And then narrow down the narrow down the possible range of $G$ corresponding to the winner data set on the data quality axis by the third item of previous theorem. The QDA reachs the maximization the system's social welfare.


  %It is straightforward that the three classes are in fact representing the three subcontract sets $Q_1$, $Q_2$, and $Q_3$ mentioned previously in the article. If we know
  %the exact sum of the quality of the elements in the winner data set, it is safe to say that all the elements in $Q_3$ are in the winner set, whereas the ones in $Q_1$ are definitely not.

  %We first randomly choose a value $G$, which separates all line segments into three classes. If the sum of the length of the line segments in $Q_2$ and $Q_3$ is less than $G$, the sum of length of the line segments in the winner data set will be on the left side of $G$ by the first item of previous theorem. We will try to move $G$ to the left in this case. If the sum of the length of the line
  %segments only in $Q_3$ is already greater than $G$, the sum of length of the line segments in the winner data set will be on the right side of $G$ by the second item of previous theorem. We will try to move $G$ to the right in this case. In this way, we are able to narrow down the possible range of $G$ corresponding to the winner data set on the data quality axis by the third item of previous theorem. All subcontracts completely on the right side of the
  %range must be in the winner data set, and all those completely on the left side of the range must not. We now only need to search those subcontracts in $Q_2$, which can maximize the system's social welfare. Those subcontracts are denoted to be in the set $V$ in previous algorithm. Finally, the winner data set should be $\mathcal{W}_j \cup \mathcal{V} $.


%In addition, in dynamic data marketplaces, the incoming buyers and data streams on the market need to be matched in real-time.  A matching-based approach dynamic pricing problem is discussed in \cite{tong2018dynamic} for spatial crowdsourcing.
%Several auction mechanisms {\color{blue}\cite{heckman2015pricing,sun2014behavior,zhao2014crowdsource}} are designed for mobile crowdsourcing, when a limited budget is assigned for sensing tasks and the platform performs a subset of tasks according to its budget constraint. Besides, a pricing model for interference and power management in 5G is explored \cite{luong2018applications}.







%Future work could concentrate on the following perspectives: In the ProMot algorithm, we only consider the situation that one platform offers the job to workers. However, in real life there are many platforms and workers can choose to take the job.  The case of multiple crowdsourcing systems with multiple platforms and propose a double auction mechanism can be considered. %The HTM method is static and fragile. It is worth working on when the information of the workers and jobs is changing.
%Besides, how to combine the user-centric model MS  and platform-centric model together and under this circumstance the overall social welfare is maximized is still a problem.
%The QDA method deployed the indoor localization system to evaluate the proposed incentive mechanism. Improvement can be made to adapt to the large-scale scenario.


\begin{comment}


 \subsection{Pricing in Real-Time Ridesharing}


%With the widespread use of smartphones and the progress of GPSs,
According to \emph{Didi Chuxing}, the biggest ridesharing platform in China, there are more than 2.4 million orders per day.
Uber has employed dynamic pricing in its system \cite{uber}.
The task price is set by considering the total number of drivers and requesters in a region during a time period.
As a consequence, the ridesharing is becoming popular due to its efficiency and monetary saving.


The shortage of vehicles becomes the major problem in peak times for ridesharing.
When it occurs, customers can offer a bonus to the platform, so they can get priorities in the dispatch procedure.
It can be viewed as an auction process, where customers act as buyers. They bid the money they would like to pay to get the service. The platform acts as an auctioneer and decides the dispatch plan.
Thus, the problem of ridesharing pricing has been extensively explored in academia, such as two-sided market pricing \cite{bimpikis2019spatial,ma2018spatio}, the equilibria among owners and renters \cite{fang2017prices} given a fixed market price, the sophisticated model \cite{banerjee2016dynamic}, and so forth.






 %The following example will show how to set the price in real-time sharing.

 %Example 1. Ride-sharing problem\cite{zheng2018order}. In typical ridesharing platforms (Uber and Didi Chuxing), the price of a ridesharing order is decided after user's input of destination and before his/her drop of an order. Therefore, the prices of the ridesharing orders are fixed regardless of the dispatch and routing results. This is quite different from non-ridesharing orders whose price may depend on the actual travel length, location of the customer, time and so on.
 %\begin{figure}[h]
 %	\centering
 %	\label{fig:ridesharing}
 %	\includegraphics[width=0.5\textwidth]{sharing.eps}
 %	\caption{Example 1.}
 %\end{figure}

 %In Figure 4, there are three orders $o_1$, $o_2$, $o_3$ and only one vehicle $v_1$. $o_1^s$, $o_2^s$, $o_3^s$ and $o_1^e$, $o_2^e$, $o_3^e$ represent the origins and destinations respectively. Circles and edges represent the nodes and paths respectively in the road network. In this example, all edges are of equal travel distance. This example corresponds to peak ordering periods where vehicles are in shortage. There are two possible travel plans for $v_1$: (i) $v_1 o_1^s o_2^s o_1^e o_2^e$; (ii) $v_1 o_1^s o_2^s o_1^e o_2^e$. Without considering the order prices, the above two plans show no difference because they own the same amount of travel distance and the same number of served orders. Let us consider the order prices and assume price($o_2$) > price($o_3$). This is reasonable
 % as $d(o_2^s,o_2^e)$ > $d(o_3^s,o_3^e)$. {\color{blue} Note that $d(\;,\;)$ represents }the shortest path distance, and has a strong impact on orders? price in practice. Then, the price-aware solution would be dispatching $o_1$ and $o_2$ to
 %$v_1$.

 %And then we can set a price for this trip according to the above price-aware solution.

%Many models are formed to solve the pricing problem in .
%An \textbf{order pricing for Greedy dispatch} is developed for ridesharing platform to dispatch customers to vehicles to reach overall utility maximization \cite{zheng2019auction}. The overall utility means the total utility or profits platform, drivers and customers can get. The idea of this approach is to compare a customer $P_h$ to other dispatched customers using the Greedy-based order dispatch. Then it finds the minimum bid for $P_h$ to replace one of them. If the inequality
%\begin{equation}
%bid_h \ge uti_i + cost_h
%\end{equation}
%holds, then one can replace $P_i$ with $P_h$. In particular, $uti_i$ and $cost_h$ represent the utility of $P_i$ and the cost of inserting $P_h$ in to the dispatch plan (i.e., the cost of detour distance).  Then one compares $P_h$ with all the other customers to get the minimum bid.

%When vehicles are in shortage, requesters are allowed to offer bonus so that their orders can get prioritized in the dispatch process.


In order to enable self-motivated bonus bidding of requesters,
an auction mechanism \cite{zheng2019auction} is devised, where requesters are supposed to submit their bids truthfully and the platform conducts order dispatch and pricing.
The goal is to maximize the overall utility of the auction.
Instead of considering each order as a single unit to be dispatched, in the proposed \textit{divide-and-walk} (DnW) mechanism, the dispatch unit is a pack.
After assigning the pack, the mechanism computes the rank of each pack and then assigns the customers to drivers according to the pack.
Results show that the mechanism enables self-motivated bonus offering of requesters and reaches maximized overall utility, which is the utility of all drivers, customers and platform.


%is developed for ridesharing platform to dispatch customersThere is another model based on Greedy method, namely \emph{ranking-based order dispatch} \cite{zheng2019auction}. First, this approach finds the optimal pack which contains $P_j$ and has at most $\bar{c}$ requesters, where $\bar{c}$ represents the capacity of each vehicle, such that dispatching this pack to one of their nearest vehicles yields the maximum utility. Then by ranking all the packs in descending orders we can assign the pack to its vehicle and therefore we get the dispatch plan.




 %Under this circumstance, an individual need to decide the best strategy to get the service with the least amount of money, which can be conclude as the following problem.\\
 %\textbf{Order Pricing Problem}: \emph{The order pricing problem is to determine the least amount of money a requester have to pay with the following constraint.}\\
 %\emph{Individual rationality}: \emph{It refers to the situation that the utility of any customer $u_j$is non-negaive, i.e.}
 %\begin{equation}
 %\forall P_i,u_j=(val_j-pal_j)x_j\ge0
 %\end{equation}

 %Where $P_i , val_j , pal_j$ refers to the customer, the valuation of $P_i$ and the payment of $P_i$. $x_j=1$ if $P_j$ is dispatched to a vehicle. $x_j=0$ for other situations.\\
 %\emph{Profitability}: \emph{An auction is profitable if the utility of the platform is non-negative,   i.e.}       $U_{plf}\ge0$.\\
%\noindent \textbf{(1) Greedy-based Order Dispatch}

%\\
 %Finally, it can be showed that the algorithm fits the constraints. Besides, the complexities of the
 %order dispatch and pricing algorithms are polynomial w.r.t. the
 %input size.\\
 %\textbf{(2) The Ranking Approach (Divide-and-Walk)}

%Instead of considering each order as a single unit to be dispatched, in \textbf{Divide-and-Walk} (DnW), the dispatch unit is a pack.  Then, it searches intervals. For each of them, we find smallest bid of $h$ for it to be successfully dispatched using Ranking-based order dispatch.







There also exist other problems in real-time ridesharing.
A particular concern is that trips may be mis-priced relative to each other, incentivizing drivers to strategize  \cite{bimpikis2019spatial,ma2018spatio}.
For example, many platforms hide trip destinations from drivers before the pick-up. However, experienced drivers will call riders to ask about trip details, and cancel those that are not worthwhile in situations like rush hour and occasionally price fluctuate.
The \textit{spatio-temporal pricing (STP)} mechanism \cite{ma2018spatio} addresses the problem of incentive alignment for drivers in the presence of spatial imbalance and temporal variation of rider trip flows, for dispatching and pricing in the context of a ridesharing platform.
The mechanism induces an extensive-form game among the drivers, where the total payoff to each driver is determined by the mechanism's dispatch and payment rules.
A rider's value is modeled as his or her willingness-to-pay, over and above a base payment that covers a driver's extra costs for picking up a rider (extra wear and tear, inconvenience, etc.), in comparison
to the cost of driving the same trip as relocation without a rider (fuel, time, and so forth).
This base payment is transferred directly to the driver, so that all drivers completing the same trip with or without a rider incur the same trip cost.
The prices determined by the STP mechanism are the
payments collected on top of the base payments.
The results show that, STP achieves substantially higher social welfare and drivers' time efficiency, in comparison to other pricing mechanism, where prices are highly unstable and drivers incur a large regret.

%\cite{ma2018spatio} formally defines a dynamic \textbf{spatio-temporal pricing} (STP) mechanism, which uses the history of actions to update the plan forward from the current state.Besides, it always dispatches all available drivers. Given economy $E^{(0)}$ at the beginning of the planning horizon, or economy $E^{(t)}(s_t)$ immediately after a deviation by one or more drivers. The main result of the work is that, the model is temporally consistent and subgame-perfect incentive compatible. It is also individually rational for riders and strictly budget balanced for any action profile taken by the drivers, and is welfare optimal, core-selecting, individually rational for drivers and envy-free in subgame-perfect equilibrium from any history onward.





%This paper conceptualizes many of the problems with current platforms as arising from prices failing to be appropriately 'smooth' in space and time if prices for trips are higher in one location then they should be appropriately higher in adjacent locations; If demand would soon increase in a location then the current prices should already be appropriately higher; and if destinations differ in continuation payoffs then trip prices to these destinations need to reflect this. With appropriately smooth prices, drivers who retain the flexibility to choose when to work will choose to accept any trip to which they are dispatched.


 %Then we define the STP mechanism by providing a method to plan or re-plan, this implicitly defining the dispatch and payment rules. For each $a\in L$ and $t\in T $, denote the welfare gain from an additional driver at $(a,t)$ that is already in the platform as:
 %\begin{equation}
 %\Phi_{a,t}=W(\mathcal{D}\cup{(1,a,t,T)})-W(\mathcal{D})
 %\end{equation}

 %where $(1,a,t,T)$ represents the type of this driver that stays until the end of the planning horizon.

 %\noindent \textbf{Definition 1}: (Spatio-Temporal pricing mechanism) The \emph{spatio-temporal pricing (STP)} is a dynamic ridesharing mechanism that
%the mechanism completes the following planning step:\\
 %\emph{Dispatch rule}: To determine the dispatches ($\alpha^{*}$), compute an optimal solution $(x, y)$ to the CE mechanism we mentioned above, and dispatch each driver $i\in \mathcal{D}$ to take the path $Z_{i,k}$ for $k$ s.t. $y_{i,k}= 1$, and pick up riders $j\in \mathcal{R} $ s.t. $x_j = 1$.\\
 %\emph{Payment rules}: To determine driver and rider payments $r^*$ and $q^*$, for each $(a,b,t)\in\mathcal{T} $, set anonymous trip prices to be $p_{a,b,t} = \Phi_{a,t}-\Phi_{b,t+\delta(a,b)}+c_{a,b,t}$

 %where $c_{a,b,t}$ and $\delta(a,b)$ denote the cost of whole trip and the time to travel time between locations.



 \begin{table*}[tb]\footnotesize
 \centering
 \setlength{\tabcolsep}{2pt}
 \caption{Overview of Ridesharing Pricing Mechanisms}
 	\begin{tabular}
 		{lllp{5.0cm}}
 		\toprule[0.7pt]
 		\textbf{Algorithm}&\textbf{Pricing model}&\textbf{Objective}&\textbf{Motivation} \\
 	    \midrule[0.5pt]
 		DnW \cite{zheng2019auction}&auction based model&maximizing overall utility &  self-motivated bonus offering  \\	
 		STP \cite{ma2018spatio} &game theory based model &maximizing overall utility &incentive alignment for drivers \\
 		%CE\cite{ma2018spatio}&Competitive equilibrium theory based&{\color{blue}Maximization of overall utility}&Computational efficient&Fragile\\
 		%PPS\cite{fang2017prices}&Equilibria based&{\color{blue}Maximization of platform revenue}&Low complexity and wide use.&Static and fragile\\
 	    QTE \cite{banerjee2016dynamic} &game theory based model &maximizing overall utility & intrinsic timescale separation in
 strategic interaction of drivers and users \\
 		\bottomrule[0.7pt]
 	\end{tabular}
 	\label{tab:ridesharingpricing}	
 \end{table*}

To captures the three features of ridesharing platforms: the  two-sided nature, the strategic reaction of market participants to marketplace policies, and the ability of the platform to price based on real-time state, a \textit{queueing-theoretic economic} (QTE) model \cite{banerjee2016dynamic} is proposed.
This mechanism is based on queueing theory and aims to reach maximized overall utility.
In particular, it considers a geographic area divided into regions, and tracks a Markov chain that tracks the number of available and busy drivers in each region.
Each ride involves a driver picking up a passenger in one region, and dropping her off in another.
Key to the QTE model is the assumption that there is an \emph{intrinsic timescale separation} in the strategic interaction of drivers and passengers.
This is based on the observation that, passengers are typically sensitive to the immediate availability and price at the moment when they need a ride, while drivers are typically sensitive to the average wages earned over a longer period of time (days or weeks), and adjust their activity levels based on their assessment of earnings during the last period.

 %The pricing policy, along with the demand and supply functions together determine an equilibrium arrival rate of driver-arrivals $\lambda$ and passenger arrivals $\mu(A)$, as well as system throughput and revenue. Suppose the maximum potential rate of exogenous driver-arrivals is $\Lambda_0$. Based on the above discussion, the equilibrium rates of passenger requests and exogenous driver-arrivals must satisfy:
 %\begin{equation}
 %\mu(A)=\mu_0(1-F_V(P(A)))\qquad,\qquad\lambda^e=\lambda q_{exit}=\Lambda_0 F_C(\frac{\eta}{\iota+\tau})
 %\end{equation}

 %Where $\eta$ denotes the expected per-ride earnings, $\iota$ the expected waiting time for a
 %driver between rides, and $\tau$ the expected ride time. Exact expressions for these can
 %be computed from standard Markov chain theory; note though that $\eta$ and $\iota$ depend
 %on $\lambda$ and $\mu$, as well as the pricing policy $P(A)$.






We compare the aforementioned mechanisms of online pricing in ridesharing.
As summarized in Table \ref{tab:ridesharingpricing}, the three mechanisms  motivated from different aspects have the same goal of maximizing the overall utility, on top of pricing models with auction or game theory.


%\cite{bimpikis2019spatial,ma2018spatio} discusses the situation in two-sided market pricing.  \cite{fang2017prices} characterizes the equilibria among owners and renters given a fixed market price. \cite{banerjee2016dynamic} is based on the equilibrium rates of passenger requests and exogenous driver-arrivals.

%We list some of the features of the model in the table. In conclusion, the ridesharing pricing is still faced with many difficulties. Future work could concentrate on the following perspectives: The DnW method is a better version of the Greedy method. Although it reaches maximized overall utility, the platform utility could be negative according to experiment. How to obtain better platform utility without the loss of overall utility can be a major problem.
%STP assumes complete information and a finite planning horizon. Future work can generalize the model to settings where there is uncertainty in demand/supply prediction, and where the planning horizon rolls forward as the uncertainty gets resolved over time. Besides, we can consider the situation that drivers could choose to accept the dispatch.%Besides, platform Pricing Strategy considers a static pricing setting and looking at dynamic pricing more generally in two-sided sharing platforms remain a difficult problem. Besides, incorporating constraints on matching, and understanding how these impact prices, is a challenge to be solved.
%The Queueing-theoretic Economic Model is built on a two-side market with the goal to maximized satisfaction to both sides. Future work can consider multi-side market situation.


\subsection{Online Advertisement Auction}

As emphasized in Section~\ref{subsec:sn-model}, viral advertising in social networks is playing an important role for the promotions of new products, ideas, and innovations.
%Online advertisement pricing is an important application.
Search engines act as platforms and sell ad-spaces to enterprises who would like to display their products or services.
When a user sends a query to the search engine, the system finds a set of ads with keywords that match the query and determines which ads to show and where to show them.

 %The next example will give a brief introduction of the online ad auction.

 %Example 1. Online ad auction\cite{constantin2009online}. Many advertisers (bidders) use Internet systems to buy display advertisements on publishers? webpages or on traditional media such as radio, TV and newsprint. They seek a simple, online mechanism to reserve ad slots in advance. On the other hand, media publishers (sellers) represent a vast and varying inventory, and they too seek automatic, online mechanisms for pricing and allocating such reservations. Such mechanisms can be established using data pricing knowledge.

% Consider one platform and two bidders' situation. The expected revenue of the advertisement can be represent by revenue per click (RPC). For these two bidders A and B with the RPC \$0.5 and \$0.4, their highest bids are \$0.5 and \$0.4. Bidders have to compete with others under the circumstance that they can profit. The platform will choose the highest bid that they can offer. Suppose that the click numbers are the same for A and B, then A will win the auction since A can bid higher than B.

The major problem in this scenario is to determine the price and the allocation of the ad-space.
There are two key issues in online ad  markets,  making it infeasible for data trade.
First, ad-space is not a replicable good.
Unlike data, for any particular user on an online platform, at any instant in time, only a single ad can be shown in an ad-space \cite{agarwal2018marketplace}.
It is more like a traditional auction where the ad-space belongs to the highest bidder.
Second, buyers of online ad-space have a strong prior on the value of a particular ad-space.
For example, a pharmaceutical company has access to historical click-through rates (CTR) for a specific keyword. It is possible for firms to make separate bids for different ad-spaces based on access to past performance information.
In most cases like \emph{Baidu}, the biggest search engine in China, the first ad-space is always more expensive because people prefer to click the first thing they see.
Table \ref{tab:auc} lists three algorithms with the used pricing models, the respective objectives, and the main techniques they employed. %contains the comparison among above algorithms. {\color{blue}It overviews aforementioned algorithms on their features and motivations. Whether models are user-centric or platform-centric and the theory they use are also discussed in the table.}

 %According to \cite{varian2009online}, another problem is that if we suppose that users who have positive experiences from ad clicks will increase their propensity to click on ads in the future, and those with negative experiences will tend to decrease their propensity to click in the future. Hence search engines may also consider various measures of ad quality in their choice of which ads to display.


%A pricing strategy based on market-based value per click \cite{chang2010designing} and a multi-dimensional values advertising method \cite{liu2006designing} are proposed to solve the pricing problem above.  %\cite{varian2007position} is a purely mathematical method based on Nash Equilibrium. The work in \cite{zhang2014optimal} goes beyond contextual advertising by motivating the bidding focused on user data. It is different from the sponsored search auction where the bid  price is associated with keywords.



 %According to specific settings of \emph{The Trading Agent Competition Ad Auction (TAC AA)} \cite{chang2010designing}, designing a successful agent mainly faces two challenges: \\
 %(i) Without knowledge of bid prices of other participants, what is the optimal position and how to decide an appropriate bid price to target it?\\
% (ii) Given nondeterministic conversion limit, how to maximize profit in terms of both number of conversion and conversion value?

 %To address the first problem, we find an alternative way to build bid prices on Market-based Value Per Click (MVPC) which can be estimated based on system parameters or market reports. To overcome the second challenge, we estimate the true maximum number of conversions allowed by distribution capacity and select only the most profitable queries to bid on and fill the expected conversion allowance every day.

%To address the problem of limited information between agents and the nondeterministic conversion, an alternative way is to build bid prices on market-based value per click (MVPC), which can be estimated based on system parameters or market reports \cite{chang2010designing}. %shown in the figure 2.
%
% \begin{figure}		
%	\centering
%	\includegraphics[width=0.4\textwidth]{application-figure1.eps}
% 	\caption{TAC AA Server\cite{chang2010designing}}
%\end{figure}

%AstonTAC is composed of four components: Agent Knowledge Base, Bid Price Generator, Query Selector and Ad Display Selector. The main idea of bid price generator is to divide the whole game into two phases based on availability of market reports. Bid price generation in both phases is based on the same concept - Market-based Value Per Click (MVPC) - of each query, which is the expected conversion revenue minus advertising cost that a click on its ad can generate. One goal for the AstonTAC is to integrate the strategy with large-scale budget constraint optimization approach \cite{kitts2004optimal} and apply the agent in a real pay-per-click auction.


%According to specific settings of \textbf{AstonTAC} it proposed,

Designing a successful agent mainly faces two challenges  \cite{chang2010designing}.
i) Without knowledge of bid prices of other participants, how to find the optimal position and how to decide an appropriate bid price to target it.
ii) Given nondeterministic conversion limit, how to maximize profit in terms of both number of conversion and conversion value?
In order to address the first problem, an alternative way is to build bid prices on market based value per click (MVPC), which can be estimated based on system parameters or market reports.
In order to overcome the second challenge, the proposed AstonTAC model \cite{chang2010designing} estimates the true maximum number of conversion allowed by distribution capacity.
It selects only the most profitable queries to bid on and fill the expected conversion allowance every day.
AstonTAC reflects the dynamic change of the market, and thus leads to the generation of flexible and adaptive bidding prices.

 %In phase one, MVPC is estimated using expected revenue-per-click multiplied by a fixed discount ratio $r_{discount}$ indicating the proportion of profit in revenue. Expected revenue-per-click is a product of expected conversion value and conversion rate. Because MVPC is\quad based on static fundamental information, it is denoted as $v_{static}$
 %\begin{equation}
 %v_{static}=P_{conversion} v_{con} r_{radious}
 %\end{equation}


 %And $v_{con}$ is given by:
 %\begin{equation}
 %v_{con}=\begin{cases}
 %USP(1+MSB)	\qquad 	if\quad q_m=MS\\
 %\frac{2}{3} USP+\frac{1}{3} USP(1+MSB)	\qquad	if\quad q_m=null\\
 %USP	\qquad	otherwise
 %\end{cases}
 %\end{equation}\\
%where USP (Unit Sale Price) is the standard conversion value, MSB=$0.5$ is MS bonus rate\cite{jordan2009ad} and $q_m$ denotes the manufacturer part of a query.

% And	$ P_{conversation} $is calculated in a similar way.
 %\begin{equation}
 %P_{conversation}=\begin{cases}
 %\frac{(1+CSB)\pi_l}{1+CSB\pi_l} \qquad if\quad q_c=CS\\
 %\frac{2}{3} \pi_l+\frac{(1+CSB)\pi_l}{3(1+CSB\pi_l)}	\qquad	if\quad q_c=null\\
 %\pi_l \qquad otherwise
 %\end{cases}
 %\end{equation}

  %Together bid of each query in phase one is given by:
 %\begin{equation}
 %b_0=v_{static} h_q h_c
 %\end{equation}

 %In phase two dynamic MVPC denoted by $v_{dynamic}$ is calculated according to dynamic market reports. Consequently, a query's bid $b$ in phase two is built on its $v_{dynamic}$ and adjusted by distribution capacity adapter $\delta$ and ranking mechanism adapter $\beta $ simultaneously.
% \begin{equation}
% b=v_{dynamic} \delta \beta
% \end{equation}

 %\emph{Dynamic MVPC}  The following formula incorporates information about a query's revenue, cost and clicks from recent W (W is the size of aggregation window for distribution capacity. Specifically, W=5) days to calculate average profit of a click so far as the expected profit a click can possibly make on the next day.
 %\begin{equation}
 %v_{dynamic}=\frac{\sum_{i=d-1}^{d-W}revenue_i-\sum_{i=d-1}^{d-W}cost_i}{\sum_{i=d-1}^{d-W}click_i}
 %\end{equation}

 %As a result of the above formula, $v_{dynamic}$ is highly responsive and adaptive to the change of environment represented by three key factors: \\
 %(i) \emph{Search user population} -it determines the baseline number of possible clicks, conversion and revenue.\\
 %(ii) \emph{Competition intensity}- it determines the ad rank and cost-per-click.\\
 %(iii) \emph{Conversion probability}- it determines the number of clicks needed to generate a conversion.\\

The majority of auction design literatures has made assumptions that, bidders' valuation can be ordered along a single dimension, largely to facilitate solving the design problem.
However, in reality, advertisers may differ both on their valuation per click on their advertisements and on their abilities to generate clicks \cite{liu2006designing}.
To accommodate the underlying bi-dimensionality of bidders' valuation, Google's approach is that each advertiser submits a bid on how much they are willing to pay for every click, and the assignment of advertising slots is based on a score rule that weighs advertisers' bid price by their past CTRs.
The main idea of this algorithm \textit{unit-price contract} (UPC) is that, every advertiser gets a signal about its expected CTR and learns its valuation-per-click before the auction.
Each advertiser then places a bid $b$ as its pay per click. The intermediary selects the winner based on the pre-announced score rule.
The winner's advertisement is displayed in the slot during the period. At the end of the period, the winner pays the intermediary according to the actual number of clicks at unit price $b$.

 %The above Unit-price Contract (UPC) auctions obtains two features: \\
 %(i) Advertisers bid unit prices, and winners pay for the actual clicks at unit prices determined by the auction. Hence, advertising intermediaries essentially sell \emph{unit-price contracts} to advertisers.\\
 %(ii) The allocation is based on a score rule that weighs bids by a factor that incorporates the available information on other dimensions of bidders' characteristics.


% All advertisers are risk-neutral. Each advertiser's total valuation for the advertising slot is its valuation per-click, $v$, times the number of clicks it can generate, $r$, which, in our case, coincides with its click-through rate. An advertiser's payoff from winning the slot is additive in its total valuation for the slot and the money it pays, that is, if an advertiser pays	 P for the slot, its payoff from winning is given by
 %\begin{equation}
 %U=rv-q
 %\end{equation}


 %Each advertiser learns its own valuation-per-click before the auction, but not others'. All advertisers and the intermediary hold a common belief about the distribution of $v$, denoted as $F(v)$. We assume $F(v)$'s density function, $d(v)$, has a fixed support $[0,1]$, and is positive and differentiable everywhere within the support. We let $F(v) = 1$ for all $v > 1$.

 %Then we define a signal $\theta_{sig}$ for every advertiser to make an inference about its own future click-through rate. To simplify our analysis, we assume $h\in{L,H}$. Advertisers who receive signal H have high expected CTR, $E_H = E[r|h =H]$, and those who receive signal L have low expected CTR, $E_L=E[r|\theta=L](E_L<E_H)$

 %Let $\gamma$ ($\gamma>0$) denote the weighting factor for L-type advertisers. The score for an advertiser who receives a signal $\theta_{sig}$ and places a bid $b$ is given by:
 %\begin{equation}
 %s(b,\theta)=\begin{cases}
 %b,\qquad if \; \theta_{sig}=H\\
 %\gamma b,\qquad if \; \theta_{sig}=L
 %\end{cases}
 %\end{equation}


 %The intermediary's problem is to choose c to maximize its expected revenue or the resource-Allokation efficiency. By allowing c to take different values, we can accommodate different auction formats.
 %The main idea of this algorithm UPC is that every advertiser gets a signal about its expected CTR and learns its valuation-per-click before the auction. Each advertiser then places a bid $b$ as its pay per click. The intermediary selects the winner based on the pre-announced score rule specified in above formula. The winner's advertisement is displayed in the slot during the period. At the end of the period, the winner pays the intermediary according to the actual number of clicks at unit price $b$.

When a user's search query matches a keyword, a set of ads is displayed. These ads are ranked by bids (or a function of bids), and the ad with the highest bid receives the best position, i.e., the position that is mostly likely to be clicked on by the user.
If the user clicks on an ad, the advertiser is charged an amount that depends on the bid of the advertiser below it in the ranking. To solve this problem, a \textit{symmetric Nash equilibrium} (SNE) model  is proposed to model the position auction as a simultaneous move game with complete information \cite{varian2007position}.
Each agent simultaneously chooses a bid $b_a$. The bids are then ordered. The price each agent must pay per click is determined by the bid of the agent below him in the ranking, and finally the system reaches the equilibrium.


%In equilibrium, each agent should prefer his/her current slot to any other slot, which motivates the following definition. Note that if an agent changes his/her bid slightly, it normally won't affect his position or payment. So, there will typically be a range of bids and prices. The analysis of the position auction is much simplified by examining a particular subset of Nash equilibria.

% \textbf{Definition 1} A Nash equilibrium set of prices (NE) satisfies
 %\begin{equation}
 %(v_s-p_s)x_s \ge (v_s-p_t)x_t \quad for\quad t>s
 %\end{equation}
 %\begin{equation}
 %(v_s-p_s)x_s \ge (v_s-p_{t-1})x_t \quad for\quad t<s
 %\end{equation}

 %Where $v_s$, $p_s$ and $x_s$ can be interpreted as the value, price and the click-through rate for slot $s$.

 %Note that if an agent changes his bid slightly it normally won't affect his position or payment, so there will typically be a range of bids and prices.
 % that satisfy these inequalities. Also note that these inequalities are linear in the prices. Hence, given $(v_s)$ and $(x_s)$ we can use a simple linear program to solve for the maximum and minimum equilibrium revenue attainable by the auction.

 %The analysis of the position auction is much simplified by examining a particular subset of Nash equilibria.
 %\textbf{Definition 2} A symmetric Nash equilibrium set of prices (SNE) satisfies
 %\begin{equation}
 %(v_s-p_s)x_s \ge (v_s-p_t)x_t \quad \forall t,s
 %\end{equation}
 %\begin{equation}
 %v_s(x_s-x_t) \ge p_s x_s-p_t x_t \quad \forall t,s
 %\end{equation}

 %Note that the inequalities characterizing an SNE are the same as the inequalities characterizing an NE for $t>s$.

%Besides, the model SNE is purely mathematical. Applications to ad auctions will be discussed and improved. In general, these supporting prices can only be calculated using a linear program or related algorithm.



%For the UPC algorithm, the bidders' involvement is not much.
%One interesting thing is to look at cases where bidders are able to manipulate their signals and the situation advertisers do not know others' past performance.
%Future work can further investigate on the bidding function which directly covers the bid request features, not the KPI alone and dynamic approaches which tune the bid according to the specific current performance can be considered in the framework.

 %As more economic transactions take place online, we will likely see other novel pricing mechanisms arise.
 \begin{table*}
 	\centering\footnotesize %\setlength{\tabcolsep}{2pt}
 		\caption{Overview of Advertisement Auction Mechanisms}
 	\begin{tabular}
 		{llll}
 		\toprule[0.7pt]
 		\textbf{Algorithm}&\textbf{Pricing model}&\textbf{Objective}&\textbf{Technique} \\
 		\midrule[0.5pt]
 		AstonTAC \cite{chang2010designing} &game theory based model &maximizing revenue & market-based value per click
 		 \\
 		UPC \cite{liu2006designing} &auction based model &maximizing revenue &a score rule weighing bid prices \\
 		SNE \cite{varian2007position}&game theory based model &maximizing revenue &Bayes-Nash equilibrium
 		 \\
 		\bottomrule[0.7pt]
 	\end{tabular}
 	\label{tab:auc}
 \end{table*}
\end{comment}

 \subsection{Data Trade with Blockchain}
\label{subsec:blockchain}


Blockchain has a number of attractive advantages, so it has been widely applied in many areas: cryptocurrency, finance,
and notary, etc.
The first advantage of blockchain is decentralization, which is realized by various types of consensus mechanisms.
By decentralization, the blockchain technology removes intermediaries, and hence reduces total costs.
Secondly, blockchain ensures unalterability of any information recorded on it, so it can be used to store important
information like certificates, contracts, etc.
Thirdly, blockchain with programmability can be used to realize complex digital contracts, which are called smart contracts over blockchain.
Additionally, the native cryptocurrency of blockchain provides a convenient way of peer-to-peer payment.



On the other hand, as the value of data has been recognized by organizations and individuals, data has become precious assets and been sold on trading platforms. There have emerged some data trading platforms such as {\color{blue}Microsoft Azure Marketplace~\cite{azure}, GBDEX \cite{gbdex}, Infochimps~\cite{infochimps}, etc.}
Although data trading platforms provide a way of sharing data from different sources, it suffers from drawbacks of data leakage, high cost, and unfairness \cite{guan2018secure}.
Firstly, different from physical assets, data can be easily copied with nearly zero cost. Thus, it is highly possible that, data trading platforms make a copy of the data to be sold and resell it for profit.
Secondly, data trading platforms charge very high transaction fee for data trading.
For example, GBDEX charges 40\% for each data exchange, data owners only get 60\% of the data payments.
Lastly, it is difficult to achieve fairness in data trading without a trusted third party.
If data trading platforms are removed to reduce transaction fee, fairness in data trading without any
trusted third needs to be guaranteed.
%Therefore, it is highly challenging to achieve data privacy, TTP-freeness and fairness in data trading at the same time.

To this end, based on the blockchain technology  and the hash chain micro-payment technique, two data trading schemes for data trading platforms are designed in order to achieve data privacy and   fairness in data trading \cite{guan2018secure}.
The first scheme realizes raw data trading, while the second one realizes data statistics trading.
Both systems involve three entities: a blockchain, a data owner, and a data consumer.
Both the data owner and the data consumer have access to the blockchain system to make transactions.
Let $O$ and $C$ be the data owner and data consumer, respectively.
It assumes that, $O$ and $C$ generate their own public key and private key pair respectively,
and the public key corresponds to an account address.


\textbf{Raw data trading scheme}.
The raw data trading scheme consists of six steps, namely data preparation, encrypted data publication, hash chain generation, fund deposit, (off-blockchain) data transaction, and payment settlement.
Assume that the data is generated periodically in real time, e.g., real-time medical data like blood pressure, heart rate.
%The data owner $O$ encrypts each data item with a different key, where $O$ uploads the encrypted data to the blockchain.
%By doing this, the real-time data cannot be modified later once its hash is recorded by the blockchain.
%There exists some cross-verification method of this data so that $O$ cannot forge data without detection.
The data owner $O$ and the data consumer $C$ trade data with a dedicated \emph{smart contract}, which essentially serves as a trusted third party.


The data owner $O$ first generates data encryption keys with a specially designed key generation algorithm,
then he encrypts data records with different encryption keys.
Next, the encrypted data records are processed, which along with the encrypted data records is uploaded to the smart contract.
On the other side, the data consumer $C$ uses the hash chain micro-payment technique to prepare payments for the encryption keys.
The data consumer $C$ generates a long hash chain whose length is exactly the size of the data records, and then $C$ makes a payment commitment by depositing the total payment to the smart contract.
Each hash value on the hash chain represents a piece of micro-payments for data records.
In the subsequent, $C$ and $O$ exchange an encryption key and a hash value one-by-one off-blockchain.
In the end, $O$ can send the latest hash value obtained from $C$ to the smart contract to claim his due payment.


 \textbf{Data statistics trading scheme}.
The data statistics trading scheme consists of the following process, i.e., data preparation, Merkle accumulative tree (MAT) generation,
encrypted data publication, hash chain generation, fund deposit, (off-blockchain) statistics vectors transaction,
data statistics, and payment settlement.
The main idea of encryption is to use vectors containing only $0$ and $1$ to represent scalars such as age, height, and weight, and then encrypts these vectors by multiplying a secret invertible matrix.
%This encryption method does not depend on any NP problem, and it is also additively homomorphic.
%To avoid the same data being encrypted into the same ciphertext, the vectors should be extended with $n$ random real numbers before encryption, where $n \ge 1$.
When the encrypted data is uploaded to the blockchain, the data consumer $C$ can obtain statistics of these encrypted medical data records with statistics vectors, which can be obtained from data owner $O$ through off-blockchain transaction.


%\begin{table*}[t]
% 	\centering\footnotesize %\setlength{\tabcolsep}{2pt}
% 		\caption{Comparison over Data Trade in Real-life Applications}
%    \begin{threeparttable}
% 	\begin{tabular}
% 		{lllll}
% 		\toprule[0.7pt]
% 		\textbf{Application}&\textbf{Seller}&\textbf{Buyer}&\textbf{Broker}&\textbf{Trustness} \\
% 		\midrule[0.5pt]
%        mobile crowd sensing     &smartphone users & task requesters & MCS platform             & no  \\
% 		real-time ridesharing    &drivers          & passengers      & ride-sharing platform    & no  \\ 		
% 		online ad auction        &search engines   & advertisers     & the system               & no  \\
% 		trade with blockchain    &data owner       & data consumer   & the blockchain           & yes \\
% 		\bottomrule[0.7pt]
% 	\end{tabular}
%%  	\begin{tablenotes}
%%  	\footnotesize
%%  	\item The replicability of product means whether or not the product can be reproducible. For example, the data itself is reproducible, but the ad auction is not because there are only limited numbers of ad spots. Besides, we study the theory used in model building and whether the overall welfare is maximized in the table.
%%     \end{tablenotes}
%  	\end{threeparttable}	
%\label{tab:App}
% \end{table*}


\textcolor[rgb]{0.00,0.00,1.00}{In summary,  data trade with blockchain considers the issues of privacy, fairness, and efficiency in data trade, while pricing in crowd sensed data markets provides solution without concerning
trustness.}
%consists of the comparisons on the applications we have introduced in this section, from the aspects of data seller, data buyer, and broker, in which only data trade with blockchain considers the issues of privacy, fairness, and efficiency in data trade.


%.  The replicability of product means whether or not the product can be reproducible. For example, the data itself is reproducible, but the ad auction is not because there are only limited numbers of ad spots. Besides, we study the theory used in model building and whether they are highly related to data.
     %The replicability of product means whether or not the product can be reproducible. For example, the data itself is reproducible, but the ad auction is not because there are only limited numbers of ad spots. Besides, we study the theory used in model building and whether the overall welfare is maximized in the table.



 %\subsection{Online assortment and pricing in revenue management}

 %Consider an airline website selling parallel flights, i.e. different flights which depart from the same origin to the same destination around the same time. Each flight represents one kind of item to be sold, and its capacity represents the number of inventories of that item. Each flight has multiple fare classes (e.g. Economy, Basic Economy) which correspond to prices at which that item could be sold. We will refer to this collection of initial information (items, inventories, prices) as the setup condition.

 %Over the booking horizon, customers sequentially arrive to the airline's website to book the ticket. We assume that the airline can reliably estimate each customer's choice probabilities from historical data. That is, upon a customer's arrival, for any combination of items and prices that could be shown, the stochastic distribution of how the customer would choose among those items/prices is given. The customer is assumed to choose at most one item and one price, as the flights are parallel. The customer could also choose to make no purchase. Given the choice probabilities, the
 %airline selects an assortment of items and corresponding prices to show the customer, where items with zero remaining inventory cannot be shown. The customer's decision is realized immediately afterward, and if she makes a purchase, then the airline earns the corresponding price as revenue, and depletes one unit of inventory of the corresponding item. The airline wants to maximize its cumulative revenue earned before the booking horizon is over (or all the flights are full).

 %\textbf{A Bid Price Algorithm when Items have Multiple Prices}

 %Suppose that there are parallel flights, whose seats have the same two fare classes: a lower price of $p^{(L)}=150$, and a higher price of $p^{(H)}=450$. At any point in time, for each flight i, let wi denote the fraction its starting inventory which has been sold. The algorithm would associate each fare class $j\in {L,H}$ of each flight $i$ with a 'pseudorevenue' equal to\\
 %\begin{equation}
 %p^{(j)} \mathcal{M}(w_i)
 %\end{equation}

 %Where $\mathcal{M}$ is a decreasing function that penalizes the revenues associated with flights i which are almost full. The algorithm then offers, to each customer, the assortment which maximizes the expected pseudorevenue of the (flight, fare)-combination that the customer would choose.

 %Although $\mathcal{M}(w_i)$ will disincentivize the offering of a flight i whose $w_i$ is large, the algorithmhas no way of setting a \textbf{booking limit} preventing sales at the lower price  $p^{(L)}$ while still allowing sales at price $p^{(H)}$ .Given a stream of customers who are only interested in the lower price, the algorithm would sell all the seats at price $p^{(L)}$, without realizing the opportunity cost of $p^{(L)}$ it gave up. Since this could happen to every flight $i$, the algorithm's competitiveness is at most $\frac{p^{(L)}}{p^{(H)}}$.

% To improve upon this, our algorithm must implement some notion of \textbf{booking limit}. As a result, we define the pseudorevenue associated with fare class $j$ of flight $i$ to be
 %\begin{equation}
 %p^{(j)}-\mathcal{W}(w_i).	
 %\end{equation}

 %where $\mathcal{W}$ is an increasing function that sets a cost to selling flights $i$ which are almost full. Multi-price Balance uses the same idea of maximizing expected pseudorevenue, with the modification that it rejects the customer outright if the maximum expected pseudorevenue is non-positive.


 %$\mathcal{W}(w_i)$ can be interpreted as a bid price, or the value placed on one unit of item i's inventory. Optimizing based on bid prices is a classical idea in revenue management where typically the bid prices are computed
 %using a large LP which encompasses both the inventories and the forecasted distribution of future
 %customers. However, since we make no assumptions about future customers, our bid prices are
 %based on only the remaining inventories, like the balance algorithms from competitive analysis.

 %\subsection{Predication Markets}

 %See \cite{wolfers2004prediction} for a detailed overview. Such markets are a recent phenomenon and have generated a lot of interest. Typically in such markets, there is a discrete random variable, denoted by $W$, that a firm wants to accurately predict. The market executes as follows: (i) ``Experts'' sell probability distributions $\Delta W$, i.e., predictions on the chance of each outcome; (ii) the true outcome, denoted by $w$, is observed; (iii) the market pays the experts based on $\Delta W$ and $w$. In such literature, payment functions such as those inspired by Kullback Leibler divergence are utilized as they incentivize ``experts'' to be truthful (cf. \cite{hanson2012logarithmic}). Despite similarities, prediction markets remain infeasible for data - ``experts'' have to explicitly choose which tasks to make specific predictions for. In contrast, it is not known a priori whether a particular dataset has any importance for a prediction task (moreover, the predictive value of a data stream can rapidly change over time). Thus a data market must instead have a real-time mechanism to match training features to prediction tasks based on empirical predictive value.

 %\subsection{Revenue Allocation}

 %In our model (as seen in Section 2.2), only an aggregate payment is made from a buyer of data whereas the marketplace is designated with fairly allocating the revenue among the
 %sellers. Following the seminal work in [31], there has been substantial progress in fairly allocating
 %revenue among cooperating entities. Efficient algorithms for computing the Shapley allocation have
 %been studied in [23] and [6].


==> auction-model.tex <==


\subsection{Auction based Pricing Model}
\label{subsec:tsm-model}

The auction based pricing (ACP) model is one of the most popular data pricing mechanisms.
An auction is an economically-driven scheme, which aims to allocate commodities and establish corresponding prices through buyers' and sellers' bidding process \cite{liang2018survey,mcafee1992dominant}.
The auction theory has been well explored in several areas {\color{blue}\cite{an2017soda,an2017sto2auc,iosifidis2013iterative,yang2002efficiency}}, such as economic, electricity market, mobile market, among others.


For example, in the online matching problem, the drivers act as auctioneers and the customers act as bidders.
Customers offer the bonus and bid the driving service  \cite{zheng2019auction}.
In crowd sensing scenarios {\color{blue}\cite{shah2015profit,wang2017towards,yang2012crowdsourcing} and online advertisement auction \cite{liu2006designing,varian2007position,zhang2014optimal}, the proposed models are also based on auction theory.
Moreover, combining game theory and auction theory  is a natural way to decide the pricing strategies, e.g., in smart grid \cite{ghosh2004game,srinivasan2017game}.}
Further description can refer to  Section~\ref{sec:applicaiton}.

%Auction theory have been widely studied and used in the real economy. Data, as a special type of commodities, can be modeled by auction theory. However, there are some challenges when applying auction theory to data pricing. For instance, replicability of data is unique to other kind of products and this may lead to a more complex situation.
%
%The auction theory can be applied in to many fields.


%\subsubsection{Auction Basics}

Due to the strong capability of ensuring fairness and efficiency, auction mechanism shows great potential to address big data trading problems. Before a detailed review of related works on auction theory, there are some basic concepts of the auction mechanism as follows.

\begin{itemize}\setlength{\itemsep}{-\itemsep}
\item{} \emph{Bidder}: in the auction process, a bidder is the one who submits the bids and aims to buy commodities in the market.
\item{} \emph{Auctioneer}: the auctioneer plays the role of an agent who runs the auction process, enacts winner determination, and conducts payments and allocations.
\item{} \emph{Seller}: the seller is the owner of the commodities to be bid upon and sold. For example, it includes the utilities that generate, collect and store large-scale data from different platforms and devices for further sale.
\end{itemize}


%$\bullet$ \emph{Clearing price}: In the auction process, the seller and buyer submit asks and bids. %The asks indicate the asking price on the commodity to be sold while bids indicate the bidding price for the requested commodity. A clearing price will be determined by the auctioneer according to the optimization goal, such as social welfare maximization. In other words, the clearing price is the price at which the buyer and seller will make a deal.

\subsubsection{One-side Auction}

A one-side auction  can be treated as a seller-side auction, which refers to the auction with one seller and many buyers (i.e., bidders) to compete against each other {\color{blue}\cite{li2017bid,wu2017vcg}}.
For instance, a \emph{multi-rounds false name proof forward auction} (MFPA) mechanism enables effective data circulation among data producers and data users \cite{an2017towards}.
It is a one-side data auction market that consists of one data seller, many data buyers, and one auctioneer.
%The data owner and multiple reliable data collectors are treated as the seller and buyers, respectively.
The operation of the data trading market is coordinated by the auctioneer in the cloud, which is capable of making decisions on big data allocation among the buyers and the seller.

Particularly, it is worthwhile to mention that, the \emph{two sided-market} theory is an economic research field,  referred to markets characterized by the presence of \emph{cross-group network externalities}. Namely, those markets are characterized by the presence of platforms serving different groups of consumers linked with each other by network externalities.
	%the concept used by Rochet and Tirole (2006) to define the two-sidedness of a market.
According to the literature \cite{armstrong2006competition}, a market is said to be two-sided when the platform can affect the volume of transactions by charging more to one side of the market and reducing the price paid by the other side by an equal amount.
In other words, price structure matters are not neutral and, accordingly, platforms design it so as to bring both sides on board. %This non-neutrality of the price structure is case of failure of the Coase theorem, stating the optimal allocation in presence of externalities.
One intuitive example of two sided-market is online shopping platforms like Amazon and Taobao, buyers and retailers interact through an intermediary or platform to get the benefit of both parties. In general, the  two-sided markets are to describe industries in which the benefit for an agent belonging to a given group (side) depends on the number of agents in the other group.
%For this interaction to occur, it is required the birth of a platform able to internalize the externalities.

%The most general and simple frameworks are presented in the works of Rochet and Tirole (2003, 2006), Armstrong (2006) and Caillaud and Jullien (2003). Rochet and Tirole (2003) and Armstrong (2006) presented models in which platforms charge only a membership fee, while Rochet and Tirole (2006) Caillaud and Jullien (2003) use both types of prices following a more general approach.



\subsubsection{Double Auction}

Double auction is the auction where multiple sellers and multiple  buyers submit bids and asks to the auctioneer.
It is one of the most commonly used auctions in the real-world
scenarios, such as the New York Stock Exchange \cite{yang2002efficiency}, the smart grid \cite{an2017soda,li2017towards}, and the mobile market \cite{iosifidis2013iterative}. At the same time, some double auction mechanisms {\color{blue}\cite{cao2017iterative,susanto2017effective}} are designed in big data trading markets.

In the mobile crowd sensing data trading, an iterative auction mechanism \cite{cao2017iterative} guilds the selfish agents to behave in a socially optimal way without direct access to their private information.
In the mechanism, the auctioneer first announces the allocations, pricing, and auction rules for the data commodities to all consumers.
Then, each consumer computes the bidding price in order to maximize the utility.
Finally, the auctioneer receives the bidding prices and, according to the rule and price, announces the result. Those three steps also exist in common auction processes.
The unique aspect of the auction mechanism in \cite{cao2017iterative} is the fourth step, based on the prior auction process.
In this step, the auctioneer can adjust and re-announce a new starting price and some auction rules to start a brand-new auction.
This iterative auction process encourages consumers to announce a reasonable price during the auction process.
Besides, in the secondary mobile market, a double auction mechanism  \cite{susanto2017effective} enables mobile data to trade in a heterogeneous and dynamic environment. The theoretical analysis has proved that, the proposed double auction scheme is capable of achieving Nash equilibrium and truthfulness.

\subsubsection{Seal-bid Auction}

Seal-bid auction refers to the auction where the buyers privately submit their bids to the auctioneer \emph{without} knowing the bidding information of other buyers.
For example, the government wants to build a new park, and many contractors can bid to get the job. They privately submit their bids and plans to the auctioneer (i.e., the government in this case). This process can be viewed as a seal-bid auction.
Unlike conventional auctions, the seal-bid auction is a one-time auction, and leads to a non-open competition for the buyers.

Seal-bid auctions have been well explored, and typical examples include the $k$-th price auction \cite{kirchkamp2009outside}, Vickrey-Clarke-Groves (VCG) auction {\color{blue}\cite{ausubel2006lovely,nisan2007computationally}}, and McAfee auction \cite{mcafee1992dominant}.
Recall that the $k$-th price auction can be divided into the first price auction  and the second price auction. In the first price auction, the winner is the bidder who submits the highest bidding price and would thus pay the highest price to win the auction.
In the second price auction, which is also known as Vickrey auction, the winner is the bidder who submits the highest bidding price, while the winner would pay the second highest price to win the auction.
Besides, a class of single round, sealed bid auctions for items in unlimited supply such as digital goods is also studied in \cite{goldberg2001competitive}. Notice that the first price auction ensures the maximum profit of the seller, while the second price auction induces the buyers to report truthfully, ensuring the fairness of the auction scheme.
%Vickrey-Clarke-Groves (VCG) auction seems to be a generalized form of Vickrey auction.
Regarding the McAfee auction, it is an extension of Vickrey auction. Specifically, the buyers and sellers submit private bids to the auctioneer, of the buyers (resp. sellers) whose bidding prices are larger (resp. smaller) than a threshold price, and the winners would pay the highest price that does not win the auction.



%\cite{jiao2017profit} proposed an optimal price seal-bid auction market model based on the Bayesian optimal mechanism. First, the data sources are divided into three groups: Crowdsensing data, Social data, and Sensing data. Then, the cost function, satisfaction rate function, and data utility function are defined. Based on those functions, the starting prices of the data commodities are identified. During the Bayesian profit maximization auction process, the valuation distribution function was computed. Based on this function, the most optimal price point and secondary optimal price point were identified. Meanwhile, the optimal size of data that takes from those collectors is identified. Nonetheless, this auction scheme only considers one round of auctions.

\subsubsection{Combinatorial Auction}

The combinatorial auction considers the situation that, the bidders in the market are allowed to bid on combinations and bundles of the commodities.
Particularly, the bidders submit bids that contain the combination of a variety of commodities and
the price of the combination.
The auctioneer then makes the optimal allocation for the bidders according to their bids and asks.
In the data trading market, the buyers' demands for data and the  sellers' supplies  of data are always manifold. Thus, when applying the aforementioned auction schemes, both buyers and sellers cannot be satisfied by simply rubbing the data together to trade.
As a result, the combinatorial auction is designed for such a situation.

For example, in a single-round combinatorial auction \cite{pekevc2003combinatorial},
all bids are submitted before a deadline, then the winner determination problem is solved.
Items go to the revenue-maximizing collection of bids, and winners pay the amounts of their bids.
The main obstacle to implement such auctions is the complexity of solving the winner determination problem.
For reasonably sized and structured auctions, the state-of-the-art integer programming can overcome this obstacle for practical purposes. In fact, aforementioned combinatorial auctions are designed in this way {\color{blue}\cite{cantillon2007combination,elmaghraby2003technology,epstein2002combinational}}.


In summary, we compare different auction mechanisms in Table \ref{tab:auctionmodels}, where the second (resp. third) column is about whether auctions have multiple sellers (resp. bidders), the forth column indicates whether it is an open auction (which requires full and open information of all participants), and the last column means whether the corresponding auction supports the bid on combinations and bundles of the commodities.
To be specific, there is one seller and multiple bidders (i.e., buyers) in the one-side auction and seal-bid auction in the general case.
In contrast, the double auction has multiple sellers and multiple bidders, as well as the combinatorial auction.
In addition to the seal-bid auction without the bidding  information of other buyers, the other three auction mechanisms are open auctions, which have full information of all participants.
Besides, the bid on combinations and bundles of the commodities is only allowed in the combinatorial auction.




\begin{table*}[t]\footnotesize
 	\centering
 		\caption{Comparison over Different Auction Mechanisms}\label{tab:auctionmodels}
 	\begin{threeparttable}
 	\begin{tabular}
 		{lllll}
 		\toprule[0.7pt]
 		\textbf{Mechanism}&\textbf{Multi-sellers}&\textbf{Multi-bidders}&\textbf{Full information}&\textbf{Bundles available}\\
 		\midrule[0.5pt]
 		one-side auction&$\times$&$\checkmark$&$\checkmark$&$\times$\\
 		double auction&$\checkmark$&$\checkmark$&$\checkmark$&$\times$\\
 		seal-bid auction&$\times$&$\checkmark$&$\times$&$\times$\\
 	    combinatorial auction&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$\\
 		\bottomrule[0.7pt]
 	\end{tabular}
% 	\begin{tablenotes}
% 	        \footnotesize
% 	        \item The second and the third column are about whether auctions have multi-sellers or multi-bidders. The full information means an open auction which require full informations of all participants. The last column {\color{blue}contains} whether the bidders in auctions can bid on combinations and bundles of the commodities.
% 	      \end{tablenotes}
 	\end{threeparttable}
 	\end{table*}
%{\color{blue}Behavior Based Price Discrimination, Two-Sided Markets, Social Networks, Monopoly Pricing, Network-Based Pricing, Search Costs.}


==> fbmodel-1.tex <==
\vspace*{0.2in}
\section{Feature-based Data Pricing}
\label{sec:fbmodel}

%We will introduce five pricing models, i.e., personal data pricing using privacy, personal data pricing with market value, relational data pricing based on accuracy, XML data pricing based on completeness, and data pricing based on multi-dimension quality.


In this section, we elaborate four representative pricing models in the feature-based data pricing (FP) strategy, and then we compare them from several aspects.


%In this section, we first elaborate five pricing models in the query pricing (QP) strategy, and then we compare them from several aspects.

The FP strategy focuses on establishing a price for a dataset, instead of pricing a query like the QP strategy described in Section~\ref{sec:qpmodel}.
The FP strategy determines the data price based on data features, including the pricing model  based on data quality (i.e., F1), the personal data pricing model using data privacy (i.e., F2), the personal data pricing model with market value (i.e., F3), and the social network pricing model with influence (i.e., F4). The underlying idea of the FP strategy is that, it is possible to derive its \emph{intrinsic} value that could be represented by data \emph{features}, even though it is hard to obtain the \emph{true} value of data.


%In the following, we describe the FP strategy
%Since the true value of data is hard to obtain, several studies aim to price data based on its intrinsic value, i.e., data quality, data privacy, etc.
%Following this idea, there are \textcolor[rgb]{0.00,0.00,1.00}{}
%In this section, we overview feature-based data pricing models, \textcolor[rgb]{0.00,0.00,1.00}{and give an analysis of them.}

%\subsection{\textcolor[rgb]{0.00,0.00,1.00}{Quality-based Data Pricing}}
%\label{subsec:db-quality}

%\textcolor[rgb]{0.00,0.00,1.00}{Since the true value of data is hard to obtain, several studies aim to price data based on its intrinsic value, i.e., data quality.
%Following this idea, there are two kinds of pricing models, including relational data pricing based on accuracy and XML data pricing based on  completeness.}
\vspace*{0.25in}
\subsection{Data Pricing based on Data Quality}
\label{subsec:fb-quality}


The data pricing model  based on data quality (i.e., F1) attempts to price various data from the perspective of data quality in different dimensions.


The  price derived by F1  concentrates on the datasets' statistic property, and thus it is easily understood and employed.
The idea of  F1 has been widely used in real life.
For example, YoueData adopts the incompleteness degree as a factor of rating the sold data~\cite{youedata}.
However, the feature of data quality only partly reflects the inherent value of data, which is insufficient to represent the true  value of data.

%{\color{blue} add the F1 pricing model's cons and pros and its application scenarios.}

%There are several studies in Q1 focusing on how to price data based on data \emph{quality}~\cite{tang2013you,tang2014get,yu2017data}.

\vspace*{0.015in}
First, based on the idea of ``what you pay for is what you get'', a theoretical and practical pricing framework trades data quality (more specifically, data accuracy) for discounted prices \cite{tang2013you}.
 In particular, the data buyer is free to propose his own price for data.
If the data consumer is able to afford the full price $p$ of the data, he/she will get them directly.
Otherwise,  an inaccurate version of data is returned to the data consumer according to his/her bid $p_b$ and the full price $p$.
The lower the price, the more inaccurate the answer.
{\color{blue}This model also belongs to posted pricing mechanism, where the price is posted by the buyers, instead of sellers/markets in previous pricing models.
}
%different from post pricing and auction, since the price is derived by consumers and every consumer can obtain data based on his/her bid $p_b$.


\vspace*{0.015in}
To be more specific, the true value of each tuple is modeled as a degenerate distribution.
In the case of a discounted price, the inaccurate tuple value is randomly determined from a probability distribution.
The distance of the distribution to the degenerate distribution is measured through earth movers distance (EMD), which is commensurate to the discount, i.e., $p_b/p$.
Moreover, the returned tuple value is drawn from the distribution with a guaranteed probability,  which is also commensurate to the discount.
Each tuple in required data is treated through the above process, thus the whole inaccurate data are traded to the consumer.
%In particular, this model first derives the tuple that the data consumer would like to purchase, and then it receives the price he/she can accept.
%If the data consumer is able to afford the full price of the tuple, he/she will get it directly.
%Otherwise, an inaccurate tuple answer is returned to the data consumer according to the bid and the full price.
%The lower the price, the more inaccurate the answer.
%It can be seen as {\color{blue}\emph{inverse} pricing}, since the price is derived by consumers.
%Also, it is different from the auction mechanism, as every consumer can obtain an answer based on his/her bid.

%\begin{comment}
%It is better to formally describe the definition of inverse pricing and also attach some references.
%\end{comment}
%To be more specific, the distribution of an exact tuple is modeled as a degenerate distribution.
%For example, if the tuple ID is 1, and the possible \textcolor[rgb]{0.00,0.00,1.00}{answer tuple set is $\{1,2,3,4\}$}, then the degenerate distribution can be formed as $(1,0,0,0)$.
%In the case of a discounted price, the inaccurate tuple value is randomly determined from a probability distribution.
%And the distance of the distribution to the actual \textcolor[rgb]{0.00,0.00,1.00}{tuple} (to the degenerate distribution) is measured through earth mover¡¯s \textcolor[rgb]{0.00,0.00,1.00}{distance (EMD)}, which is commensurate to the discount.
%Meanwhile, the published \textcolor[rgb]{0.00,0.00,1.00}{tuple} comes with a guarantee on its probability, which is also commensurate to the discount.

\vspace*{0.015in}
Furthermore, following the idea of ``what you pay for is what you get'', a pricing framework for trading XML data considers the case of XML documents with completeness as the trading products \cite{tang2014get}.
The data completeness is traded for a discount.
Specifically, the XML data is formed as a tree, and the completeness is defined as the weight ratio between the full tree and answered tree.
A sampling problem is derived  to find a subtree that satisfies the weight, which is with respect to a discount price.
%It is easy to find that, it also employs .
Meanwhile, the pricing mechanism is proved to be arbitrage-free, and the situation where consumers have repeated requests is also considered.
%Then, they identify the tractable cases in this problem, and provide polynomial time (PTIME)  solutions.

%belongs to inverse pricing.
\vspace*{0.015in}
Moreover, a novel pricing framework considers multi-dimensional quality features~\cite{yu2017data}, instead of solely considering one single data quality feature.
%This model prices data in a theoretical way, where multi-dimension quality features are considered.
%And the granularity of pricing is the dataset, since the multi-dimension quality is measured on different versions of dataset.
It has the assumptions that, there are multiple versions of datasets, and prices are based on multi-dimension quality.
In particular, the data cost is modeled as a linearly increasing function of quality levels on different dimensions.
Also, the willingness of data consumers is represented through a piecewise function based on multi-dimensional quality levels.
As a result, \textcolor[rgb]{0.00,0.00,1.00}{a bi-level programming problem is formulated for revenue maximization}, and a genetic algorithm is proposed to solve \textcolor[rgb]{0.00,0.00,1.00}{it}.

%\textcolor[rgb]{0.00,0.00,1.00}{Note that, the previously mentioned incomplete data pricing model~\cite{miao2020towards} also considers data quality, i.e., data completeness.
%However, we category it to the query pricing model, since it aims to pricing queries, and data usage/provenance is the main part in pricing.
%Overall, the pricing schemes based on data quality take data intrinsic features into account.}

%\subsection{Relational Data Pricing based on Accuracy}
%\label{subsec:fb-accuracy}
%
%This model \textcolor[rgb]{0.00,0.00,1.00}{prices a very small subset of the data, i.e., a tuple, and the price of tuple relies on its accuracy.}
%Different from aforementioned models, this model first \textcolor[rgb]{0.00,0.00,1.00}{derives the tuple that the data consumer would like to purchase, and receives} the price he/she can accept.
%\textcolor[rgb]{0.00,0.00,1.00}{If the data consumer is able to afford the full price of the tuple, he/she will get it directly.
%Otherwise, an inaccurate tuple answer is returned to the data consumer according to the bid and the full price.}
%Thus, the behind idea of this model is called ``what you pay for is what you get''.
%
%
%%data quality (more specifically, data accuracy) for discounted prices.
%A theoretical and practical pricing framework~\cite{tang2013you} is proposed, in order to \textcolor[rgb]{0.00,0.00,1.00}{trade data accuracy} for discounted prices.
%In the framework, tuple value answered to data consumer is determined by the full price of tuple and the consumer bid.
%The tuple provided to a data consumer is exact if he/she offers the full price for it.
%Otherwise, \textcolor[rgb]{0.00,0.00,1.00}{the answered tuple} is approximate when he/she offers to pay only a discounted price.
%The lower the price is, the more inaccurate the answer.
%In particular, the distribution of exact tuple is modelled as a degenerate distribution.
%For example, if the tuple ID is 1, and the possible \textcolor[rgb]{0.00,0.00,1.00}{answer tuple set is $\{1,2,3,4\}$}, then the degenerate distribution can be formed as $(1,0,0,0)$.
%In the case of a discounted price, the inaccurate tuple value is randomly determined from a probability distribution.
%And the distance of the distribution to the actual \textcolor[rgb]{0.00,0.00,1.00}{tuple} (to the degenerate distribution) is measured through earth mover¡¯s distance(EMD), which is commensurate to the discount.
%Meanwhile, the published \textcolor[rgb]{0.00,0.00,1.00}{tuple} comes with a guarantee on its probability, which is also commensurate to the discount.
%Ancillary pricing functions are defined to facilitate the necessary algorithms under several principles.


%\textcolor[rgb]{0.00,0.00,1.00}{In order to trade data quality for discounted prices, a theoretical and practical pricing framework~\cite{tang2013you} is proposed.
%The answer from model is determined by the full price of tuple and the consumer bid.
%In the framework, the data provided to a data consumer is exact if she offers the full price for it. The data is approximate if she offers to pay only a discounted price. In the case of a discounted price, the value of data is randomly determined from a probability distribution.
%The distance of the distribution to the actual value (to the degenerate distribution) is commensurate to the discount. The published value comes with a guarantee on its probability. The probability is also commensurate to the discount. Ancillary pricing functions are defined to facilitate the necessary algorithms under several principles.
%(more specifically, data
%accuracy)
%The structual granu}


%\subsection{XML Data Pricing based on Completeness}
%\label{subsec:fb-completeness}
%Similar with relational data pricing model based on accuracy, this model also employs the idea of ``what you pay for is what you get''.
%When consumer offers a price, this pricing model provides \textcolor[rgb]{0.00,0.00,1.00}{him/her} an incomplete XML data.
%%Since XML data is formed as a tree, the granularity of pricing is the tree produced by XML data.
%
%A pricing framework for XML data is explored~\cite{tang2014get}, which data \textcolor[rgb]{0.00,0.00,1.00}{completeness} can be traded for a discount.
%It considers the case of XML documents with completeness as the \textcolor[rgb]{0.00,0.00,1.00}{trading products.
%To be more specific, the XML data is formed as a tree,} and the completeness is defined as the weight ratio between the full tree and answered tree.
%Thus, a sampling problem is derived, in order to find \textcolor[rgb]{0.00,0.00,1.00}{a subtree that} satisfies the weight, which is related to the discount price.
%Then they identify the tractable cases in this problem, and provide \textcolor[rgb]{0.00,0.00,1.00}{polynomial time(PTIME)} solutions.
%The situation where consumers have repeated requests is also considered.
%
%\textcolor[rgb]{0.00,0.00,1.00}{For XML data which data quality can be traded for a discount, a pricing framework~\cite{tang2014get} is explored.
%It considers the case of XML documents with completeness as the quality dimension.
%Namely, a data provider offers an XML document, and sets both the price and weights of nodes of the document.
%The data consumer proposes a price but may get only a sample if the proposed price is lower than that of the entire document.}


%\subsection{Data Pricing based on  Multi-dimension Quality}
%\label{subsec:fb-multifeature}
%
%This model prices data in a theoretical way, where multi-dimension quality features are considered.
%%And the granularity of pricing is the dataset, since the multi-dimension quality is measured on different versions of dataset.
%
%This model assumes that, there are multi versions of datasets, and prices are based on multi-dimension quality~\cite{yu2017data}.
%In particular, the data cost is formulated as a linearly increasing function \textcolor[rgb]{0.00,0.00,1.00}{of quality} levels on different dimensions.
%Also, the willingness of data consumers is represented through a piecewise function based on multi-dimension quality levels.
%Thus, a revenue maximization problem is formulated, and a genetic algorithm is proposed to solve the problem.



\subsection{Personal Data Pricing using Data Privacy}
\label{subsec:fp-privacy}
%\vspace*{0.1in}





The amount of data in real-world is increasing at an amazing speed, and personal data accounts for a large part of it.
For instance, Facebook collected 300 petebytes of personal data in 2014~\cite{vagata2014scaling}.
However, personal data are difficult to share and use directly, due to the critical privacy concern.


The data market offers an important way to bridge the gap between sellers and buyers who are interested in personal data.
The personal data pricing model using data privacy (i.e., F2) takes into consideration the growing public concern about data privacy to promote personal data circulation.
%~\cite{li2014theory,li2017theory,niu2019making,niu2020online,niu2018unlocking,niu2019erato} .
%Thus, the pricing problem of personal data has been widely explored.


%These models price personal data based on different features, and we first introduce the pricing model using privacy in the following.

%\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Personal Data Pricing using Privacy}}
%\label{subsubsec:db-privacy}



%In the context of data pricing problem, a typical kind of data, i.e., personal data, has become a new asset in real world~\cite{pdata}.




%Recent studies~\cite{li2014theory,li2017theory,niu2018unlocking,niu2019making,niu2018achieving,niu2019erato} have been proposed to solve above problems, which build a pricing framework, as shown in Figure~\ref{PData basics}.

The problem of pricing private data is firstly studied in ~\cite{li2014theory,li2017theory} with
a typical pricing framework based on data privacy  shown in Figure~\ref{fig:PData}.
Similar as existing data markets, the pricing framework includes three parts, i.e., data owner, data broker, and data consumer.
The data broker is an intermediary agent between data owners and data consumers, which deals with the request from data consumer, determines monetary compensation of data owner, returns the noisy answer to data consumer, and prices the answer.

In particular, the request from data consumer can be formalized as $S=(\mathbf{q}, v)$, where $\mathbf{q}$ can be seen as a function that outputs some aggregate statistics, such as linear aggregate query, histogram count, weighted sum, mean, standard deviation, etc.
{\color{blue}To be more specific, the whole database is formulated as a data vector $\mathbf{x}$, which can be seen as the output of the function on the original data.
For example, each element $\mathbf{x}_i$ in $\mathbf{x}$ is the number of records that in specific domains, such as ``is the age greater than 18'', female, etc~\cite{li2017theory}.}

Moreover, the request $\mathbf{q}$ is also a vector, and the true answer of $\mathbf{q}(\mathbf{x})$ can be formulated as the vector product, i.e., $\mathbf{q} \mathbf{x}=q_{1} x_{1}+\cdots+q_{n} x_{n}$.
%The form of $\mathbf{x}$ is different in the studies.
%The data vector $\mathbf{x}$ is directly the output which concatenates each record in the numerical database~\cite{li2014theory}, while $\mathbf{x}$ is the number of records that in different domains~\cite{li2017theory}.
%Moreover, the element $x_i$ in $\mathbf{x}$ represents any general function on original data, such as quadratic polynomial function and nonlinear comparison~\cite{niu2018unlocking,niu2019erato}.
Note that, the data broker does not return the \emph{raw} data (like traditional SQL query does), since the original data is sensitive.
The parameter $v$ is the tolerable variance of noise added to the true answer.
Once the data broker receives the request, he/she not only needs to return the noisy answer, but also has to derive the price and privacy compensation.

%{\color{blue} To be more specific, the whole database is formulated as a data vector $\mathbf{x}$, which can be seen as a function of the original data.
%For example, $\mathbf{x}$ is the number of records that in different domains, such as ``is the age greater than 18'', gender, etc~\cite{li2017theory}.
%Moreover, the request $\mathbf{q}$ is also a vector, and the true answer of $\mathbf{q}(\mathbf{x})$ can be formulated as the vector product, i.e., $\mathbf{q} \mathbf{x}=q_{1} x_{1}+\cdots+q_{n} x_{n}$.
%The form of $\mathbf{x}$ is different in the studies.
%The data vector $\mathbf{x}$ is directly the output which concatenates each record in the numerical database~\cite{li2014theory}, while $\mathbf{x}$ is the number of records that in different domains~\cite{li2017theory}.
%Moreover, the element $x_i$ in $\mathbf{x}$ represents any general function on original data, such as quadratic polynomial function and nonlinear comparison~\cite{niu2018unlocking,niu2019erato}.}

%\vspace*{0.1in}
Based on this framework, two critical items in pricing problem are introduced, namely, (a) how to ensure privacy and compensate the data owners, and (b) how to derive \emph{arbitrage-free} price function.
To protect the privacy, \emph{Laplace} mechanism is employed to guarantee the dependent differential privacy~\cite{dwork2011firm}.
In other words, the returned answer is processed by adding noise to perturb the true value of answer, i.e., $S(\mathbf{x}) = \mathbf{q}(\mathbf{x})+Laplace(b),$ and $b = \sqrt{v / 2}$, so as to make it hard to infer private information.
By comparing the output of the randomized mechanism $\mathcal{M}$ over the data vector $\mathbf{x}$ and the data vector with absence of data owner $\mathbf{x}^{(i)}$ \cite{ghosh2011selling}, the individual privacy loss can be formulated as stated in Definition~\ref{defn:indi-privacy-loss}, which is used in~\cite{li2014theory,li2017theory,niu2018unlocking,niu2019erato}.

%On the other hand, the individual privacy loss is formulated based on \emph{differential privacy}, {\color{blue}as stated in Definition~\ref{defn:indi-privacy-loss} \cite{}.}
%In particular, a mechanism $\mathcal{M}$ is differential privacy if the probability of a specific output $O$ on any neighboring database is almost the same, i.e., the output $O$ is hard to distinguish.
%As a result, the individual privacy loss can be formulated .


\begin{figure}[t]
	\centering
	\includegraphics[width=0.47\textwidth]{pdata.eps}
	\caption{The framework of pricing private data \cite{li2014theory,li2017theory}}%from Pricing Approaches for Data Markets
	\label{fig:PData}
	\vspace*{0.05in}
\end{figure}


\begin{definition}\label{defn:indi-privacy-loss}
{\bf (Individual privacy loss)}.
The privacy loss of the data owner $i$ in the randomized mechanism $\mathcal{M}$ over the database $\mathbf{x}$ is defined as:
\begin{equation}
\epsilon_{i}(\mathcal{M})=\sup _{\mathbf{x}, O}\left|\log \frac{\Pr(\mathcal{M}(\mathbf{x})=O)}{\Pr\left(\mathcal{M}\left(\mathbf{x}^{(i)}\right)=O\right)}\right|
\end{equation}
\noindent
where $\mathbf{x}$ is the data vector, $\mathbf{x}^{(i)}$ simulates the absence of data owner $i$, and $O$ ranges over all possible outputs.
\end{definition}

In particular, the privacy loss measures the influence of data from owner $i$ on the output (denoted by a random variable $\mathcal{M}(\mathbf{x})$).
Furthermore, the upper bound of the privacy loss on data owner $i$ is found, as follows.
$$\epsilon_{i}(S) \leq \frac{\sup _{\mathbf{x}, i}\left|\mathbf{q}(\mathbf{x})-\mathbf{q}\left(\mathbf{x}^{(i)}\right)\right|}{\sqrt{v / 2}}$$

Thus, a payment for data owner $i$, i.e., the privacy compensation, is derived, as follows.
$$\mu_{i}(S)=c_i\cdot\epsilon_{i}(S),\quad c_i \text{ is a constant},c_i>0$$
Given the payment for data owners, the whole price of $S$ is formulated in the following.
\begin{equation}
\label{eq:pdataprice}
    \pi(\mathbf{q}, v)=\pi(S)=\sum_{i} \mu_{i}(S)
\end{equation}
%$$$$


In order to ensure the arbitrage freeness,
the price functions $\pi(\mathbf{q}, v)$ following these properties are proved to be arbitrage-free~\cite{li2014theory,li2017theory}.

\begin{proposition}
\label{prop:arb-privacy}
Any arbitrage-free price function $\pi(\mathbf{q}, v)$ satisfies the following properties,  where $\mathbf{q}$ refers to data analysis method that produces output, and $v$ is the noise level.

\noindent
$(i)$ The zero $\mathbf{q}$ is free: $\pi(\mathbf{q}, v)=0$.

\noindent$(ii)$ Higher variance is cheaper: $v \leq v^{\prime}$ implies $\pi(\mathbf{q}, v) \geq \pi(\mathbf{q}, v^{\prime}) $.

\noindent$(iii)$ The zero-variance $\mathbf{q}$ is the most expensive: $\pi(\mathbf{q}, 0) \geq \pi(\mathbf{q}, v) \text { for all } v \geq 0$

\noindent$(iv)$ Infinite noise is free: if $\pi$ is continuous at $\mathbf{q}=0,$ then $\pi(\mathbf{q}, \infty)=0$.

\noindent$(v)$ As $v \rightarrow \infty, \pi(\mathbf{q}, v) = \Omega(1 / v)$.
\end{proposition}

%{\color{blue}
%Since the payment function is arbitrage-free, the whole pricing function is a linear combination based on $ \mu_{i}(S)$ and is arbitrage-free.
%}


%\begin{enumerate}
%  \item The zero $\mathbf{q}$ is free: $\pi(\mathbf{q}, v)=0$
%  \item Higher variance is cheaper: $v \leq v^{\prime}$ implies $\pi(\mathbf{q}, v) \geq \pi(\mathbf{q}, v^{\prime}) $
%  \item The zero-variance $\mathbf{q}$ is the most expensive: $\pi(\mathbf{q}, 0) \geq \pi(\mathbf{q}, v) \text { for all } v \geq 0$
%  \item Infinite noise is free: if $\pi$ is continuous at $\mathbf{q}=0,$ then $\pi(\mathbf{q}, \infty)=0$.
%  \item As $v \rightarrow \infty, \pi(\mathbf{q}, v)=\Omega(1 / v)$.
%\end{enumerate}
This proposition is different from  Proposition~\ref{pro:free-qpricing}, as it considers the variable noise $v$.
The last property ensures that, the price function is arbitrage-free only if it decreases lower than 1/$v$ .
In such case, data consumers cannot purchase $(\mathbf{q}, v)$ with lower price by combining a series of $(\mathbf{q}, v_{i})$ when $\frac{1}{m} \sum_{i=1}^{m} v_{i} \leq v$, and thus arbitrage is avoided.
It is easy to find that, the price function $\pi(\mathbf{q}, v)$ in Eq.~\ref{eq:pdataprice} is arbitrage-free.
%the opportunity of arbitrage is avoided

%On the other hand, the individual privacy loss is formulated based on \emph{differential privacy}, {\color{blue}as stated in Definition~\ref{defn:indi-privacy-loss} \cite{}.}
%In particular, a mechanism $\mathcal{M}$ is differential privacy if the probability of a specific output $O$ on any neighboring database is almost the same, i.e., the output $O$ is hard to distinguish.
%As a result, the individual privacy loss can be formulated .

%{\color{blue}
%\begin{definition}\label{defn:indi-privacy-loss}
%{\bf (Individual privacy loss)}.
%The privacy loss of the data owner $i$ in the randomized mechanism $\mathcal{M}$ over the database $\mathbf{x}$ is defined as:
%\begin{equation}
%\epsilon_{i}(\mathcal{M})=\sup _{\mathbf{x}, O}\left|\log \frac{\Pr(\mathcal{M}(\mathbf{x})=O)}{\Pr\left(\mathcal{M}\left(\mathbf{x}^{(i)}\right)=O\right)}\right|
%\end{equation}
%\noindent
%where $\mathbf{x}$ ranges over all possible database instances, and $O$ ranges over all possible outputs.
%\end{definition}}

\begin{comment}
What is the mechanism M. What is the relation between M and the overall pricing framework.
How the privacy loss of the data owner is applied to the pricing framework.
What is the definition of neighboring databases?
what is \mathbf{x}^{(i)}, \mathcal{M}(\mathbf{x})...
It is better to also describe the general meaning of this equation in words with several sentences.

\end{comment}

%One can observe that, it is the deformation of differential privacy, which considers the neighboring databases by varying the data from owner $i$.


%{\color{blue}The above studies determine the basic framework of personal data pricing, laying the foundation for follow-up work.
%However, the specific form of the price function and the feasible privacy compensation strategy have not been certain, leading it not practical.}

%Thus, the structural granularity on pricing can be seen as the tuple, since the privacy loss of each tuple is considered.

%To make personal data trade more feasible, several critical problems have to take into consideration.
%On one hand, one problem is how to quantify the monetary compensation, in order to incentivize data owners/providers to contribute their private data.
%Another problem is the price of personal data concerning the privacy loss of data owners or providers.
%\begin{property}\label{prop:arbitrage-free-pdata}
%{111}
%\end{property}
%
%Following \cite{li2014theory,li2017theory}, Niu et al. then introduce the privacy compensation function, and the arbitrage-free pricing function, which leads personal data pricing more practical via a framework called \emph{ERATO}


%Following \cite{li2014theory,li2017theory}, a more practical framework \textsc{Erato} is proposed~\cite{niu2018unlocking,niu2019erato}.

It is worthwhile to note that, there are several differences between a practical framework \textsc{Erato} \cite{niu2018unlocking,niu2019erato} and previous studies \cite{li2014theory,li2017theory}.
First, the $\epsilon$-dependent differential privacy is guaranteed in \textsc{Erato}, which results in the different forms of the upper bound on privacy loss and price function.
Second, there is another payment function in \textsc{Erato} for data owner $i$, i.e., $\mu_{i}(S)=b_{i} \cdot \tanh \left(c_{i}\cdot  \epsilon_{i}(S)\right)$, for constants  $b_i$, $c_i>0$, which bounds the payments of data owners. Third, a top-down design is considered in \textsc{Erato}, where the payment budget $B$ for data owners is allocated to each owner based on the $\epsilon_{i}(S)$.
Last but not least, the evaluation results show that, \textsc{Erato}
improves the utility of aggregate statistics, guarantees arbitrage freeness, and compensates data owners in a fairer way than the classical differential privacy based approaches~\cite{li2014theory,li2017theory}.
%achieve more utility and privacy than dependent differential privacy and differential privacy, and is able to fairly distribute the privacy compensation among owners that differential privacy~\cite{li2014theory,li2017theory}.


%including the specific privacy compensation function, and the arbitrage-free pricing function.
%Specifically, \emph{Laplace} mechanism is employed to guarantee $\epsilon$-dependent differential privacy.
%Meanwhile, arbitrage-free pricing functions are designed according to Proposition \ref{prop:arb-privacy}, where the noisy answer of $\mathbf{q}$ is regarded as random variables with expectation $\mathbf{w}^{T} \mathbf{x}$, and the determinacy relation is given.
%As for privacy compensation, the bound of the privacy loss of each data owner $i$ is found, and privacy compensation functions are presented based on the bound.
%In particular, the compensation can also been allocated when a total compensation is $B$, which is called a top-down design.
%Numerous experiments have been conducted to demonstrate the feasibility of \textsc{Erato}.



%Following \cite{li2014theory,li2017theory}, a more practical framework \textsc{Erato} is proposed~\cite{niu2018unlocking,niu2019erato}, including the specific privacy compensation function, and the arbitrage-free pricing function.
%Specifically, \emph{Laplace} mechanism is employed to guarantee $\epsilon$-dependent differential privacy.
%Meanwhile, arbitrage-free pricing functions are designed according to Proposition \ref{prop:arb-privacy}, where the noisy answer of $\mathbf{q}$ is regarded as random variables with expectation $\mathbf{w}^{T} \mathbf{x}$, and the determinacy relation is given.
%As for privacy compensation, the bound of the privacy loss of each data owner $i$ is found, and privacy compensation functions are presented based on the bound.
%In particular, the compensation can also been allocated when a total compensation is $B$, which is called a top-down design.
%Numerous experiments have been conducted to demonstrate the feasibility of \textsc{Erato}.



%as an example, it aims to trade time-series data.
%evaluates the max-influence of the state $X_t$ on a set of ¡°remote¡± states $X_M$
Furthermore, there is a pricing framework  \textsc{Horae} for time-series private data~\cite{niu2019making}.
%which makes pricing time-series private data possible~\cite{niu2019making}.
First, \textsc{Horae} employs \emph{Pufferfish} privacy to quantify privacy losses under temporal correlations.
%which is a general form of differential privacy.
In particular, the Pufferfish privacy can capture the correlations in different timestamps, and thus it is suitable for time-series data.
\textsc{Horae} compensates data owners with distinct privacy strategies in a satisfying way.
%Specifically, the privacy loss is identified and the upper bound is computed through a Markov Quilt mechanism.
%Specifically, \textsc{Horae} designs a mechanism $\mathcal{M}$ to achieve Pufferfish privacy, i.e., adding noise, and computes the upper bound of the privacy loss for each data owner.
%Based on the upper bound,
%of privacy loss,
%\textsc{Horae} provides several valid privacy compensation functions, and prices the request $\mathbf{q}$ corresponding to privacy compensation.
Besides, the theoretical analysis and experiments confirm that, \textsc{Horae} not only guarantees good profitability at the data broker, but also ensures arbitrage freeness against cunning data consumers.
%The experiments on real dataset prove that, \textsc{Horae} is feasible to price time-series personal data, which not only has the ability to avoid arbitrage attacks, but also can control the profit radio.

\label{subsec:fb-analysis}
\begin{table*}[tbp]
%\footnotesize
  \setlength{\tabcolsep}{2.5pt}
  \centering
  \caption{Comparison of Feature-based Data Pricing Models}
 % |p{3em}<{\centering}|p{7.5em}<{\centering}|p{9em}<{\centering}|p{7em}<{\centering}|p{10.5em}<{\centering}|p{3em}<{\centering}|p{1.8em}<{\centering}|p{3em}<{\centering}|
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \textbf{Model} & \textbf{Reference} & \textbf{Perspective} & \textbf{Mechanism} & \textbf{Presetting} & \textbf{Technique}  & \textbf{Arbitrage-free} & \textbf{Market} \\
    \hline
     F1 & \cite{tang2014get,tang2013you,yu2017data}      & data quality &\makecell[c]{posted pricing} &basic price  & \makecell[c]{sampling, \\bi-level programming}  & uncertain   & $\checkmark$ \\
    \hline
     F2 &\cite{li2014theory,li2017theory,niu2019making,niu2018unlocking,niu2019erato} &  data privacy & posted pricing & N/A  & differential privacy & $\checkmark$    & $\times$ \\
    \hline
     F3 &\cite{niu2020online}     & market value & online pricing & feature & L$\ddot{\text{o}}$wner-John ellipsoid & uncertain   & $\checkmark$ \\
    \hline
%     F4 &\cite{tang2014get}     &  Data completeness & Basic price & Sampling & IP& $\times$   & $\times$ \\
%    \hline
%     F5 &\cite{yu2017data}     &  Data quality & Basic price  & Bi-level programming& PP & $\bigcirc$   & $\checkmark$  \\
%    \hline
    F4 &\cite{Zhu2020snpricing}     & node influence & posted pricing   &N/A & sampling & uncertain   & $\times$  \\
    \hline

    \end{tabular}%
    \label{tab:pricing-fbmodels}
\vspace*{0.06in}
\end{table*}

\subsection{Personal Data Pricing with Market Value}
\label{subsubsec:db-pmarket}


In addition to the pricing model concerning data privacy, there is another pricing model based on the market value of data (w.r.t. F3), which prices data in an online fashion.
The goal of this model  F3 is to minimize the regret during the ongoing transaction for maximizing the revenue, where the market value is modeled as a feature-based function.
Hence, the pricing model F3 is suitable to adjust the price based on the market feedback, so as to obtain the long-term gains.


Inspired by existing feature based pricing work \cite{cohen2020feature}, the market value of differentiated product can be formulated as a function, as stated in Definition~\ref{defn:market-value-goods}.

\begin{definition}\label{defn:market-value-goods}
{\bf (Market value of the product)}.
The market value \textcolor[rgb]{0.00,0.00,1.00}{$v_t$ of a product $t$} in the feature based pricing setting is defined as
\begin{equation}
v_t = f\left(\mathbf{x}_{t}\right)+\delta_{t}
\end{equation}
\noindent
where $\mathbf{x}_{t}$ is the feature vector of product, $f\left(\mathbf{x}_{t}\right)$ is the mapping function from feature vector $\mathbf{x}_{t}$ to the deterministic part in market value, and $\delta_{t}$ models the uncertainty in market value.
\end{definition}

The price of each product mainly relies on its features, and the uncertainty in markets is also considered.
Note that, the deterministic part $f\left(\mathbf{x}_{t}\right)$ is an arbitrary function, and can support different kinds of functions in both linear and non-linear forms.
When the price $p_t$ is lower or equal to the market value $v_t$, the consumer decides to buy the product, otherwise the transaction fails, resulting in zero profit.
To achieve more profit, the optimal price $p_{t}^{*}$ is the market value $v_t$.
%Hence, the structural granularity in this model can be varied in different levels of data, which depends on the level of features.

Since the knowledge of market value is limited, the data broker cannot directly determine the market value $v_t$.
Instead, he/she can only passively receive each product request $\mathbf{q}_t$, and then post a price $p_t$.
When the posted price is no more than the market value, i.e., $p_{t} \leq v_{t}$, the data broker can earn a revenue.
Thus, a revenue maximization problem is identified. This problem is solved via transforming it to a regret minimization problem \cite{cohen2020feature}.
%To solve it, \textcolor[rgb]{0.00,0.00,1.00}{\cite{cohen2020feature}} transforms such problem to a regret minimization problem.
In particular, it approximates the polytope-shaped knowledge set with ellipsoid to provide a worst-case regret of {\color{blue}$O\left(n^{2} \log T\right)$, where $n$ is the dimension of the feature $\mathbf{x}_{t}$, and $T$ is the number of rounds that the price $p_t$ is posted. Specifically, this} is essentially the pure version of pricing mechanism in \cite{niu2020online}.


Moreover, the personal data pricing model with market value in \cite{niu2020online}  models \textcolor[rgb]{0.00,0.00,1.00}{$\mathbf{x}_{t}$} as the privacy features of a request $\mathbf{q}_t$ with the reserve price constraint.
The differentiated product can be seen as the request \textcolor[rgb]{0.00,0.00,1.00}{$\mathbf{q}_t$} of data consumer, i.e., the concrete statistic and tolerable level of noise.
In this setting, the features can be obtained by the privacy compensation and other techniques.
The analysis and experiments demonstrate the usefulness to set a proper reserve price, and the feasibility of this online pricing mechanism.
%\textcolor[rgb]{0.00,0.00,1.00}{And the proper reserve price is proved to be helpful for decreasing regret.}
%Extensive experiments demonstrate that, it is feasible to apply existing online pricing \textcolor[rgb]{0.00,0.00,1.00}{methods} to personal data pricing.






\subsection{Pricing Social Network with Influence}
\label{subsec:fb-influence}


The rapid development of online social network applications makes social network attract  much attention, and thus generates the huge amount of economic value.

The online advertising becomes an essential way to promote the product via the word of mouth \textcolor[rgb]{0.00,0.00,1.00}{effects~\cite{eMarketer2017}.}
For example, the expenditure of advertisement on social media will be over \$50 billion by 2020, according to Fortune's claim~\cite{Reuters2016}.
The information can be propagated widely and rapidly through social networks, influencing users' decisions and behaviours in the diffusion process.

%In online social advertising, the online advertisers are often paid, so as to  a product via the word of mouth effects~\cite{eMarketer2017}.
%In this case, the online celebrities are often given free products, which results in the emergence of traditional influence maximization problem, or paid with a price, which is the main content in \cite{Zhu2020snpricing}.

The model of pricing social network with influence (i.e., F4) is born in the context of viral marketing and online advertising.
It aims to derive the prices for a set of nodes (i.e., online celebrities/users) in social network  based on the expected \textcolor[rgb]{0.00,0.00,1.00}{influence \cite{Zhu2020snpricing}}.
It not only presents a solution for online advertising, but also first involves the data pricing in social network, considering the information of network structure.

Specifically, the advertisers select a seed set $S$ from a node set $C$ and pay them in order to market the product and obtain more profit, where $C$ is provided by the online social network providers, corresponding to the online users that have ability or willingness to promote a product.
Intuitively, the price of any set of users should effectively reflect the expected influence spread that these users can generate in the information diffusion process.

Therefore, the divergence between the price and the influence spread can be characterized by $(c \cdot \sigma(S)$ $-$ $\sum_{s_{i} \in S} p_{i})^{2}$, where $c$ is a constant representing the expected revenue to derive from influencing a node.
$\sigma(S)$ is the influence spread of a node set $S$, which  is proportional to the probability that $S$ intersects with a random reverse reachable set \cite{borgs2014maximizing}. $p_i$ is the price of the node $s_i$. What's more, since the advertisers can choose any subset of nodes in $C$, the minimization problem of expected divergence between the price and influence spread can be formulated as follows.
$$
\min \quad \frac{1}{2^{n_{c}}} \sum_{S \subseteq C}\left(c \cdot \sigma(S)-\sum_{s_{i} \in S} p_{i}\right)^{2}$$
This problem is proved to be \#P-hard. There is an advanced algorithm to estimate the price profile with accuracy guarantees, which employs sampling technique to achieve a $(\varepsilon, \delta)$-approximation.

As a result, this pricing model finally aims to price nodes in a social network  (which is a special kind of data) via minimizing  the divergence between prices and influence of nodes.
\textcolor[rgb]{0.00,0.00,1.00}{It is the first data pricing model in social networks, and is suitable for} viral marketing and online advertising.
%provides price based on the influence of \textcolor[rgb]{0.00,0.00,1.00}{nodes}, i.e., the influence spread of node set.

\subsection{Analysis on Feature-based Data Pricing Models}
%
In this part, we compare the four representative feature-based data pricing models, as summarized in Table~\ref{tab:pricing-fbmodels}.
%as shown
%\textcolor[rgb]{0.00,0.00,1.00}{
%\textbf{Catagory(Cat.).} As we mentioned before, we divide the pricing models into three categories, i.e., query pricing (QP), personal data pricing (PDP), quality-based data pricing (QDP).}

\textbf{Pricing perspective.}
The data quality based pricing model F1 trades low quality data with a lower price.
The pricing model using data privacy F2 derives the price based on the privacy loss of data owners.
The pricing model with market value F3 decides the price in an online fashion, making the price closer to data's true market value.
The pricing model for social network F4 assigns the price to a node  based on its influence.
%To some extent, the name of pricing model can reflect its pricing perspective, as we mentioned before.
%For instance, personal data pricing using privacy trades data based on the privacy feature.

%For other query pricing models, the pricing perspective is contained in its name, such as query pricing with information value and query cost, as we mentioned before.


\textbf{Pricing mechanism.}
{\color{blue}The pricing models F1, F2, and F4 employ posted pricing mechanism, where the prices are posted by buyers (two models \cite{tang2014get,tang2013you} in F1) or sellers (F2 and F4).}
While the pricing model F3 gradually obtains the optimal price in an online fashion, and thus it belongs to the online pricing mechanism.
%For data quality based pricing model F1, there are two different mechanisms.
%One is the idea of ``what you pay for is what you get'', i.e., the price is proposed by data buyers, and the returned data rely on the proposed price.
%Another is the post pricing, which provides the different prices for different versions of data.
%As data pricing based on data accuracy/completeness first receives the price provided by data buyers and then offers data based on the price, we mark it as inverse pricing (IP).
%Personal data pricing using privacy and data pricing based on multi-dimension quality belong to the post pricing (PP) mechanism, since they directly price data according to data feature.
%Thus, the quality based pricing involves both post pricing (PP) and inverse pricing (OP).
%For pricing personal data using market value, it derives the price in an online fashion, thus is an online pricing (OP) mechanism.
%For pricing social network, it belongs to traditional post pricing mechanism.

\textbf{Presetting.}
For the pricing model F1, there is a requirement for a predetermined price as the basic price of original data.
The pricing model F3 requires data features in \textcolor[rgb]{0.00,0.00,1.00}{request} before pricing, and the features should be carefully selected.
The other two pricing models, i.e., F2 and F4, generate the data prices in different ways, which do not need to preset some parameters.
%For example, F3 can obtain the optimal price in an online way, i.e., the price is continuously optimized, in order to obtain higher benefits.

\textbf{Techniques of price computation.}
The sampling technique is employed in F1, in order to derive a ``worse'' version of data, while the bi-level programming is used to tackle the revenue maximization problem in F1.
The differential privacy is used to \textcolor[rgb]{0.00,0.00,1.00}{not only} protect the privacy of private data, \textcolor[rgb]{0.00,0.00,1.00}{but also} quantify the privacy loss of data owners in F2.
As for the pricing model with market value F3, the L$\ddot{\text{o}}$wner-John ellipsoid method is helpful to support the price optimizing process.
Meanwhile, F4 utilizes the sampling technique  to boost the computation efficiency of nodes' influence spread.

\textbf{Arbitrage-free property.}
First, the pricing model with data privacy F2 and one pricing solution (i.e., data pricing based on completeness \cite{tang2014get}) in F1 consider the arbitrage freeness in the pricing framework.
In contrast, the other pricing models in F1, F3 and F4  do not take this property into consideration.
In other words, there is an opportunity for consumers to buy more information with a lower price.
For the online pricing model F3, it pays more attention on the market revenue, compared to the arbitrage issue.
The arbitrage-free property needs to be further explored in various real-life scenarios.

\textbf{Market-oriented.}
The data quality based pricing model F1 is market-oriented, since the willingness of buyers for versions of data is considered, and a revenue maximization problem is solved.
Meanwhile, the pricing model with market value F3 is obviously  market-oriented, since the optimal price is the market value.
The other two pricing models F2 and F4 are not market-oriented, since no market factor is considered in them.


%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Requirement.}}
%For data pricing based \textcolor[rgb]{0.00,0.00,1.00}{on quality, it needs the basic price of ``better'' data (high accuracy/completeness/qulity), in order to derive the prices for data of different quality levels.
%The pricing model using privacy requires nothing for preparation of pricing, since it automatically derives price based on privacy.
%As for pricing with market value, it requires \textcolor[rgb]{0.00,0.00,1.00}{human} to determine the feature of market value.
%Meanwhile, there is no requirement for pricing social network with influence, since it obtains the price based on the influence of nodes in the socials network}.


%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Techniques.}}
%\textcolor[rgb]{0.00,0.00,1.00}{For data pricing based on quality (i.e., accuracy and completeness) and pricing social network with influence, they both leverage the sampling technique.
%However, the former uses sampling to derive ``worse'' data, and sampling is employed to boost efficiency in pricing social network.
%And a bi-level programming technique is used to solve the revenue maximization problem in pricing based on multi-dimension quality \cite{yu2017data}.}
%In personal data pricing using \textcolor[rgb]{0.00,0.00,1.00}{privacy,} the differential privacy is employed to measure privacy loss, while personal data pricing with market value learns real market value through L$\ddot{\text{o}}$wner-John ellipsoid method.

%For data pricing based on data accuracy and completeness, they both use sampling technique to derive ``worse'' data.
%And a bi-level programming technique is used to solve the revenue maximization problem in pricing based on data quality, while sampling technique is leveraged in pricing social network with influence.





%\textbf{Arbitrage.} There is no arbitrage in personal data pricing using privacy and data pricing based on data completeness.
%However, other feature-based pricing methods do not consider the arbitrage issue, \textcolor[rgb]{0.00,0.00,1.00}{and there are opportunities to lead arbitrage.
%Thus, the quality based pricing model is marked as $\bigcirc$ since there are pricing models that may result in arbitrage.}
%
%
%
%\textbf{Market.} Only personal data pricing with market value and data pricing based on multi-dimension quality consider market factors, such as buyers' valuation and revenue, while other pricing models are not marker-oriented, since they derive price of data directly.
%\textcolor[rgb]{0.00,0.00,1.00}{We mark the quality based pricing model as market-oriented, as there is a model concerning it.}
%
%Overall, the feature-based pricing models consider the important \textcolor[rgb]{0.00,0.00,1.00}{features} of different data, and derive prices in different ways.
%However, some issues about data pricing should \textcolor[rgb]{0.00,0.00,1.00}{be further studied}, such as arbitrage and market factors.




==> gt-model.tex <==


\subsection{Game Theory based Pricing Model}
\label{subsec:gt-model}

Game theory is a fundamental discipline used primarily in economics. It models situations in which decision makers have to make specific actions that have mutual-possibly conflicting-consequences.
It precisely models the competitions and cooperations between different companies.
%in order to model competition between companies. Besides, game theory can also be applied to pricing problem.
%Game theory is a useful method used in the fields of pricing
%and markets, especially in pricing data commodities. In this paper, we
Game theory has been widely studied in the real economy. Data, as a special type of commodities, can be modeled by game theory.
However, there are some challenges when applying game theory to data pricing.
For instance, replicability of data is unique to other kind of products and this may lead to a more complex situation.

	

Game theory is related to the actions of decision makers who are conscious that their actions affect each other \cite{charilas2010survey}. A game consists of a principal and a finite set of \emph{players} $P = \{p_1, p_2, \cdots, p_n\}$, each of which selects a strategy $s_i \in S_i$ with the objective of maximizing his/her utility $u_i$.
The utility function $u_i(s): S \rightarrow R$ represents each player's sensitivity to everyone's actions. According to the above, a game can be modeled as
$G = (P, A, S_i, r_{ij})$ where


\begin{itemize}\setlength{\itemsep}{-\itemsep}
\item{} $P = \{p_1, p_2, \cdots, p_n\}$ denotes the set of players.
\item{} $A = \{a_1, a_2, \cdots, a_n\}$ denotes the available resources in the game.
\item{} $S_i$ denotes the set of strategies for player $i$, i.e., all possible choices from set $A$.
\item{} $r_{ij}$ denotes the payoff/revenue assigned to player $i$ after choosing resource $a_j$.
\end{itemize}

%In a cooperative game, the players cooperatively try to come to an agreement, and the players have a choice to bargain with each other so that they can gain maximum benefit, which is higher than what they could have obtained by playing the game without cooperation. The cooperative game is an attractive scheme to a complex negotiation condition, e.g., improving the performance of data auction process \cite{berz2016game}, network resource auction and sharing \cite{azimi2016cooperative}, setting the aircraft landing fees \cite{littlechild1977aircraft}, broadband networks \cite{yaiche2000game}, and energy efficiency management \cite{yang2015joint}.

%While in non-cooperative games, each player selects strategies without coordination with others. %{\color{blue}The strategy profile $s$ is the vector containing the strategies of all players: $s = (s_i), i \in N = (s_1, s_2, \cdots, s_N)$.} A large number of real-life applications utilize the non-cooperative game, such as pricing IoT sensing data \cite{luong2016data,yaiche2000game}, power coordination and SE optimization in HetNets \cite{al2011game,la2012performance,shen2013dynamic}, the problem of rate allocation and charging in communication networks \cite{low1999optimization,anastasi2005rate,kelly1997charging}. All of them consider the issue of maximizing the social benefit, which is the sum of the user utilities.




%In order to provide the composite services with a certain Quality of Service (QoS) to users, SOs need to collect the simple services from entities. SOs attracts entities to collect and submit $SS$ by issuing the purchase service price. The required numbers of $SS$ $v_e$ are certain in a small period. SOs can provide composite services with a certain QoS as long as simple services $v_e$ are collected. SOs expects to collect $v_e(i)$ simple services in the $i$th time slot, and in the time slot of $i$, SOs collect $v(i)$ simple services. Thus, the SO's goal is to make the difference $v_{\Delta}$ between $v_i$ and $v_e(i)$ is minimize, that is
%\begin{equation}
%\operatorname{Min}\left(v_{\Delta}\right)=\min \sum_{i \in %t}\left|v_{e}(i)-v(i)\right|
%\end{equation}

%And the total payment need to be paid by SOs are
%\begin{equation}
%\mathrm{M}=\sum_{i \in t}\left(v(i) \lambda_{i}\right)
%\end{equation}

%In the traditional game, the game matrix of each entity is the same. But this does not reflect the actual situation of the cyber-physical systems. In a real cyber physical systems, each entity does not adopt the same game matrix when play with another entity, but the best game matrix should make maximum profit.


%Game theory is a useful method used in the fields of pricing and markets, especially in pricing data commodities\cite{liang2018survey}. In this paper, we introduce two branches of game that are used to build pricing models: (i) Cooperative game (ii) Non-cooperative game. In some models, both conditions are considered.

%The cooperative game theory refers to a condition in which the vendors and consumers reach an agreement, and to achieve this agreement, the vendors and consumers need to negotiate. \cite{littlechild1977aircraft} uses cooperative game theory to set the aircraft landing fees. Since the cooperative game is a proper scheme to a complex negotiation condition, it is often used to improve the performance of the data auction process\cite{berz2016game}, network resource auction and sharing\cite{azimi2016cooperative}, and energy efficiency management\cite{yang2015joint}. \cite{yaiche2000game} consider the Nash bargaining framework for bandwidth allocation and pricing in broadband networks. As for the non-cooperative game, \cite{luong2016data} and \cite{yaiche2000game} designed a pricing model to evaluate IoT sensing data. Besides available works on game theory-based power coordination and SE optimization in HetNets usually adopt a non-cooperation game-theoretic approach including \cite{al2011game,la2012performance,shen2013dynamic}. More recently, \cite{low1999optimization}, \cite{anastasi2005rate} and  \cite{kelly1997charging} have considered the problem of rate allocation and charging based on knowledge of user utility functions. All consider the issue of maximizing the social benefit, which is the sum of the user utilities.

%In the next section we will introduce some game theory based models.

%Game theory is a discipline aiming to model situations in which decision makers have to make specific actions that have mutual-possibly conflicting-consequences. It has been used primarily in economics, in order to model competition between companies. Besides, game theory can also be applied to pricing problem.

%\subsubsection{Game theory basics}
%Game theory is related to the actions of decision makers who are conscious that their actions affect each other. Let us begin with a standard representation of a game, which is known as a normal form game, or a game in strategic form\cite{jackson2011brief}:\\
%\begin{itemize}\setlength{\itemsep}{-\itemsep}
%\item{} The set of players is $N = {1, . . . , n}$.
%\item{} Player $i$ has a set of actions, $a_i$, available. These are generally referred to as pure strategies. This set might be finite or infinite.
%\item{} {\color{blue} Let $a = a_1 \times ???\times a_n$ be the set of all profiles of pure strategies or actions, with a generic element denoted by $a = (a_1, . . . , a_n)$.}
%\item{} {\color{blue}  Player $i$'s payoff as a function of the vector of actions taken is described by a function $u_i: A \rightarrow \mathcal{R}$, where $u_i(a)$ is i's payoff if the $a$ is the profile of actions chosen in the society.}
%\end{itemize}

%Normal form games are often represented by a table. There are many games that might have different descriptions motivating them but have a similar normal form in terms of the strategic aspects of the game. One famous game is the prisoners' dilemma, which is represented in Figure~\ref{fig:prison}. In this game there are two players who each have two pure strategies, where $a_i = {C, D}$, and $C$ {\color{blue} stands for 'cooperate' and $D$ stands for 'defect'.} The first entry indicates the payoff to the row player (or player 1) as a function of the pair of actions, while the second entry is the payoff to the column player .

%The payoffs in the matrix represent time lost in terms of years in prison. The term cooperate refers to cooperating with the other player. The term defect refers to confessing and agreeing to testify, and so breaking the (implicit) agreement with the other player.

%\begin{figure*}[h]
%		\centering
%		\includegraphics[width=0.5\textwidth]{prison.eps}
%		\caption{ {\color{blue} A prisoners' dilemma game}
%}\label{fig:prison}
%\end{figure*}



%Two types of games are distinguished: in non-cooperative games, each player selects strategies without coordination with others. On the other hand, in a cooperative game, the players cooperatively try to come to an agreement, and the players have a choice to bargain with each other so that they can gain maximum benefit, which is higher than what they could have obtained by playing the game without cooperation.


In what follows, we will discuss how game theoretic frameworks address some important issues in data pricing.
There are three major branches of game theory based pricing models using \emph{cooperative game}, \emph{non-cooperative game}, and \emph{mixed game strategy}, respectively.

\subsubsection{Pricing using Cooperative Game}

In game theory, a cooperative game (a.k.a. \emph{coalitional game}) is a game with competition between groups of players due to the possibility of external enforcement of cooperative behavior (e.g., through contract law).
The players cooperatively try to come to an agreement, and have a choice to bargain with each other so that they can gain maximum benefit, which is higher than what they could have obtained by playing the game without cooperation.
Those are opposed to non-cooperative games in which there is either no possibility to forge alliances or all agreements need to be self-enforcing (e.g., through credible threats).

%Cooperative games are often analyzed through the framework of cooperative game theory, which focuses on predicting which coalitions will form, the joint actions that groups take and the resulting collective payoffs.



%\noindent{\bf (1) Game Based Services Priing (GSP) Model}.

%In cyber-physical systems (CPS), there exist complex interactions among the CPS Organizers, entities and users. Maximizing profit is the primary concern for CPS Organizers, which might be achieved by having high price level for users and low investment on the infrastructure. On one hand, users wish to maximize their utility by consuming high QoS with low service price.

%\cite{liu2015service} is mainly concerned about price competition between CPS Organizers and entities as well as internal entities. In the CPS, there are price competition relationships between CPS Organizers and entities. Each CPS Organizer makes an investment in the collection and organizing services, CPS Organizers want to receive more service at lower price to improve the quality of combined service for the user (or customer) to maximize its profit. And a game-based services pricing (GSP) model is proposed to depict price competition phenomenon of the CPS on the principles of game theory in economics.



%\subsubsection{Cooperative game}

%In game theory, a cooperative game (or coalitional game) is a game with competition between groups of players due to the possibility of external enforcement of cooperative behavior (e.g. through contract law). Those are opposed to non-cooperative games in which there is either no possibility to forge alliances or all agreements need to be self-enforcing (e.g. through credible threats).

The framework of cooperative game theory focuses on predicting which coalitions will form, the joint actions that groups take and the resulting collective payoffs.
Cooperative game theory has been proven to be an essential tool in capturing the complex and strategic interactions among market participants and for strategic analysis of situations involving multiple
independent players.
For example, a game theory-based loss reduction allocation in energy management for smart grids is studied in \cite{wang2015game}.
The cooperative game is an attractive scheme to the complex negotiation condition, e.g., improving the performance of data auction process \cite{berz2016game}, network resource auction and sharing \cite{azimi2016cooperative}, setting the aircraft landing fees \cite{littlechild1977aircraft}, broadband networks \cite{yaiche2000game}, and energy efficiency management \cite{yang2015joint}.
% and some examples of data pricing using game theory.

\begin{example}{\bf  Game based services pricing (GSP) model}.
In cyber-physical systems (CPS), service organizers (SOs) aim to collect service from service entities at lower price and provide better combined services to users.
For instance, the travel agency works as a service organizer and collect service (e.g., transportation, accommodation) from service entities like hotels.
When you take a vacation, you act as the user and require the service provided by the travel agency.
In order to collect those simple services, SOs publish some service gathering tasks to entities. Then an entity could collect and submit services to SOs and obtain given payoffs. In a cooperative game, entities give certain payment to others and get service from others.
For example, after two entities $e_1$ and $e_2$ receive the service gathering task from the SOs, they sense the surrounding environment and get some their services respectively.
If $e_1$ and $e_2$ gave services to each other in their game, a cooperative game is formed in this way.
In this situation, $e_1$ and $e_2$ not only have its own services, but also receive each other's services. Thus they can report more services to their own SOs and obtain more payoffs.
%However, each entity receives payoffs when providing services, which leads to competition between SOs and service entities or within internal service entities.
%The interaction between the entities can be regarded as a game. {\color{blue}If the two entities cooperate with each other in an interaction, it can be seen as a cooperative game. In a cooperative game, entities give certain payment to others and get service from others.}
%Maximizing profit is the primary concern for SO(service organizers)s, which might be achieved by having high price level for users and low investment on the infrastructure. Each SO makes an investment in the collection and organizing services, SOs want to receive more service at lower price to improve the quality of combined service for the user (or customer) to maximize its profit.
%{\color{blue} And interaction between the two entities can be regarded as a game.} %If the two entities cooperate with each other in an interaction, it can be seen as a cooperative game. In a cooperative game, entities give certain payment to others and get service from others. However, entities don¡¯t always cooperate with others in a cooperator-defector pair. So, the game between the entities is very complicated and has a great deal of uncertainty in the CPS model.

The price competition between entities has been studied recently  {\color{blue}\cite{jiang2014optimal,rose2014pricing,zhang2014research}}. % aim  at the price competition pattern between service providers and service consumer.
A game based services pricing (GSP) model \cite{liu2015service} is proposed to depict price competition in service organizer versus CPS entities and entities versus entities.
In this model, each entity has its own payoff matrix, increasing the payoff can stimulate entities to game in order to get more payoffs. An entity $e$ can give the price $p_{e}$ to another entity which provides service, and the entity $e$ will obtain payoff $\lambda$ when reporting the services to SOs.  The entity $e$ also needs to pay the price $q_{e}$ when entity $e$ \emph{senses} service, thus server price $p_{e}$ of the entity $e$ should meet the following relations:
\begin{equation}
\lambda-p_{e}-q_{e} \geq p \quad|\quad p \geq 0
\end{equation}
Only under the condition of $p\ge0$ which represents the net profit,  the entity can obtain payoffs when it receives services.



%Entities will also reduce the number of game when reducing the payoffs of entities; this is consistent with the characteristics of the CPS. %The entity is glad to provide more services if the entity obtains more payment in the game. On the contrary, the entity will weaken its participation degree if the entity obtains negative payoffs in the process.

%In order to provide the composite services with a certainQuality of Service (QoS) to users, SOs need to collect the simple services from entities. SOs attracts entities to collect and submit $SS$ by issuing the purchase service price. The required numbers of $SS$ $v_e$ are certain in a small period. SOs can provide composite services with a certain QoS as long as simple services $v_e$ are collected. SOs expects to collect $v_e(i)$ simple services in the $i$th time slot, and in the time slot of $i$, SOs collect $v(i)$ simple services. Thus, the SO's goal is to make the difference $v_{\Delta}$ between $v_i$ and $v_e(i)$ is minimize, that is
%\begin{equation}
%\operatorname{Min}\left(v_{\Delta}\right)=\min \sum_{i \in %t}\left|v_{e}(i)-v(i)\right|
%\end{equation}

%And the total payment need to be paid by SOs are
%\begin{equation}
%\mathrm{M}=\sum_{i \in t}\left(v(i) \lambda_{i}\right)
%\end{equation}

%In the traditional game, the game matrix of each entity is the same. But this does not reflect the actual situation of the cyber-physical systems. In a real cyber physical systems, each entity does not adopt the same game matrix when play with another entity, but the best game matrix should make maximum profit.
%In the GSP model, each entity publishes their payoff matrix when playing game with others; Some payoffs can be obtained from the other entity if it reports services to the entity.



The game among entities is as follows. First, an entity $e$ determines its initial prices $q_e$ and $p_e$ on the determined price $\lambda$ according to above equation and adjusts the price based on earnings.
Moreover, the game among entities needs to adjust the parameters of several other aspects.
(i) The cooperative ratio which reflects how cooperative entities can be. For example, in the real world, the entity would be
glad to play game with the entity when an entity offers high payments and the cooperation ratio is also high in interaction.
For the entity with relatively low payments, the cooperation rate drops when playing game with others and the betrayal ratio rises.
(ii) The entity determines the game times according to the results of the last game. (iii) The entity is in evolution on the basis
of the probability. The entity with different strategies constantly adapts to the environment in the process of game.
So each entity updates its strategy with a certain probability in the game according to rules.

The GSP model can reach rapidly to a stable state under the condition of any given parameters for the system, and entities with difference strategies have different optimal prices, even the entities with same strategy have different optimal prices when the system reaches to a stable state.
The model precisely captures the game interaction between service providers and service consumers.
Through the model, one can predict in advance what price is optimal for SOs, the average payoff for each entity, each entity's game times, and the cooperation ratio for the system. As a result, this GSP model provides a good decision support for decision makers.
\end{example}


\subsubsection{Pricing using Non-Cooperative Game}

The non-cooperative game theory is usually employed to analyze the customers' behaviors in response to any changes of price.
In a non-cooperative game, every player adheres to a strategy that maximizes its own utility, without necessarily concerning about the social welfare and the coordination with others.
The term ``non-cooperative'' does not necessarily mean that there is no cooperation between players; it rather implies that there is no communications or binding agreements between them.
One example is the non-cooperative game theory employed in the spread spectrum technology in the physical layer \cite{al2008stackelberg}, which considers a revenue maximization version of the pricing problem.
Moreover, a large number of real-life applications utilize the non-cooperative game, such as pricing Internet of thing (IoT) sensing data \cite{luong2016data,yaiche2000game}, power coordination and optimization in heterogeneous networks \cite{al2011game,la2012performance,shen2013dynamic}, the problem of rate allocation and charging in communication networks {\color
{blue}\cite{kelly1997charging,kelly1998rate,low1999optimization}}.
All of them consider the issue of maximizing the social benefit, which is the sum of the user utilities.


\begin{example}{\bf Pricing in wide-band cognitive radio networks}.
Given the recent reports on scarcity of available frequency bands and inefficiency in spectrum utilization, the importance of cognitive radio paradigm has emerged for allocating valuable wireless resources. Unlike traditional wireless devices, cognitive radio nodes are aware of their capabilities, environment, and intended use, and can also learn new waveforms, models, or operational scenarios.
Such smart characteristics of cognitive nodes can also help implementing various operational features of telecommunication networks that have always suffered from lack of flexibility on the operator and user sides. In this context, pricing is one important topic that can be revived by the virtue of cognitive radio technology.

For a revenue maximization version of the pricing problem, it focuses on systems that apply spread spectrum technology in the physical layer \cite{al2008stackelberg}.
The problem involves a service provider that accommodates cognitive radio users transmitting on the uplink channels. The problem is formulated as a non-cooperative Stackelberg game.
Namely, the service provider (i.e., the leader) imposes differentiated prices per unit of transmitting power on the different users in the network. Consequently, the users (i.e., the followers) update their power levels to maximize their net utilities. In this game, the ``leader'' means that service provider made its decision before the ``followers'', i.e., users.

Consider a wide-band wireless network that has $N$ cognitive radio nodes numbered $1, \cdots, N$. The service provider charges the $i$-{th} user the amount $\lambda_i$ per unit of transmitting power on the uplink channel.
Namely, if the transmitting power of user $i$ is $p_i$, then the amount charged is $\lambda_ip_i$.
The total revenue, denoted by $R(\boldsymbol{\lambda}, \boldsymbol{p})$,  for the service provider is then given by Eq.~\ref{eq:non-cooperative-example}.
In particular, $\boldsymbol{\lambda} = \left(\lambda_{1}, \lambda_{2}, \cdots, \lambda_{N}\right)$ and $\boldsymbol{p} = \left(p_{1}, p_{2}, \cdots, p_{N}\right)$.
\begin{equation}\label{eq:non-cooperative-example}
R(\boldsymbol{\lambda}, \boldsymbol{p})=\sum_{i=1}^{N} \lambda_{i} p_{i}
\end{equation}
The problem involves a non-cooperative setup where each user in the network is interested in maximizing its net utility. In specific, for a given price $\lambda_i$, and a vector of power levels of all users except the $i$-{th} user, denoted by $p_{-i}$, the objective of user $i$  is to find $p_i^*$ that solves the following problem.
\begin{equation}\label{eq:objective-non-cooperative}
\max _{p_{i} \geq 0} U_{i}\left(p_{i}, p_{-i}, \lambda_{i}\right)
\end{equation}

Therefore, the problem of the service provider for maximizing revenue is characterized by Eq. \ref{eq:non-cooperative-example}. The service provider aims to impose optimal prices on the users given their selfish behavior as represented by Eq. \ref{eq:objective-non-cooperative}. The problem in this context can be considered from a game theoretical perspective and formulated as a Stackelberg game. In the leader-follower game, the service provider, i.e., the leader in this case, sets the prices, and consequently the users, or followers, update their power levels in accordance with their own preferences or utilities.

The game provides incentive compatibility for the users while maximizing revenue for the service provider. The pricing policy suggests charging the users proportional to their uplink channel conditions and willingness to pay for the provided service. It shows that participation of all the users in the game is subject to having a large enough spreading factor for the wideband network.
%With the developments of technologies in sensing, communication and storage, big data can be acquired with a higher velocity, volume and variety in this era \cite{zheng2017bridging}. Traditional data processing methods, such as standard statistics, are inadequate to cope with the problems in big data due to the complexity of the model, the heterogeneity of the data, and more importantly, the huge data and network size. An important trend of large-scale optimization approaches is to let a controller set up a hierarchy, divide the heavy computation caused by the large size into different small groups, and implement the calculations on different agents in a distributed manner \cite{hong2015unified}. In such approaches, each separated computational step is simple, the intermediate results are easy to store for agents, and the iterations of the division and aggregation are fast to converge.
%Therefore, faster and more scalable computational methods are needed to deal with modern big data networks. %As an efficient approach, large-scale optimization has attracted a great deal of attention since it can usually guarantee the fast convergence for the large data and network size.


%In order to help the controller promote agents to achieve controller's objective, one interesting  pricing framework \cite{zheng2017bridging} is designed as an incentive mechanism in a hierarchical network with one controller and a large number of agents. Consider a hierarchical network with one controller and $N$ agents, denoted by ${A_1, A_2,...,A_N}$. The network size can be large, when $N \sim \infty$. Each agent $A_i$ holds a certain resource denoted by $x_i$. Each agent $A_i$ has its own objective with resource $x_i$. It abstracts the objective for each agent as a general minimization problem, namely
%\begin{equation}
%\min _{x_{i}} u_{i}\left(x_{i}\right), \quad \forall 1 \leq i \leq N
%\end{equation}
%where $u_i(x_i)$ denotes the agent's objective function.

%The controller can also benefit with the agent's resource $x_i$. The objective is abstracted as a general minimization problem, which is given below.
%\begin{equation}
%\min _{\mathbf{x}} f(\mathbf{x})
%\end{equation}
%where $u(x)$ denotes the controller's objective function, and $\mathbf{x} = (x_1, x_2, ..., x_N )^{{}^T}$ is the resource vector.

%We denotes $\mathbf{x}^{*}=\left(x_{1}^{*}, x_{2}^{*}, \ldots, x_{N}^{*}\right)^{T}$ as the optimal point.

%Let each agent optimize an incentive function $\Phi_{i}\left(u_{i}\left(x_{i}\right), \theta_{i}\right)$ instead of $u_i(x_i)$. Through adjusting the parameter $\theta_i$. Hence, the incentive mechanism design problem can be formulated as a Stackelberg game below

%\begin{equation}
%\begin{array}{ll}{L G :} & {\boldsymbol{\theta}^{*}=\left(\theta_{1}^{*}, \theta_{2}^{*}, \ldots, \theta_{N}^{*}\right)^{T}=\underset{\theta_{1}, \theta_{2}, \ldots, \theta_{N}}{\operatorname{argmin}} \sum_{i=1}^{N} f_{i}\left(x_{i}\right)} \\ {F G :} & {x_{i}^{*}=\underset{x_{i}}{\operatorname{argmin}} \Phi_{i}\left(u_{i}\left(x_{i}\right), \theta_{i}\right), \quad \forall 1 \leq i \leq N}\end{array}
%\end{equation}
%where $LG$ represents the leader's game, $FG$ is the follower's game. The controller is defined as the leader and $\theta$ are the variables controlled by the leader, i.e., the leader's strategy. Each agent is defined as each follower, and $x_i$ is the variable controlled by the follower $P_i$, i.e., follower $P_i$'s strategy. For convenience, for the rest of this paper, the author uses the term 'leader to represent the controller, and the term 'follower' to represent each agent.

%The task is to properly design the incentive function $\Phi=\left(\Phi_{1}, \Phi_{2}, \ldots, \Phi_{N}\right)^{T}$ and incentive parameters $\theta=\left(\theta_{1}^{*}, \theta_{2}^{*}, \ldots, \theta_{N}^{*}\right)^{T}$ , to solve the Stackelberg game.

%The pricing framework on incentive functions $\Phi(\mathbf{u}(\mathbf{x}), \boldsymbol{\theta})$ and incentive {\color{blue}parameters $\theta$ gradually let the optimal} point of $\Phi_{i}\left(u_{i}\left(x_{i}\right), \theta_{i}\right)$ approximate the optimal point of each $f_i(x_i)$, step by step. {\color{blue}Finally, the linear convergence of the pricing framework is proved}.
\end{example}


%The paper focused on the incentive mechanism design in hierarchical networks and formulated the problem as a Stackelberg game and proposed a pricing framework to help the leader (controller) promote followers' (agents') to reach the optimal point for the leader's objective. The parameters $\theta$ can be physically interpreted as the price, which equals the marginal cost of followers' objective functions. The pricing framework is guaranteed to converge if all the objective functions are convex. Furthermore, the pricing framework converges linearly, when each part of the leader's objective is strongly convex and the followers' objective functions hold a uniform Lipschitz gradient. The convergence and linear convergence are regardless of the network size, which indicates that it can work properly in big data networks. Finally, the pricing framework is tested in wireless virtualized networks to verify its fast convergence.

%Future work could concentrate on the multi-controller situation, and decides whether agent's objectives have a uniform Lipschitz gradient and further more converge.
%\noindent {\bf (2) Online Marketing Pricing (OMP) Model}

%The advent of the Internet has made it easier for many manufacturers who traditionally distribute their products through retailers to engage in online sales. Why does a manufacturer add an online store to distribute directly his product rather than letting an independent retailer distribute it? To answer this question the following part develops a simple model consisting of a manufacturer distributing a product to a market of potential heterogeneous customers.

%The advent of the Internet has made it easier for many manufacturers who traditionally distribute their products through retailers to engage in online sales.

%\cite{fruchter2005dynamic} consider a manufacturer who distributes a product to a market of $N$ potential customers. The manufacturer may distribute the product to either or both of two shopping choices: a network of physical stores operated by an independent retailer and an online store operated directly by the manufacturer. To each individual customer, the choice is between the closest physical store and the online store, so from now on our discussion in the paper will be framed as if there is only one physical store. Such choices are broadly available to customers today. For example, a potential traveler may buy travel tickets through a travel agent or through the Internet-accessing directly to the company.

%Consider a Stackleberg differential game where the manufacturer is leader and the retailer is a follower. Let $V$ be the value of a homogenous product in real inspection, i.e., when it is bought through a retailer. When the product is bought online through virtual inspection, one can assume that it has a smaller value $\theta V$, where $0 \le \theta \le 1$, due to the lack of contact between the consumer and the product at its acquisition. The parameter $\theta$ thus represents the acceptance of the virtual inspection by the consumer. Then label this term as a consumer virtual acceptance. To express consumers' heterogeneity in the virtual acceptance the paper assumes that $\theta$ is a random variable with cumulative density function $D_{\theta}(\cdot)$. The determination of $D_{\theta}(\cdot)$ is an empirical question revealed by customer distribution observed along channels acquisition. However, in the sequel, $D_{\theta}(\cdot)$ is considered as an arbitrary general distribution function.

%The economic-added value provided to a consumer by the product can be measured by the concept of consumer surplus, which is equal in our model to the consumer value from the product, less its price. Therefore, if the product is sold through a retailer at a price $p_r$, then the resulting consumer surplus is $V -p_r$. If the product is sold online at the price $p_{on}$, then the resulting consumer surplus is $\theta V-p_{on}$.

%Assume a risk-neutral manufacturer and a strategic retailer. This implies a dynamic hierarchical game-theoretic problem. More exactly, the paper considers a Stackelberg differential game, with the manufacturer acting as the leader and the competitive retailer as the follower.

%Assuming that firms maximize the present value of their profit stream over an infinite horizon, the manufacturer maximizes $\Pi_m$ with respect to $p_{on}$ and $w$ which is the manufacturer supplies the retailer of the physical store at a wholesale price while the competitive retailer maximizes $\Pi_r$ with respect to $b$.


%Where
%\begin{equation}
%\Pi_{m}=\int_{0}^{\infty}\left[\left(p_{o n}-c_{o n}\right) %q+\left(w-c_{r}\right)(1-q)\right] N e^{-r t} d t
%\end{equation}\\
%where the manufacturer incurs a cost per unit $c_r$ that includes the cost of manufacturing and logistics, while using the online channel, a cost per unit $c_{on}$. And  consider that the retailer will use a markup b for pricing, i.e.,
%\begin{equation}
%p_r=(1+b)w
%\end{equation}

%The competitive retailer maximizes $\Pi_r$ with respect to $b$, where
%\begin{equation}
%\Pi_{r}=\int_{0}^{\infty}\left[\left(p_{r}-w\right)(1-q) N\right] %e^{-r t} d t
%\end{equation}\\
%where Let $q(t)$ be the probability that a customer will buy the product through an online site at time t.	

%Overall, the manufacturer and retailer's optimization problems can be summarized by the following differential game:

%\begin{equation}
%\left\{\begin{aligned} \operatorname{Max}_{p_{o n}, w} \Pi_{m} &=\int_{0}^{\infty}\left\{\left(p_{o n}-c_{o n}\right) q+\left(w-c_{r}\right)(1-q)\right\} N e^{-r t} d t \\ \operatorname{Max}_{b} \Pi_{r} &=\int_{0}^{\infty} b w(1-q) N e^{-r t} d t \\ s . t . \quad \dot{q} &=-\alpha\left[q-1+F_{\theta}\left(1-\frac{(1+b) w-p_{o n}}{V}\right)\right], \quad q(0)=q_{0} \end{aligned}\right.
%\end{equation}

%The paper starts by solving the follower's problem, which is an optimal control problem and then computes the markup of the competitive retailer as the rational reaction to the prices used by the manufacturer. Subsequently, the rest part solves an optimal control problem of the manufacturer, taking into account the constraints on the manufacturer and the reaction function of the competitive retailer.

%A number of extensions might be considered however. First, the marketing mix policy (for example, including advertising, services provided by the retailer, guarantees provided by the manufacturer) can be considered and their effects on consumers' channel selection assessed. Second, while the author has used a risk neutral framework, it is evident that risk aversion if considered would favor a discriminating price policy and assume the survival of a channels portfolio. In this framework, one can expect that the distribution of consumers' acceptance level will play an important role. Finally, while the model considered here is of a theoretical nature, empirical data regarding channels selection by consumers (reveling thereby the consumers' acceptance level) can provide a strong empirical verification to out analytical results.

\subsubsection{Pricing using Mixed Game Strategy}

In addition to cooperative and non-cooperative games, there are some pricing models based on mixed game strategies, e.g., the multi-channel pricing model \cite{yan2008pricing}, in which two kinds of competitive games are generally considered, i.e., Bertrand and the Stackelberg models in the marketing process.
Below we describe one typical example of pricing with mixture game.

\begin{example}{\bf  Quality of service (QoS) model in Internet pricing}.
%Cloud computing has recently been experiencing a high rate of growth, %mainly due to the ability of realizing highly scalable and reliable infrastructures for running software applications in an efficient and cost-effective way.
With the great advancement in computer technology, %a wider use of internet emerged for allocating valuable wireless resources.
there are many companies that provide internet services like broadband to computer or smart phone users. Many approaches have been proposed to study the pricing problem of the Internet Service Provider (ISP) and the users. Game theory can be applied to %the study of the Internet pricing issue. Particularly, game theory is used to
study the game equilibrium between the service provider and the users in Internet pricing. %Unlike traditional wireless devices, cognitive radio nodes are aware of their capabilities, environment, and intended use, and can also learn new waveforms, models, or operational scenarios.

%The central issue of Internet service is pricing, which can be used as an effective means to recover cost, to increase competition among different service providers, and to reduce congestion or to control the traffic intensity.


Most existing works applying game theory to Internet pricing adopt a non-cooperative game framework, in which the ISP sets up a price as a leader and the users respond with a demand.
In contrast, \cite{cao2002internet} tackles the Internet pricing problem using two branches of game theory, i.e., non-cooperative game and cooperative game.
It is assumed that, the requests come from a Poisson process with an arrival rate $\lambda$, and each request requires a unit bandwidth to serve for an exponentially distributed time with a unit means. %Then the paper proposes a simple model for the QoS requirement. Besides the paper assumes that
Each request has a maximal acceptable response time, denoted as $s$, and $d(s)$ represents a distribution density function.
If the real service response time (i.e., the transmission time plus the waiting time) is smaller, the service is successful. Otherwise, it is considered a failure. A user earns $g(s)\ge0$ for a successful service with a maximal acceptable response time $s$ and earns 0 for a failed service.
%(This function can be discretized by using Dirac delta functions to represent a finite set of QoS requirements corresponding to different applications, such as voice over IP (VoIP), and email; A user earns $g(s)\ge0$ for a successful service with a maximal acceptable response time $s$($g(s)$ can also be discretized), and earns 0 for a failed service.

%The study confirms our original concern about the solution of the leader-follower game approach: it may not be on the Pareto boundary and may not be fair and show that by cooperation a 'fair' solution can be obtained at which both the ISP and the user are better off than the leader-follower solution.

%In the game, the ISP and the user choose respectively their best strategies (price for the ISP and demand for the user) to get their desired outcomes.

%The leader-follower game model has been widely used in studying the pricing issue. Let be the price that the ISP announces. With this price, the user determines its demand.  Given any price, the user chooses, where is the set of all 's, to maximize its utility. Knowing this reaction of the user, the ISP chooses a price, where is the set for all's, to maximize its utility.



%First, consider the case where the ISP provides only one type of service with link capacity unit $\mu$. Hence, for every request, the ISP charges a fee $c$. When a request with maximal acceptable response time arrives, the user submits it to the Internet with a probability $\alpha(s)$ and discards it with a probability $1-\alpha(s)$. One will see that if $d(s)$ is a continuous function, $\alpha(s)$ is either $0$ or $1$. When $d(s)$ is discretized, $\alpha(s)$ specifies the portion of a particular application that is submitted by the user. Overall, the arrival rate to the Internet is $\alpha \lambda$, where}
%\begin{equation}
%\alpha=\int_{0}^{\infty} \alpha(s)d(s)\;ds
%\end{equation}

%\noindent The user's utility is\begin{equation}
%u(c, \alpha)=\lambda \int_{0}^{\infty} g(s) \alpha(s) d(s)\left[1-e^{-(\mu-\alpha \lambda) s}\right] d s-\alpha \lambda c
%\end{equation}

%\noindent The ISP's utility is\begin{equation}
%U(c, \alpha)=\alpha \lambda c
%\end{equation}

The  QoS model consists of the cooperative model and the non-cooperative model.
Two players of the game are the ISP and the user (representing a group of users having the same characteristics). The ISP sets up a price for its service; based on the price and other considerations, the user determines the amount of request that it wants to submit to the Internet. The outcomes of a game are the utilities of each player (i.e., profits for the ISP and the user). In the game, the ISP and the user choose respectively their best strategies (price for the ISP and demand for the user) to get their desired outcomes.
(i) In the \textbf{non-cooperative game model}, the ISP is the ``leader'' who does the decision first, then the ``followers'', i.e., users, do their decisions. Let $c$ be the price that the ISP announces. With this price, the user determines its demand $r$. The utilities for the user and the ISP are denoted as $U(c,r)$ and $V(c,r)$, respectively. Given any price $c$, the user chooses $r(c) = \arg \left\{\max _{r \in R}[U(c, r)]\right\}$ (where $R$ is the set of all possible demands) to maximize its utility.
Knowing this reaction of the user, the ISP chooses a price $c^{*}=\arg \left\{\max _{c \in C}[V(c, r(c))]\right\}$, where $C$
is the set for all possible prices, to maximize its utility.
(ii) In  the \textbf{cooperative game model}, the two players are called bargainers. They work on the utility space. Each pair of reactions they make corresponds to one point in the utility space. The set of all the points in the utility space corresponding to all the feasible reactions, is called a bargaining set. The problem that the two bargainers are faced with is to negotiate for a ``fair'' point on this set as the outcome. %If no agreements can be reached by the two bargainers, one particular point, called the starting point, will be the outcome of the game. %Thus, only those points in with and should be considered.
The fair point chosen by the two players is called the solution to the problem.
%The cooperative game theory provides guidance to the negotiation or arbitration process.
In this approach, the two players, the ISP and the user, will choose a point on the Pareto boundary as their solution. %On the Pareto boundary, the social welfare defined as
%\begin{equation}
%\begin{aligned} S(\alpha) &=U(p, \alpha)+V(p, \alpha) \\ &=\lambda \int_{0}^{\infty} g(s) \alpha(s) f(s)\left[1-e^{-(\mu-\alpha \lambda) s}\right] d s \end{aligned}
%\end{equation}\\
%is maximized.

%The two players are faced with two main issues: what point should be chosen as the starting point, and what fairness criteria should be used. Recall that if the negotiation fails, the starting point will be picked up as the outcome. Thus, there seem to be two natural ways of choosing the starting point. The first one is to pick up the solution of the leader-follower game as the starting point of the bargaining problem. This implies that if they fail in negotiation, the ISP will determine a price. In this case, with the cooperative game, both the ISP and the user are better off. Another way is to choose the origin $(0,0)$ as the starting point. This may happen when either ISP or the user thinks that the leader-follower game gives an unacceptable solution and therefore decides not to have any business if negotiation fails. In this case, the cooperative game solution is fairer than the leader-follower one. After the starting point is determined, one only need to consider the upper-right quadrant with the starting point as the origin. The problem that remains is simply how to choose a parameter $\beta$ to determine the fair point on the Pareto.

With a simple QoS model, it is demonstrated that, the non-cooperative game may lead to a solution that is not Pareto optimal and, in some sense, may be unfair.
In contrast, the cooperative approach can provide a better solution.
The cooperative game approach between the ISP and the user is usually difficult to maintain.
The practical implication is that some regulations or arbitration will be helpful for reaching a fairer and more efficient solution.
%The paper also applied the QoS model to study the competition between two ISPs in a numerical example and found the Nash equilibrium point from which the two ISPs would not move without cooperation.
\end{example}

%The numerical result indicates that the non-cooperative situation seems not to be efficient enough. Future work cold concentrate on the non-cooperative part and try to establish the existence and uniqueness of the Nash equilibriums.\\
 	
%\begin{table*}[h]
%	\centering
%     \caption{Comparison on All Models}
%	\begin{tabular}
%		{p{60 pt}p{80 pt}p{100 pt}p{120 pt}}
%		\toprule[1pt]
%		\textbf{Model}&\textbf{Applications}&\textbf{Branch of Game}&\textbf{Features}\\
		
%		\midrule[1pt]
%		GSP(\cite{liu2015service})&Internet resource pricing&Cooperative game&Multi-server and multi-structure\\
		
%		UF(\cite{al2008stackelberg})&Internet resource pricing&Non-Cooperative game&Signal-to-Noise Ratio(SNR) based\\
		
%		GHP(\cite{zheng2017bridging})&Big data pricing&Non-Cooperative game&Hierarchical and single-controller\\
		
%		OMP(\cite{fruchter2005dynamic})&Channel pricing&Non-Cooperative game&Probability based and dual-channel\\
		
%		QoS(\cite{cao2002internet})&Internet resource pricing&		Mixed Strategies game&Numerical single-server\\
		
%		MCP(\cite{yan2008pricing})&Channel pricing&Mixed Strategies game&Multi-channel and multi-competition\\
%		\bottomrule[1pt]	
%	\end{tabular}
%\end{table*}


==> introduction-1.tex <==


\section{Introduction}
\label{intro}




The data from various data generation sources have significant economic and social value, which play an important role in big data era.
Data are transforming science, business, and governance by making decisions increasingly and by enabling data-driven applications.
Due to many reasons such as separated systems, company regulations, and  data privacy,  mining data value suffers from the ``isolated data islands'' where the data scatter at different places.
For example, most of data owners are very unwilling to share their data.
It thus drives the emergence of modern data markets to bridge the gap between data owners and data buyers under the dilemma of ``isolated data islands''.



%break the issue of data isolation.
%Fortunately, the data markets, which \textcolor[rgb]{0.00,0.00,1.00}{allow} data owners to sell data and benefit from transactions, bridge the gap between data owners and data buyers, and alleviate the problem of ``isolated data islands''.
The data market acts as an intermediator for the buying and selling of diverse data, through which, the data generator (i.e., the seller) gets paid from the sold data, and the data consumer (i.e., the buyer) obtains beneficial data, as illustrated in Figure~\ref{fig:market}. In this way, the financial (resp. data) asset flows efficiently from the data consumer (resp. generator) to the data generator (resp. consumer).
%However, some markets fail to sell data among interested parties.
A good data market is able to carry out the  data circulation among interested parties.
%{\color{blue}It allows groups to not only strategically purchase available datasets to avoid the labor costs and skill requirements necessary for data curation, but also confidently understand  how a dataset was collected and cleaned and reliably generates a profit from sought-after datasets.}
It not only allows groups to strategically purchase available datasets to avoid the labor costs and skill requirements necessary for data curation, but also helps them concentrate on how to
take advantage of these datasets and reliably generates
a profit from sought-after datasets.
%\textcolor[rgb]{0.00,0.00,1.00}{Two real-life data trading scenarios are described as follows.}


%Eventually, a heathy and efficient data circulation will be built through such data markets.

%Fortunately, the recent emergence of modern data markets provides a good opportunity to break the issue of data isolation, and eventually to build a heathy and efficient data circulation.

%Fortunately, the data markets, which \textcolor[rgb]{0.00,0.00,1.00}{allow} data owners to sell data and benefit from transactions, bridge the gap between data owners and data buyers, and alleviate the problem of ``isolated data islands''.

%In particular, GBDEx~\cite{gbdex} possesses 225 high-quality data sources and more than 4,000 tradable data products, which has made 150PB trade volume involving more than thirty application fields.
%Microsoft Azure Marketplace~\cite{azure}, as an online store, offers applications and services either built on or designed to integrate with Microsoft's Azure public cloud.
%Infochimps~\cite{infochimps} is a data platform and marketplace for sharing and selling data of all types. The InfoChimps datasets API provides access to 2,000 ``tables'' of data across several categories, including science, government, sports and music. The site allows for searching for datasets by keyword, cost and tags. Sample API calls are documented along with each dataset. Free datasets can be accessed up to 100,000 calls per month, then InfoChimps offers tiered pricing.
%Meanwhile, there are a variety of data  markets selling specified types of data. For example, GNIP~\cite{gnip} aggregates and sells social media data from Twitter before the general data protection regulation (GDPR);
%Xignite~\cite{xignite} vends real-time financial data;
%Here~\cite{here} trades tracking and positioning data for location-based advertising;
%Factual~\cite{factual} enables location data to power innovation in product development, mobile marketing and real-world analytics.
%In addition, the value of human data is estimated at \$1.3 trillion but most of it is untapped. Datasift~\cite{datasift} helps extract and create more value in the ever-expanding universe of human data.



%(e.g., YoueData\footnote{YoueData is available at http://www.youedata.com}, Factual\footnote{Factual is available at https://www.factual.com/}, GBDEX\footnote{GBDEX is available at http://www.gbdex.com/}, and Datasift\footnote{Datasift is available at https://datasift.com/}) to facilitate the buying and selling of data.

%Also, some particular kind of data is attracting more and more attentions in data markets. %


\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{struc.eps}
\caption{The structure of a data market}%from Pricing Approaches for Data Markets
\label{fig:market}
%\vspace{-1.5em}
\end{figure}


%Data pricing is critical for a dynamic data market.

During the management of data markets, how to price the data is an indispensable problem.
It has received much attention from both  \emph{industry} and \emph{academia}.
First, %regarding the industry development,
the emerging data markets (such as Microsoft Azure Marketplace~\cite{azure}, GBDEx~\cite{gbdex}, InfoChimps~\cite{infochimps}, etc.)  have the goals of completely enabling the data circulation and effectively solving the data isolation issue, so as to facilitate the openness and share of global data resources~\cite{youedata}.
On the other hand, regarding the academic research, the term ``data marketplace'' was firstly used by Armstrong and Durfee \textcolor[rgb]{0.00,0.00,1.00}{as early as in 1998~\cite{armstrong1998mixing}, and also attracts much attention recently~\cite{fernandez2020data,muschalle2012pricing,schomm2013marketplaces}.}
%It models information trade between digital libraries, concentrating on the motivation and behavior of participants and identifying factors that affect cooperation in a network.
%Followed by the work of Ge et al.~\cite{ge2005model}, it
%investigates five different initial question and answer websites (e.g., Askjeeves \cite{askjeeves})  and  their business models.
%However, no technical details have been analyzed.
The problem of data pricing is important yet challenging in modern data markets.
An incentive pricing mechanism helps facilitate a dynamic and healthy data market development.
Two real-life data pricing scenarios are described as follows. %make the basis of categories easy to understand.

%show how data pricing works in real world, for ease understanding on
%Up to now, some modern data pricing solutions have been proposed in a wide range of practical situations.
%Below are two application examples.

%Real estate price data

\begin{example}\label{exm:estate}


\textbf{Pricing real estate trade data}.
Suppose a data company collects a real estate trade dataset $D$ in Hangzhou, a city of China.
This dataset not only contains the real estate price, but also records the information around the house, e.g., how many shopping malls around, the convenience of transportation facilities, etc.
It is beneficial for a \emph{real estate investment company} to make decisions of building a new apartment in certain region.
For example, an investment analyst, John, is willing to require a subset of the real estate trade dataset $D$, i.e., the real estate trade at West lake district of Hangzhou, to make a thorough quarterly report for this area.
Thus, in addition to trading the whole dataset, it is very common to trade the $D$'s subsets to meet various preferences.
On the other hand, for real estate investment, it is very important to obtain a real estate price prediction model for a newly developing district to accurately estimate the profit after investment.
In such situations, John concentrates more on some  machine learning models, instead of the original  dataset $D$.
Hence, there are urgent needs to trade the machine learning models.
\end{example}

%\begin{example}\label{exa:american}
%\textbf{American traffic data trade}.
%	Suppose a data company sells the American traffic database for \$399. A customer can also buy the subset of companies that have an email address for \$299 or only information about businesses in Washington State for \$199.
%	A customer interested only in a set of specific counties in various states may not be willing to pay \$399 for data she does not need, and so refuses to buy.
%	In response, the seller might provide a database for each county in every state. However, the relationship between state-based pricing and county-based pricing is difficult for either the seller or the buyer to reason about, where \emph{inconsistencies} or \emph{arbitrage} situations may result. For example, if the database does not contain any business information for some fraction of counties in a state, purchasing the data for the remaining counties could be cheaper, yet could yield the same information content as purchasing the data for the entire state.
%\end{example}

%A more recent study has been performed by EDD DUMBILL, who takes a closer look at the four biggest data marketplaces (Infochimps, Factual, Windows Azure Data Marketplace,
%and DataMarket).
%However, the underlying methodology is not disclosed, the work is not reviewed and only published as a blog article.

%Ge et al.~\cite{ge2005model} is one of the most important predecessors of studying information marketplaces.
%The potential of an electronic information marketplace is initially discussed, including the review of existing business models.



%Thus, the vale of data is getting more and more attentions from the industry, and thus a variety of data markets appear, such as Window Azure , Infochimps , etc.












%\subsection{Application Examples}
%\label{sec:2}

%Data pricing can be applied to various fields, we will give some examples.

%Further applications will be discussed in section 5.
%
%\textbf{Ride-sharing problem}. In typical ridesharing platforms (Uber and Didi Chuxing), the price of a ridesharing order is decided after user's input of destination and before his/her drop of an order. Therefore, the prices of the ridesharing orders are fixed regardless of the dispatch and routing results. This is quite different from non-ridesharing orders whose price may depend on the actual travel length, location of the customer, time and so on.
%\begin{figure}
%	\centering
%	\includegraphics[width=0.5\textwidth]{sharing.eps}
%	\caption{Example 1.}
%\end{figure}
%
%In Figure 1, there are three orders $o_1$, $o_2$, $o_3$ and only
%one vehicle $v_1$. $o_1^s$, $o_2^s$, $o_3^s$ and $o_1^e$, $o_2^e$, $o_3^e$ represent the origins and destinations respectively. Circles and edges represent the nodes
%and paths respectively in the road network~\cite{zheng2018order}. In this example, all
%edges are of equal travel distance. This example corresponds to
%peak ordering periods where vehicles are in shortage. There are
%two possible travel plans for $v_1$: (i) $v_1 o_1^s o_2^s o_1^e o_2^e$; (ii) $v_1 o_1^s o_2^s o_1^e o_2^e$.
%Without considering the order prices, the above two plans show
%no difference because they own the same amount of travel distance
%and the same number of served orders. Let us consider the order
%prices and assume price($o_2$) > price($o_3$). This is reasonable
%as $d(o_2^s,o_2^e)$ > $d(o_3^s,o_3^e)$. Note that $d(¡¤, ¡¤)$ represents the shortest path distance, and has a strong impact on orders' price in practice. Then, the price-aware solution would be dispatching $o_1$ and $o_2$ to
%$v_1$.
%
%And then we can set a price for this trip according to the above price-aware solution.
%\end{example}
%
%Example 2. Online ad auction\cite{constantin2009online}. Many advertisers (bidders) use Internet systems to buy display
%advertisements on publishers' webpages or on traditional
%media such as radio, TV and newsprint. They seek
%a simple, online mechanism to reserve ad slots in advance.
%On the other hand, media publishers (sellers) represent a vast
%and varying inventory, and they too seek automatic, online
%mechanisms for pricing and allocating such reservations. Such mechanisms can be established using data pricing knowledge.
%
%Consider one platform and two bidders' situation. The expected revenue of the advertisement can be represent by revenue per click (RPC). For these two bidders A and B with the RPC \$0.5 and \$0.4, their highest bids are \$0.5 and \$0.4. Bidders have to compete with others under the circumstance that they can profit. The platform will choose the highest bid that they can offer. Suppose that the click numbers are the same for A and B, then A will win the auction since A can bid higher than B.
%
%Example 3. Prediction market. Such markets are a recent phenomenon and have generated a lot of interest,
%rightly so. See \cite{wolfers2004prediction} for a detailed overview. Typically, in such markets, there is a discrete random
%variable, $W$, that a firm wants to accurately predict. The market executes as follows: (i) ¡°experts" sell
%probability distributions $\Delta_W$ i.e., predictions on the chance of each outcome; (ii) the true outcome,
%$w$, is observed; (iii) the market pays the ¡°experts" based on $\Delta_W$ and $w$. In such literature, payment
%functions based on the Kullback¨CLeibler divergence are commonly utilized, as they incentivize ¡°experts" to be truthful (\cite{hanson2012logarithmic}). Despite similarities, prediction markets remain infeasible for data as ¡°experts" have to explicitly choose which tasks to make specific predictions for. In contrast, it is not known a priori whether a particular dataset has any importance for a prediction task;
%
\begin{example}\label{exm:flow}
\textbf{Pricing passenger flow data}.
%The passenger flow dataset records the number of passengers in public places, such as shopping mall and museum. It is useful for business and decision-making.
Suppose there is a passenger flow dataset from commercial districts that is collected by the cameras in the malls.
The passenger flow data analysis is essential for managers to make smart business decisions and harvest more profit.
For instance, a restaurant manager, David, has to leverage the nearby passenger flow data on the second floor to  reasonably determine the marketing plan.
Hence, he needs to consume a fraction of the passenger flow dataset to achieve this goal.
Moreover,  predicting the number of passengers in the peak time of holidays  can better plan staff allocation in advance.
In this setting, it is necessary to trade machine learning models over the passenger flow dataset.
%Thus, the trading for raw data subsets and machine learning models is indispensable for practical applications.
%There are some cases calling for the various pricing schemes.
%Consider David, a restaurant owner, would like to open a new shop in this area.
%He wants to know the people flow data around the location of his new shop, in order to estimate the revenue.
%Thus, his need is only part of the data set.
%Buying the whole dataset is obviously not suitable for him.
%
%Also, a clothes shop owner, Linda, is willing to buy the predictive service based on the dataset.
%Specifically, she needs to determine how many temporary workers will be employed in the holiday.
%To achieve this, the predictive people flow data is required.
%In this setting, Linda would like to buy a model to predict and make better decisions.
\end{example}
%\begin{example}\label{exm:flow}
%{\color{blue}
%\textbf{People flow data trade}.
%Suppose there is a dataset, which records the people flow data in a specific area for a period of time.
%For instance, how many the people in the mall at 3pm on June 1st is recorded.
%This dataset can be generated by sensors, and we assume it is ready.
%
%There are some cases calling for the various pricing schemes.
%Consider David, a restaurant owner, would like to open a new shop in this area.
%He wants to know the people flow data around the location of his new shop, in order to estimate the revenue.
%Thus, his need is only part of the data set.
%Buying the whole dataset is obviously not suitable for him.
%
%Also, a clothes shop owner, Linda, is willing to buy the predictive service based on the dataset.
%Specifically, she needs to determine how many temporary workers will be employed in the holiday.
%To achieve this, the predictive people flow data is required.
%In this setting, Linda would like to buy a model to predict and make better decisions. }
%\end{example}
%\begin{example}\label{exm:demographic}
%\textbf{Demographic data trade}.
%Consider John, a journalist, studying the relationship between demographics and economic indicators for an article. He wants to test how predictive some demographic features are of the average annual household income.
%Datasets online is available but too expensive for him. In this scenario, if datasets are sold with fixed price, John will not be able to obtain them, and the sellers cannot get revenue as well.
%\textcolor[rgb]{0.00,0.00,1.00}{What's more, using a simplistic pricing scheme may create undesirable arbitrary opportunities and cheaper prices, when John is with machine learning skills.}
%If a data \textcolor[rgb]{0.00,0.00,1.00}{market} allows John to be charged only based on his machine learning (ML) task(s) and desired accuracy, both John and the sellers will be satisfied. In particular, a linear regression model instance with a square loss might be sufficient for his purposes and cheap enough for John to purchase. \end{example}
%\textcolor[rgb]{1.00,0.00,0.00}{With ML skills, John will be able to build simplistic pricing schemes which may create undesirable arbitrary opportunities and cheaper prices.}


%Data pricing is critical for a dynamic data market.
%
%During the management of data markets, how to price the data is an indispensable problem.
%It has received much attention from both  \emph{industry} and \emph{academia}.
%First, %regarding the industry development,
%the emerging data markets (such as Microsoft Azure Marketplace~\cite{azure}, GBDEx~\cite{gbdex}, InfoChimps~\cite{infochimps}, etc.)  have the goals of completely enabling the data circulation and effectively solving the data isolation issue, so as to facilitate the openness and share of global data resources~\cite{youedata}.
%On the other hand, regarding the academic research, the term ``data marketplace'' was firstly used by Armstrong and Durfee in 1998~\cite{armstrong1998mixing}.
%%It models information trade between digital libraries, concentrating on the motivation and behavior of participants and identifying factors that affect cooperation in a network.
%%Followed by the work of Ge et al.~\cite{ge2005model}, it
%%investigates five different initial question and answer websites (e.g., Askjeeves \cite{askjeeves})  and  their business models.
%%However, no technical details have been analyzed.
%The problem of data pricing is important yet challenging in modern data markets.
%An incentive pricing mechanism helps facilitate a dynamic and healthy data market development.
%%Two real-life data pricing scenarios are described as follows. %make the basis of categories easy to understand.
%
%%show how data pricing works in real world, for ease understanding on
%%Up to now, some modern data pricing solutions have been proposed in a wide range of practical situations.
%%Below are two application examples.
%
%%Real estate price data

\begin{comment}
First, the conclusion of each example is ''the trade for xx is needed'', which do not reflect the urgent need of data pricing.
Second, the "Therefore, in this paper, we conduct xxx" is better to connect with the last paragraph " An incentive pricing mechanism helps facilitate a dynamic and healthy data market development.", since the 2 examples do not reflect the pros of data pricing.
\end{comment}
%As a matter of fact, in addition to the two scenarios directly referring to big data analytics, there exist some other data pricing solutions originated from other disciplines, e.g., microeconomics, management science, operation research, etc.
%Up to now
%\textcolor[rgb]{0.00,0.00,1.00}{Inspired by these real-life scenarios, some modern data pricing solutions have been proposed in a wide range of practical situations.
\textcolor[rgb]{0.00,0.00,1.00}{In such scenarios, how to derive the price of data is the basis of data trading, and determines whether the transaction can be completed.}
Therefore, in this paper,  we conduct a comprehensive survey on data pricing solutions.
%As a brand-new topic emerged in smart data analytics and management, there are emerging pricing solutions for the data trade.
%We also overview the related pricing schemes that are potential to the data pricing issue.
We build a taxonomy of data pricing solutions. It consists of \emph{three} pricing strategies,  i.e., the \emph{query pricing strategy} (QP strategy for short), and the \emph{feature-based data pricing strategy} (FP strategy for short), and \emph{pricing strategy in machine learning} (MLP strategy for short).
To the best of our knowledge, this is a thorough taxonomy of so many data pricing solutions, which  basically cover all the existing data pricing methods. %there are several specific pricing models in each category, according to the different pricing perspectives among them.
%, and \emph{pricing strategy in database}, and \emph{pricing strategy in machine learning}.
%To be more specific, regarding the field of pricing model, \emph{query} pricing and \emph{feature-based} data pricing mainly belong to database field, and another is for \emph{machine learning}.

Specifically, we elaborate the three pricing strategies and make in-depth analyses over them.
In particular, the query pricing strategy established by the database community aims to derive prices for diverse queries proposed by data buyers.
It is mainly composed of five pricing models, i.e., query pricing with data view (Q1), query pricing based on information value (Q2), query pricing using data provenance (Q3), auction-based query pricing (Q4), and pricing in mobile crowd sensing (Q5).
In contrast, the feature-based data pricing strategy focuses on how to price data with data features, such as data quality, data privacy, and so on.
There are four pricing models in this strategy, namely, data pricing based on data quality (F1), personal data pricing using data privacy (F2), personal data pricing with market value (F3), and pricing social network with influence (F4).
In addition, the pricing strategy in machine learning (ML) community  supports the trade of ML models.
To be more specific, there are four pricing mechanisms for pricing in machine learning, i.e., the noise-injection pricing mechanism (M1), pricing with shapley value (M2), end to end pricing framework (M3), and pricing in federated learning (M4).
\textcolor[rgb]{0.00,0.00,1.00}{Overall,} these pricing schemes can be used to offer reasonable prices for various queries and ML models, so as to support the data pricing scenarios like Example \ref{exm:estate} and Example \ref{exm:flow}.   %These pricing schemes are suitable for people with similar requirements of John and Linda, as Example \ref{exm:estate} and \ref{exm:flow} show.









%The former four pricing mechanisms mainly relies on the database schema, and sets price for a certain number of tuples or values in the dataset, which can be adopted in Example \ref{exa:american}.


%However, pricing in mobile crowd sensing focuses on pricing mobile crowd sensing data, and the queries over data are different from traditional SQL queries, as the data product is modeled as a distribution.
%Meanwhile, the feature-based data pricing \textcolor[rgb]{0.00,0.00,1.00}{strategy} is able to provide the price of whole dataset according to data features, such as privacy, market value, accuracy, completeness, and multi-dimension quality.
%For pricing social network strategy, it is different from the former feature-based pricing methods, since it trades the nodes on social networks, which are a special format of data.
%It utilizes the influence of nodes to derive a proper price.



%In contrast, the machine learning pricing mechanism incorporates both the trained data and the learned models into the pricing process, which is suitable for Example \ref{exm:demographic}.
%There are four different pricing mechanisms in machine learning, including the noise-injection pricing mechanism, pricing with shapley value, end to end pricing framework, and pricing in federated learning.
%The noise-injection pricing mechanism provides different versions of model for trade by adding noise, and the price is derived with the goal of revenue maximization.
%And pricing with shapley value is a fair way to measure the contribution of data, and offers data price based on data contribution.
%The end to end pricing framework considers both model pricing and data pricing, and build a whole framework for data \textcolor[rgb]{0.00,0.00,1.00}{market} in machine learning.
%The pricing mechanism in federated learning \textcolor[rgb]{0.00,0.00,1.00}{aims to incentivize data sharing among data owners, and data price} depends on what data brings to federated learning.

%The second pricing strategy contains the \emph{game theory based pricing} (GTP) model and  \emph{auction based pricing} (ACP) model.
%The GTP model considers the bargaining battle between the data seller and buyers with the support of game theory.
%While the ACP model  is based on auction  theory to price the data in data markets.
%The pricing models in social networks (i.e., SNP model) belong to the third pricing strategy.
%The reason that we highlight the pricing models in social networks lies, more and more knowledge is formatted as complex graphs/networks, which makes the pricing issue in networks more challenging.
%\ref{subsec:tsm-model}.
%Also, pricing on social networks is another important line of data pricing, and we describe the SNP model in Section \ref{subsec:sn-model}.
%We sincerely hope that, this survey could provide useful insights for researchers who are interested in data pricing and data trade. We do believe that, this work puts a substantial step to the development of data economy.

%It is our sincere hope that, this survey could provide useful insights for researchers who are interested in data pricing and data trade.

%\textcolor[rgb]{0.00,0.00,1.00}{Over recent years, there are also some surveys of data pricing \textcolor[rgb]{0.00,0.00,1.00}{~\cite{sen2013survey,liang2018survey,Zhang2020survey,pei2020survey}}.
%Some of them focus on survey of broadband pricing or digital products pricing, instead of data pricing we mentioned, while survey in \cite{Zhang2020survey} lacks pricing for ML models, and there is no taxonomy in \cite{pei2020survey}.
%In contrast, we not only conduct a comprehensive survey on existing \emph{data} pricing methods, but also build a \emph{taxonomy} over them (with analysis and comparison).
%To the best of our knowledge, this is the first attempt to tackle the problem of taxonomy of data pricing.}
%However,
%the ``smart'' data pricing in \cite{sen2013survey} refers to the broadband pricing schemes, which \textcolor[rgb]{0.00,0.00,1.00}{is different} from the meaning of data pricing in this paper.
%And the pricing models in \cite{liang2018survey} mainly focus on pricing of digital products, while \cite{Zhang2020survey} does not consider data pricing in machine learning methods, \textcolor[rgb]{0.00,0.00,1.00}{where training} models are a special product of data.


%Over recent years, there are also some surveys of data pricing \textcolor[rgb]{0.00,0.00,1.00}{~\cite{sen2013survey,liang2018survey,Zhang2020survey,pei2020survey}}.
%However,
%the ``smart'' data pricing in \cite{sen2013survey} refers to the broadband pricing schemes, which \textcolor[rgb]{0.00,0.00,1.00}{is different} from the data pricing that we mean.
%And the pricing models in \cite{liang2018survey} mainly focus on pricing of digital products, while \cite{Zhang2020survey} does not involves machine learning pricing \textcolor[rgb]{0.00,0.00,1.00}{methods, where trained }models are a special product of data.
%The survey conducted in \cite{pei2020survey} \textcolor[rgb]{0.00,0.00,1.00}{offers} a general \textcolor[rgb]{0.00,0.00,1.00}{vision} of data pricing, involving digital products pricing and data products pricing.
%%\textcolor[rgb]{0.00,0.00,1.00}{and some pricing related issues are pointed out}
%Different from this work, we carefully overview the existing data pricing model on data \emph{products}, and conduct a \emph{taxonomy} of these pricing models, while \cite{pei2020survey} just points out the related issues of data pricing, such as fairness, arbitrage-freeness, etc.
%And these issues are also included in our study, which are introduced in different pricing \textcolor[rgb]{0.00,0.00,1.00}{models}.
%Meanwhile, the pricing \textcolor[rgb]{0.00,0.00,1.00}{scheme} about federated learning we mentioned is not considered in \cite{pei2020survey}.
%Different from prior works, we carefully overview the existing pricing model, not only in database field, but also in machine learning filed.



Moreover, we identify five research challenges of data pricing, and provide some preliminary ideas on how to approach these challenges in principle.
%In addition, we put forwards more concerns about the data lifecycle in data markets as well as the regulations on data trade.
We put forwards some interesting topics about data pricing in data markets for future direction.
We aim at providing useful insights for researchers who are interested in data pricing and data trade.
%In contrast, we not only conduct a comprehensive survey on existing \emph{data} pricing methods, but also build a \emph{taxonomy} over them (with analysis and comparison).
We do believe that, this survey puts an initial but substantial step to the development of data trade and share.
In addition, it is worthwhile to mention that, this survey is different from existing data pricing surveys, which either focus on  other products pricing such as broadband and digital products~\cite{liang2018survey,sen2013survey}, or only simply survey existing methods without offering a taxonomy~\cite{pei2020survey,Zhang2020survey}.
To the best of our knowledge, this is the first attempt to tackle the problem of taxonomy over data pricing.
In a nutshell, this paper mainly  has the following notable contributions.
%
%Over recent years, there are also some surveys of data pricing \textcolor[rgb]{0.00,0.00,1.00}{~\cite{sen2013survey,liang2018survey,Zhang2020survey,pei2020survey}}.
%Some of them focus on survey of broadband pricing or digital products pricing, instead of data pricing we mentioned, while survey in \cite{Zhang2020survey} lacks pricing for ML models, and there is no taxonomy in \cite{pei2020survey}.


\begin{itemize}
\item \textbf{New taxonomy.} We propose a new taxonomy of modern data pricing models. It consists of three parts, including query pricing (QP) strategy, feature-based data pricing (FP) strategy, and pricing strategy in machine learning (MLP).
    %We conduct a comprehensive survey of data pricing. It is so far the most complete taxonomy of data pricing solutions.
\item \textbf{Comprehensive review.} We conduct a comprehensive overview of modern data pricing solutions to various scenarios. We elaborate representative data pricing models, and provide a series of insights and comparisons for modern data pricing models.
     %propose a taxonomy of data pricing solutions with three pricing strategies and thirteen pricing models.
% We elaborate the thirteen pricing models via in-depth comparisons, including pricing perspectives, techniques, etc.
\item \textbf{Future directions.} We put forward five research challenges in terms of efficiency, universality, scalability, interdisciplines, and adaptability. We also present several future directions of data pricing study.
\end{itemize}



The rest of the paper is organized as follows. We introduce the basic concepts  of data markets in Section \ref{sec:concpet}.
Section~\ref{sec:taxonomy} establishes the taxonomy of data pricing solutions.
We elaborate three pricing strategies in Section \ref{sec:qpmodel}, Section \ref{sec:fbmodel}, and Section \ref{sec:mlmodel}, respectively.
Then, we highlight five challenges and some interesting topics over data pricing in Section~\ref{sec:future}.
%In addition, we summarize and compare existing commercial data markets in Section~\ref{sec:market}.
Finally,  we conclude our survey in Section~\ref{sec:conclusion}. %Based on these trends, we highlight four challenges and possible solutions.
%we conclude the survey and put forward a series of potential research directions on the data pricing study.
%roots. Section 5 provides our conclusions and four
%possible development trends in cloud pricing. Based on these trends, we highlight four challenges
%and possible solutions. All acronyms in this article are listed



%The outline of the paper is organized as follows.
%Section \ref{sec:concpet} introduces basic concepts of data and describes the key factors of valuing the data.
%and the pricing model taxonomy in Section~\ref{sec:taxonomy}.
%In Section~\ref{sec:model}, we elaborate each modern pricing model including database-based pricing model in Section \ref{subsec:db-model}, machine learning based pricing model in Section \ref{subsec:ml-model}, game theory based pricing model in Section \ref{subsec:gt-model}, pricing on two-sided markets in Section \ref{subsec:tsm-model}, pricing in social networks in Section \ref{subsec:sn-model}. %and price discrimination in Section \ref{subsec:pd-model}.
%We explore data pricing applications in Section \ref{sec:applicaiton} including pricing in real-time sharing, pricing in mobile crowd sensing, online advertisement auction, and some others.
%Existing commercial data markets are investigated in Section~\ref{sec:market}.
%In Section~\ref{sec:other}, we discuss some potential research directions closely related to data pricing, including data copyright, data access, data privacy, data economy, etc.
%Finally, Section~\ref{sec:conclusion} concludes the survey.

%The outline of the paper is organized as follows.
%Section \ref{sec:concpet} introduces basic concepts of data markets.
%We describe the key factors of valuing the data and the pricing model taxonomy in Section~\ref{sec:taxonomy}.
%In Section \ref{sec:model}, we elaborate each modern pricing model including database-based pricing model in Section \ref{subsec:db-model}, machine learning based pricing model in Section \ref{subsec:ml-model}, game theory based pricing model in Section \ref{subsec:gt-model}, pricing on two-sided markets in Section \ref{subsec:tsm-model}, pricing in social networks in Section \ref{subsec:sn-model}, and price discrimination in Section \ref{subsec:pd-model}.
%We explore data pricing applications in Section \ref{sec:applicaiton} including pricing in real-time sharing, pricing in mobile crowd sensing, online advertisement auction, and some others.
%Existing commercial data markets are investigated in Section~\ref{sec:market}.
%In Section~\ref{sec:other}, we discuss some potential research directions closely related to data pricing, including data copyright, data access, data privacy, data economy, etc.
%Finally, Section~\ref{sec:conclusion} concludes the survey.


==> model.tex <==


\section{Pricing in Database}
\label{sec:dbmodel}

\textcolor[rgb]{0.00,0.00,1.00}{In this section, we first overview the concept of data pricing in database, and the basic pricing strategies in data markets.
Then we elaborate three categories, and introduce six existing pricing models.
Last, we summarize and compare these works carefully.
}

 %\emph{database based pricing model} (DBP model for short),  \emph{machine learning based pricing model} (MLP model for short),  \emph{game theory based pricing model} (GTP model for short),  \emph{auction based pricing model} (ACP model for short),  \emph{pricing in social networks} (SNP model for short). %and  \emph{the pricing model incorporating price discrimination} (PDP model for short).
%Table \ref{tab:symbol} consists of the symbols frequently used throughout this paper.


%\begin{table*}[h]
%	\centering\small
%\caption{Symbols and Description}\label{tab:symbol}
%%\setlength{\tabcolsep}{35pt}
%\centering%\small
%	\begin{tabular}[t]	%{ll}
%		{p{100 pt}p{240 pt}}
%		\toprule[0.7pt]
%		\textbf{Symbol}& \textbf{Description}\\
%		\midrule[0.3pt]
%		$D$   &a database\\		
%		$Q$   &a query\\		
%		$\mathbf{Q}$/$\mathbf{V}$   &query bundles\\
%        $Q(D)$   & the query result set of $Q$ w.r.t. the database $D$ \\	
%        $p_D(Q)$   & the price of the query $Q$ w.r.t. the database $D$\\
%		$P$   &the set of players\\
%
%        $U/u(*)$ &the data buyer's utility function\\
%
%        %$D/d(*)$ &the {\color{red}density function}\\
%
%        $p/q$ &the price\\
%
%        $R/r$&the revenue (payoff) of data trade\\
%
%        $t$& the time parameter\\
%
%		\bottomrule[0.7pt]
%	\end{tabular}
%\end{table*}



%{\color{blue}In this section, we will introduce some pricing models including (i) database based pricing model, (ii) machine learning based pricing model, (iii) game theory based pricing model, (iv) auction based pricing model and (v) pricing in social networks.}





%Following the s of data marketplaces~\cite{armstrong1998mixing,ge2005model},
The \textcolor[rgb]{0.00,0.00,1.00}{pricing model in database} refers to sell the relational datasets by tables or relations.
Balazinska et al.~\cite{balazinska2011data} firstly introduce the concept of \emph{data markets} into database community.
They present several modeling parameters that a pricing market should define:
(i) the structural granularity at which the seller should attach prices (this could be either tuples or cells of tables, queries, relations, etc.);
(ii) a base pricing function attaching seller defined prices at the chosen granularity;
(iii) a method for determining the price of every other allowable interaction with the database (e.g., query price) from the base pricing function; and (iv) a subscription mode specifying how updates to the data are priced. %
They also axiomatically define some desiderata for pricing functions, like \emph{arbitrage-freeness}, \emph{fairness}, and \emph{efficiency}.


Several initial data marketplace surveys~\cite{muschalle2012pricing,schomm2013marketplaces} have been conducted in database community, and four general and typical pricing strategies are summarized.


%\textbf{Arbitrage-freeness}.
%
%\textbf{Fairness}.
%
%\textbf{Efficiency}.


%\footnote{https://www.data.gov/}

\begin{itemize}\setlength{\itemsep}{-\itemsep}
\item{} \textbf{Freemium}. These data (services) can be used at no charge, e.g., data can be obtained from public authorities.
Reasons for offering a service for free are, among others, that it is only a beta test or research project, the vendor is a public authority funded by tax money, or simply interested in attracting more customers.
For example, Data.gov~\cite{datagov} is free as it is a website of the U.S. government.
%Vendors in this category do not count towards one of the following categories.



%In addition, \emph{freemium} is another approach to price data on marketplaces.


\item{} \textbf{Usage-based pricing}. It corresponds to how many data are utilized with the human rationality, and each single unit of a commodity raises the total amount of money to pay for.
Customers are billed based on how much they use the respective service. % (it manifests mostly in the form of \$$x$ per thousand API calls);


\item{} \textbf{Package pricing}. It refers to a pricing model that offers a customer a certain
amount of data or API calls for a fixed fee. Alternatively, after paying a fixed amount of money, customers can make unlimited use of the service for a limited time, mostly a month or a year (i.e., the typical subscription model). A related topic is \emph{product bundling}, which occurs when distinct products are sold together as a package. Bundling is a common practice for information goods. One of Microsoft's most successful products in recent years has been Microsoft Office, which is a bundle of different software products.



\item{}  \textbf{Flat fee tariff}. It is one of the simplest pricing models with minimal transaction costs.
    It is based on time as the only parameter.
\end{itemize}

In addition, the freemium models are always combined with at least one of the aforementioned payment models.
The idea is to let users join and use basic services for free and charge them for (premium) services that provide additional value to customers.
%The payment model for additional services can take any other pricing models.
It offers a limited access at no cost with the possibility of an update to a fee-based premium access.


\textcolor[rgb]{0.00,0.00,1.00}{The above pricing strategies are mainly used in real data marketplaces, which are too simple to adapt to reality.
Hence, a series of studies make efforts to price data in database, and we divide them \textcolor[rgb]{1.00,0.00,0.00}{three} categories, namely, the \emph{query} pricing models and the \emph{personal data} pricing models in database.
In particular, \textcolor[rgb]{1.00,0.00,0.00}{six} pricing models are introduced, i.e., pricing model with data view, pricing with information value, pricing using data provenance, pricing using query cost, pricing personal data with privacy, pricing personal data with market value.}

%(iv) \emph{the flat fee tariff}: it is one of the simplest pricing models with minimal transaction costs. It is based on time as the only parameter.
%In addition, \emph{freemium} is another approach to price data on marketplaces.
%The idea is to let users join and use basic services for free and charge them for (premium) services that provide additional value to customers.
%The payment model for additional services can take any of the aforementioned forms.
%It offers a limited access at no cost with the possibility of an update to a fee-based premium access;
\subsection{Query Pricing}
\label{subsec:dbquery-model}
\textcolor[rgb]{0.00,0.00,1.00}{
Query pricing is proposed to be inspired by such a scenario, where the buyers cannot afford the fee of whole dataset.
Instead, he/she is willing to purchase the subset of data that they need.
Thus, the concept of query pricing is introduced, and extensive studies focus this problem.
Up to now, there are four major pricing models designated for relational queries in the field of databases, namely, pricing model with \emph{data view}, pricing with \emph{information value}, pricing using \emph{data provenance}, pricing using \emph{query cost}.
These query pricing models price data from different perspective, and we will introduce them in the following.}
%The whole pricing framework is different from query pricing.
%To some extent, the view-based one relies  on the basis of the package pricing model, while the provenance-based one is closely related to the usage-based pricing.
%We also summarize the market-oriented models in database, which take market factors, such as revenue, social welfare, and market value, into account.


\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Query Pricing with Data View}}
\label{subsubsec:view-model}

First, in the data view-based QP model, the structural granularity of pricing is a query. The seller sets the price of a specific set of base queries (also called view), and then, the algorithm has to derive the price of any other query that could be made to the database.


There are a series of substantial studies in this category, consisting of pricing generalized chain queries (i.e., a special type of join conjunctive query when the base queries are only selection queries)~\cite{koutris2012querymarket,koutris2015query},
pricing SQL queries~\cite{balazinska2013discussion,deep2017qirana,koutris2013toward}, pricing aggregate queries~\cite{deep2017qirana,li2012pricing}, as well as pricing general queries~\cite{lin2014arbitrage}.


The pricing function should be arbitrage-free.  In particular, the \emph{arbitrage} property is studied based on an \emph{instance based determinacy} relationship~\cite{koutris2012querymarket,koutris2015query}.
Consider the USA business dataset: if $p$ is the price for the entire dataset and $p_1, \cdots, p_{50}$ the prices for the data in each of the 50 states, a rational seller would ensure that $p_1 + \cdots + p_{50}\geq p$. Otherwise, no buyer would pay for the entire dataset, but would instead buy all 50 states separately. In general, we say that a pricing function is arbitrage-free if whenever a query $q$ is ``determined'' by the queries $q_1, \cdots, q_n$, their prices satisfy $p \leq p_1 +\cdots + p_n$.


%A query bundle is a finite set of queries. % we use the term ``bundle'' rather than ``set'' to avoid confusion between a set of queries and a set of answers.
%$B(L)$ denotes the set of query bundles over $L$, and write a bundle as $Q$ = $(Q_1, \cdots, Q_m)$. The output schema of a query bundle is $\mathbf{R}_Q = (R_{Q_1}, \cdots, R_{Q_m})$, and consists of one relation name for each query. Thus, a bundle defines a function $Q$: $Inst_{\mathbf{R}} \rightarrow Inst_{\mathbf{R_Q}}$.

Let a query bundle $\mathbf{Q}$ = $(Q_1, \cdots, Q_n)$ be a finite set of queries that is asked simultaneously on the database. Given two query bundles $\mathbf{Q}_1$ and $\mathbf{Q}_2,$ we denote their union as $\mathbf{Q}$ = $\mathbf{Q}_1 \cup \mathbf{Q}_2$. This $\mathbf{Q}$ is the query bundle consisting of all queries in $\mathbf{Q}_1$ and $\mathbf{Q}_2$.

\begin{definition}\label{defn:determinacy}
{\bf (Instance based determinacy)}~\cite{koutris2015query}.
Let $D$ be a database instance and $\mathbf{V}, \mathbf{Q}$ be two query bundles. It is said that, $\mathbf{V}$ determines $\mathbf{Q}$ given $D$, in notation $D\vdash\mathbf{V}\twoheadrightarrow \mathbf{Q}$, if for any $D'$, $\mathbf{V}(D) = \mathbf{V}(D')$ implies $\mathbf{Q}(D) = \mathbf{Q}(D')$.
\end{definition}

Informally, a query bundle $\mathbf{V}$ (that contains a set of queries/views)  determines a query $Q$ if one can compute answers of $Q$ only from answers of these views in $\mathbf{V}$ without having access to the underlying database. Specifically, given a database $D$, $\mathbf{V}$ determines $Q$
(denoted as $D\vdash\mathbf{V} \twoheadrightarrow Q$) if one can answer $Q$ from answers of $\mathbf{V}$ by applying a function $f$ such that $Q(D)$ = $f(\mathbf{V}(D))$~\cite{koutris2015query}. The impact on pricing is that if the user needs to answer the query $Q$, s/he has also the option of querying $\mathbf{V}$ and then applying $f$.
Put it differently, $\mathbf{V}$  determines $Q$ if $\mathbf{V}$ provides enough information to uniquely determine answers to $Q$.
If $\mathbf{V}$ determines $Q$, a potential buyer interested in purchasing $Q$ can
buy $\mathbf{V}$ instead, and derive from it answers to $Q$: arbitrage \emph{occurs} when the price of $\mathbf{V}$ is lower than that of $Q$.
 % below.


\begin{definition}({\bf Arbitrage-freedom})~\cite{koutris2015query}.
 A pricing function $p_D$ is arbitrage-free if, whenever $D\vdash\mathbf{Q}_1, \cdots, \mathbf{Q}_k\twoheadrightarrow \mathbf{Q}$, then $p_D(\mathbf{Q})\leq \sum_{i=1}^kp_D(\mathbf{Q}_i)$.
\end{definition}

\begin{proposition}
\label{pro:free-qpricing}
Any arbitrage-free pricing function $p_D$ satisfies the following properties. In particular, $p_D()$ denotes the price of the empty bundle, and the identity bundle, denoted by $\mathbf{ID}$, is the bundle that returns the entire dataset $D$.

\noindent
$(i)$ Subadditivity: $p_D(\mathbf{Q}_1, \mathbf{Q}_2)\leq p_D(\mathbf{Q}_1) + p_D(\mathbf{Q}_2)$.

\noindent$(ii)$ Nonnegativity: $p_D(\mathbf{Q})\geq 0$.

\noindent$(iii)$ Not asking is free: $p_D()=0$.

\noindent$(iv)$ Upper-boundedness: $p_D(\mathbf{Q})\leq p_D(\mathbf{ID})$.
\end{proposition}

%\begin{definition}({\bf Bundle arbitrage})~\cite{green2017semiring}.
%Let the query bundle $\mathbf{Q}$ = $\mathbf{Q}_1$, $\mathbf{Q}_2$.
%The query price  $p$ has no bundle arbitrage if for every database $D$, we have $p_D(\mathbf{Q}) \leq p_D(\mathbf{Q}_1) + p_D(\mathbf{Q}_2)$.
%\end{definition}


The first property exactly refers to \emph{bundle arbitrage}. It regards the scenario where a data buyer that wants to obtain the answer for the bundle $\mathbf{Q}$ = $\mathbf{Q}_1$, $\mathbf{Q}_2$ creates two separate accounts, and uses one to ask for $\mathbf{Q}_1$ and the other to ask for $\mathbf{Q}_2$.
To avoid such an arbitrage situation, we must make sure that the price of $\mathbf{Q}$ is at most the sum of the prices for $\mathbf{Q}_1$ and $\mathbf{Q}_2$.


%The arbitrage is defined based on a notion of \emph{instance based determinacy}~\cite{koutris2015query}.










The QueryMarket system automatically prices a large class of SQL queries requested by buyers based on price-points specified by sellers~\cite{koutris2012querymarket,koutris2013toward}. It supports updates to the database and accounts for query history. It also allows multiple sellers to share revenues fairly.
Computing arbitrage-free prices is theoretically hard, and thereby a novel approach that translates them into optimized integer linear programs (ILPs) is described for computing prices.
\textcolor[rgb]{0.00,0.00,1.00}{The idea is to find the minim sum price of views that cover the query results over database.}





The pricing of aggregate queries assigns the prices to the special type of linear queries (i.e. aggregate queries that can be expressed as a linear combination of the column entries of a relationship)~\cite{li2012pricing}.
The approach is similar as~\cite{koutris2015query} in that the seller prices a base set of linear queries and then the market algorithm computes the price of the remaining queries such that it satisfies arbitrage freeness.
However, there are several crucial differences with~\cite{koutris2015query}.
First, the arbitrage freeness is based not on an \emph{instance based determinacy} relationship but rather on a \emph{schema based determinacy}: if for any instance of the database, one could determine a linear query $Q$ using the answer to a bundle of linear queries $Q_1, \cdots, Q_k$, then it must be that $p(Q) \leq \sum_{i=1}^k p(Q_i)$.
This crucial difference makes the price function independent of the database instance.
%This is a crucial property that Li et al. actually require as an axiom; if the price function were dependent on the instance then just asking for a price quote for a specific query could potentially reveal information about the database entries.
%The latter could potentially lead to manipulation by the buyers. This is the property of non-disclosive pricing introduced in Liu et al.
%It is interesting to observe that the pricing function of Koutris et al. doesn't satisfy this property and hence is potentially susceptible to such manipulations.


%\emph{Information-theoretic} determinacy, denoted $\mathbf{V}\twoheadrightarrow Q$,
%is discussed by Segoufin and Vianu~\cite{segoufin2005views} and by Nash et al.~\cite{nash2007determinacy,nash2010views}. It is a notion that is independent of the database instance.
%Their motivation comes from local-as-view data integration and semantic caching, where an instance independent rewriting is needed.


\textcolor[rgb]{0.00,0.00,1.00}{\textcolor[rgb]{1.00,0.00,0.00}{Authors in \cite{wang2018pricing}} considers a more realistic pricing scenario for aggregate query, where consumers are willing to accept the approximate aggregate query, due to the constraints on time, resources, etc.
In this setting, they propose a theoretical framework to support pricing approximate aggregate queries.
In particular, they use a sample technique to achieve an error-bounded approximate answer over data queries.
Meanwhile, a transforming function function is provided, which convert the original arbitrage-free pricing function to the one that supports approximate aggregate queries.}

The relationship between arbitrage-freeness in the query-pricing framework and envy-freeness in
pricing theory for appropriately chosen buyer valuations is studied~\cite{syrgkanis2015pricing}.
On the other hand, a formal framework for pricing queries over data allows the construction of general families of pricing functions, with the main goal of avoiding arbitrage~\cite{deep2016design}.
It considers two pricing schemes: \emph{instance-independent} schemes, where the price depends only on the structure of the query, and \emph{answer-dependent} schemes, where the price also depends on the query output.








%In addition, there are some efforts on pricing queries over data considering the privacy issue~\cite{kifer2015privacy,li2014theory,li2012adaptive,niu2018unlocking}.


\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Query Pricing based on Information Value}}

\textcolor[rgb]{0.00,0.00,1.00}{The information value based pricing model also regards the query as the structural granularity.
The price of this model can be customized according to seller's specifications.
And the difference between this model and view-based pricing is that, this pricing model prices data based on information value.}

The framework \textsc{Qirana}~\cite{deep2017qirana,deep2017qirana-d}, standing the viewpoint of the data buyer, employs the \emph{possible world} semantic to price relational queries.
\textcolor[rgb]{0.00,0.00,1.00}{In particular, \textsc{Qirana} think that, the data buyer can remove any possible database $\mathscr{D}$ that $Q(\mathscr{D}) \neq Q(D)$, thus the possible databases shrink, and data buyer learn more information about possible databases.
Hence, \textsc{Qirana} assigns a price to $Q$, which can be formulated as a function of how the possible databases shrinks.
This price reflects only the value of the information learned by obtaining the query answer, and we category it as the information value based pricing model.
Since it is infeasible to keep track of all the possible databases, it attempts to circumvent this issue by leveraging the \emph{support set} $\mathcal{S}$ (via sampling methods).
Specifically, it employs a random neighborhood sampling method, to better generate the \emph{support set} $\mathcal{S}$.}

\textcolor[rgb]{0.00,0.00,1.00}{
It also proposes several pricing functions, including weighted coverage pricing, uniform entropy gain pricing, Shannon entropy. etc.
It utilizes the \emph{weighted coverage} pricing function by default, and acts as a \emph{broker} between the buyer and the seller.
The comparison of the proposed pricing functions is discussed in detail.
Moreover, \textsc{Qirana} can support the case that some price points $\left(\mathbf{Q}_{j}, p_{j}\right)$ are specified, by solving a entropy maximization problem.
Furthermore, \textsc{Qirana} optimizes the pricing computations, in order to support history-aware pricing, batch updates, and aggregation.
As a result, a pricing system for efficiently implementing a data marketplace is developed.}



%The studies on query pricing we introduced before aim to build a framework in theory and practice, ensuring the arbitrage-freeness of pricing functions.
%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Revenue maximization for query pricing.}
\textcolor[rgb]{0.00,0.00,1.00}{Then \cite{chawla19revenue} first identifies the revenue maximization aspect of query pricing.
Inspired by existing work~\cite{deep2017qirana,deep2017qirana-d}, the pricing functions are based on the information value, leveraging the concept of \emph{support set} $\mathcal{S}$.
Specifically, they conduct a hypergraph  $\mathcal{H}=(\mathcal{V}, \mathcal{E}),$ with vertex set $\mathcal{V}=\mathcal{S},$ and hyperedges $\mathcal{E}=\left\{e_{i} \mid i=1, \ldots, m\right\},$ where $e_{i}=\mathcal{C}_{S}\left(\mathbf{Q}_{i}, \mathcal{D}\right) .$ and $\mathcal{C}_{S}$ is the conflict set of $\mathbf{Q}_{i}$ with respect to $\mathcal{S}$.
They cast the revenue maximization task as bundle pricing problem for single-minded buyers and unlimited supply, and propose several simple pricing functions, including unform bundle pricing, item pricing, and $XOS$ pricing.
In particular, unform bundle pricing assigns same price to every hyperedge, while item pricing computes price as the weight sum of vertex in the hyperedge, and $XOS$ pricing uses the max weight of vertex in the hyperedge.
Then they also present some approximation algorithms, in order to efficiently deriving the optimal price.}


\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Query Pricing using Data Provenance}}
\label{subsubsec:provenance-model}

The DBP model using data provenance considers the tuples of relations as the structural granularity of the pricing function, and is based on the data provenance, i.e., the set of the tuples contributing to the result tuples of a {\color{blue}query~\cite{tang2013you,tang2013price,upadhyaya2016price}}.
In other words, the seller places prices on tuples of the database and then the price of a query is a function of the tuples that contribute to the response of the query.

\emph{Provenance} information describes the origin and the history of data in its life cycle.
Cui et al.~\cite{cui2000tracing} are among the first to formalize a notion of provenance, of data in the context of relational databases, called \emph{lineage}. Each tuple $t$  occurs  in the output of a query with a set of tuples presented in the input, called the lineage of $t$. Intuitively, the lineage of $t$ is meant to collect all of the input data that ``contribute to'' $t$ or help to ``produce'' $t$.
As discussed in some studies~\cite{balazinska2011data,green2007provenance,green2017semiring}, the pricing scheme based on provenance is captured elegantly in the framework of provenance semirings: \textcolor[rgb]{1.00,0.00,0.00}{ the price semiring is ($\mathbb{R}^{\infty}_+, \min, +, \infty, 0$)}.
The concept of the lineage set is stated in Definition~\ref{defn:min-lineage-tuple}.














\begin{definition}\label{defn:min-lineage-tuple}
{\bf (Result tuple's lineage set)}.
Given a database $D$ with tables $T_1, \cdots, T_m$,  and a relational operator $Q$.
Let $Q(D)$ = $Q(T_1, \cdots, T_m)$ be the result set of the query $Q$ over tables $T_1, \cdots, T_m$.
For a tuple $t\in Q(D)$, one  $t$'s lineage set w.r.t. $Q$  in $T_1, \cdots, T_m$, denoted as $L(t\in Q(D), D)$ $(L(t, D)$ for short$)$, is defined by Eq.~\ref{eq:minimal-tuple-lineage}.
\begin{equation}\label{eq:minimal-tuple-lineage}
L(t, D) = \bigcup_{i=1}^m T^*_i
\end{equation}
\begin{equation}
\centering
\label{eq:tuple-lineage-vector}
Q^{-1}_{\langle T_1, \cdots, T_m\rangle}(t) = \langle T^*_1, \cdots, T^*_m\rangle
\end{equation}
\noindent
where $Q^{-1}_{\langle T_1, \cdots, T_m\rangle}(t)$ $= \langle T^*_1, \cdots, T^*_m\rangle$ is the vector form of a lineage set of $t$, with each element $T^*_i$ having tuples from the table $T_i$. It is said that $Q^{-1}_{T_i}(t) =  T^*_i$ is $t$'s lineage in $T_i$, and each tuple in $T^*_i$ contributes to the result tuple $t$, for $i = 1, \cdots, m$. In particular, $T^*_1, \cdots, T^*_m$ are subsets of $T_1, \cdots, T_m$, such that:

(a) $Q(T^*_1,$ $\cdots,$ $T^*_m)$ $= \{t\}$;

(b) $\forall T^*_i, \forall T^{'}\subseteq T^*_i, Q(T^*_1,$ $\cdots,$ $T^{'}, \cdots, T^*_m) =  \varnothing$;

\end{definition}

The  requirements (a) and (b) in Definition \ref{defn:min-lineage-tuple} follows the explanations in~\cite{cui2000practical,cui2000tracing}: ``The requirement (a)  means that lineage tuple sets (i.e., $T_i^*$'s) derive exactly $t$. From relational semantics, we know that, for any result tuple $t$, there must exist such tuple sets.
The requirement (b) indicates that each tuple in the lineage does indeed contribute something to $t$.''


%\begin{table}[t]\footnotesize
%	\centering
%		\caption{A Sample Database of an Online Shopping System}\label{tab:sample}%\vspace*{-0.1in}
%\setlength{\tabcolsep}{20pt}
%\centering%\small
%\begin{tabular}{p{15pt}p{15 pt}p{35 pt}p{15 pt}}
%\toprule[0.7pt]%\rowcolor{pink}
%\textbf{Pid} & \textbf{Size}  & \textbf{Memory} & \textbf{Price}\\
%\midrule[0.3pt]
%$p_1$ & 4.7 & 64 & \$5988 \\
%$p_2$ & 4.7 & 256 & \$7288 \\
%$p_3$ & 5.5 & 64 & \$6888 \\
%$p_4$ & 5.5 & 256 & \$8188 \\ \bottomrule[0.7pt]
%\end{tabular}
%\end{table}
%
%
%
%
%
%
%
%\begin{example}\label{exa:lineage}
%For the sample dataset (denoted by $D_1$) in Table~\ref{tab:sample}  which records four products (i.e., smart phones), in terms of the projection query $Q^{\pi}$ (\texttt{ SELECT  DISTINCT Size  FROM $D_1$}),  its result tuples are $\{$`4.7', `5.5'$\}$.
%According to Definition~\ref{defn:min-lineage-tuple}, the result tuple `4.7' has two lineage sets, i.e.,   $\{p_1\}$ and  $\{p_2\}$, both of which can produce the tuple `4.7'.
%Similarly, for the result tuple `5.5', it has two  lineage sets, namely $\{p_3\}$ and  $\{p_4\}$. Consequently, %according to Definition~\ref{defn:lineage},
%there are four  lineage sets for the query $Q_5^{\pi}$ including $\{p_1, p_3\}$,  $\{p_1, p_4\}$, $\{p_2, p_3\}$, and $\{p_2, p_4\}$.
%\end{example}


As a consequence, based on the query lineages, the data pricing model is developed to accumulate the prices of the query lineage {\color{blue}tuples \cite{ruiming2014quality,tang2013price}}.  The proposed model fulfills desirable properties such as contribution monotonicity, bounded-price and contribution arbitrage-freedom.
\textcolor[rgb]{0.00,0.00,1.00}{Moreover, the pricing framework is extended to support query pricing for probabilistic databases.
In particular, the concept of lineage set is updated, and the price of probabilistic tuple is redefined.
To summarize, this pricing model employs the idea of data usage, and price data based on the tuples that contribute to the query.}





\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Query Pricing with Query Cost}}
\label{subsubsec:db-cost}
\textcolor[rgb]{0.00,0.00,1.00}{The pricing model using \emph{query cost} considers the query resource consumption into pricing issues, which takes the query as the structural granularity in pricing function.
The difference between this category and above studies is that, above studies in query pricing have an implicit assumption, where the queries over data can be seen as unlimited supply.
In contrast, the idea of this category is that, queries over data need inevitable cost, such as time and resource, thus they are limited. }


\textcolor[rgb]{0.00,0.00,1.00}{Wang et al. propose an auction-based query pricing scheme based on query cost \cite{wang2019novel}.
The differences between this work and above studies are mainly two aspects.
One is the limited supply of queries, and another is that, it does not support customizing the price, since it is an auction mechanism while above studies are based on post pricing.
It first uses query plan generation technique, to compute the execution time and resource demands.
Then based on the query cost, it designs an auction to trade query, where the information value is reflected by consumers' bids and resource provisioning represents computational cost.
It formulates a social welfare maximization problem, and proposes a dual linear programming problem to solve it.
Moreover, it designs a greedy primal dual algorithm, which is available in bothe offline scenarios and online scenarios.
To summarize, this is the first pricing schema, which prices query based on query cost, and incorporates it with auction mechanism, which is totally different from above studies. }

%which is totally different from above studies

%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Auction-based query pricing.}
%\cite{wang2019novel} proposes an auction-based query pricing algorithm, which is different from existing work.
%They consider the execution time and resource demands of query, and present a social welfare maximization problem under auction mechanism.
%To solve the NP-hard problem, they cast the query auction design into an integer linear programming problem, and design a primal-dual algorithm.
%Based on that, they obtain the price of each winning bids.}

\subsection{Personal Data Pricing}
\label{subsec:dbpdata-model}

\textcolor[rgb]{0.00,0.00,1.00}{
The amount of data in our world is increasing at an amazing speed, and personal data accounts for a large part of it.
For instance, Facebook collected 300 petebytes of personal data in 2014~\cite{vagata2014scaling}.
While people reap the benefits of data-driven society, there is a growing public concern about data privacy.
Due to the critical privacy concern, personal data is difficult to share and use directly.
However, data market is an important way to bridge the gap between data owners and data consumers, in order to promote personal data circulation.
Thus, the pricing problem of personal data has been widely explored~\cite{li2014theory,li2017theory,niu2019making,niu2018unlocking,niu2019erato,niu2020online} .
We divide them into two categories, i.e., pricing personal data with privacy and pricing personal data with market value.}

\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Personal Data Pricing using Privacy}}
\label{subsubsec:db-privacy}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{pdata.eps}
	\caption{Pricing Personal Data Framework with Privacy~\cite{li2014theory,li2017theory,niu2019making,niu2018unlocking,niu2019erato}}%from Pricing Approaches for Data Markets
	\label{fig:PData}
	%\vspace{-1.5em}
\end{figure}

%In the context of data pricing problem, a typical kind of data, i.e., personal data, has become a new asset in real world~\cite{pdata}.




%Recent studies~\cite{li2014theory,li2017theory,niu2018unlocking,niu2019making,niu2018achieving,niu2019erato} have been proposed to solve above problems, which build a pricing framework, as shown in Figure~\ref{PData basics}.
\textcolor[rgb]{0.00,0.00,1.00}{
Li et al. ~\cite{li2014theory,li2017theory} first studied the pricing problem of private data , and proposed a theoretical framework, as shown in Figure~\ref{fig:PData}.
Similar with existing data markets, the pricing framework includes three parts, i.e., data owner, data broker, and data consumer.
The data broker is an intermediary agent between data owners and data consumers, which deal with the request from data consumer, determine monetary compensation of data owner, return the noisy answer to data consumer, and price the answer.
In particular, the request from data consumer can formed as $S=(\mathbf{q}, v)$, where $\mathbf{q}$ can be seen as a function that outputs some aggregate statistics, such as linear aggregate query, histogram count, weighted sum, mean, standard deviation, etc.
Note that, $\mathbf{q}$ does not return the raw data (like traditional SQL query does), since the original data is sensitive.
$v$ is the tolerable variance of noise added to the true answer.
Once the data broker receives the request, he/she not only needs to return the noisy answer, but also has to derive the price and privacy compensation.}

\textcolor[rgb]{0.00,0.00,1.00}{
Li et al. introduced the critical item in pricing problem, namely, arbitrage-free functions and privacy loss of data owner.
They proved that, pricing functions $\pi(\mathbf{q}, v)$ following these properties are arbitrage-free.}

\begin{proposition}
\textcolor[rgb]{0.00,0.00,1.00}{Any arbitrage-free pricing function $\pi(\mathbf{q}, v)$ satisfies the following properties,  where $\mathbf{q}$ refers to data analysis method that produces output, and $v$ is the noise level.}

\noindent
$(i)$ The zero $\mathbf{q}$ is free: $\pi(\mathbf{q}, v)=0$.

\noindent$(ii)$ Higher variance is cheaper: $v \leq v^{\prime}$ implies $\pi(\mathbf{q}, v) \geq \pi(\mathbf{q}, v^{\prime}) $.

\noindent$(iii)$ The zero-variance $\mathbf{q}$ is the most expensive: $\pi(\mathbf{q}, 0) \geq \pi(\mathbf{q}, v) \text { for all } v \geq 0$

\noindent$(iv)$ Infinite noise is free: if $\pi$ is continuous at $\mathbf{q}=0,$ then $\pi(\mathbf{q}, \infty)=0$.

\noindent$(v)$ As $v \rightarrow \infty, \pi(\mathbf{q}, v)=\Omega(1 / v)$.
\end{proposition}

%\begin{enumerate}
%  \item The zero $\mathbf{q}$ is free: $\pi(\mathbf{q}, v)=0$
%  \item Higher variance is cheaper: $v \leq v^{\prime}$ implies $\pi(\mathbf{q}, v) \geq \pi(\mathbf{q}, v^{\prime}) $
%  \item The zero-variance $\mathbf{q}$ is the most expensive: $\pi(\mathbf{q}, 0) \geq \pi(\mathbf{q}, v) \text { for all } v \geq 0$
%  \item Infinite noise is free: if $\pi$ is continuous at $\mathbf{q}=0,$ then $\pi(\mathbf{q}, \infty)=0$.
%  \item As $v \rightarrow \infty, \pi(\mathbf{q}, v)=\Omega(1 / v)$.
%\end{enumerate}
\textcolor[rgb]{0.00,0.00,1.00}{Note that, this proposition is different from that in Proposition~\ref{pro:free-qpricing}, as it considers the variable noise $v$.
The last property ensures that, the pricing function cannot decrease faster than 1/$v$.
Thus, the data consumer cannot purchase $(\mathbf{q}, v)$ with lower price by combining a series of $(\mathbf{q}, v_{i})$ when $\frac{1}{m} \sum_{i=1}^{m} v_{i} \leq v$.}
\textcolor[rgb]{0.00,0.00,1.00}{
\begin{definition}\label{defn:indi-privacy-loss}
{\bf (Individual Privacy Loss)}.
The privacy loss of the data owner $i$ in the randomized mechanism $\mathcal{M}$ over the database $\mathbf{x}$ is defined as:
\begin{equation}
\epsilon_{i}(\mathcal{M})=\sup _{\mathbf{x}, O}\left|\log \frac{P(\mathcal{M}(\mathbf{x})=O)}{P\left(\mathcal{M}\left(\mathbf{x}^{(i)}\right)=O\right)}\right|
\end{equation}
\noindent
where $\mathbf{x}$ ranges over all possible database instances, and $O$ ranges over all possible outputs.
\end{definition}}
\textcolor[rgb]{0.00,0.00,1.00}{Besides, the individual privacy loss is formulated based on differential privacy.
In particular, a mechanism $\mathcal{M}$ is differential privacy if the probability of a specific output $O$ on any neighboring database is almost the same, i.e., the output $O$ is hard to distinguish.
As a result, the individual privacy loss can be introduced as Definition~\ref{defn:indi-privacy-loss}. One can find that, it is the deformation of differential privacy, which considers the neighboring databases by varying the data from owner $i$.
Thus, the structural granularity can be seen as the tuple, since the privacy loss of individual is considered.
The above study determines the basic framework of personal data pricing, laying the foundation for follow-up work.
However, the specific form of the price function and the feasible privacy compensation strategy have not been determined.}


%To make personal data trade more feasible, several critical problems have to take into consideration.
%On one hand, one problem is how to quantify the monetary compensation, in order to incentivize data owners/providers to contribute their private data.
%Another problem is the price of personal data concerning the privacy loss of data owners or providers.
%\begin{property}\label{prop:arbitrage-free-pdata}
%{111}
%\end{property}
%
%Following \cite{li2014theory,li2017theory}, Niu et al. then introduce the privacy compensation function, and the arbitrage-free pricing function, which leads personal data pricing more practical via a framework called \emph{ERATO}

\textcolor[rgb]{0.00,0.00,1.00}{Following \cite{li2014theory,li2017theory}, Niu et al.~\cite{niu2018unlocking,niu2019erato} then introduce a more practical framework \textsc{Erato}, including the specific privacy compensation function, and the arbitrage-free pricing function.
Specifically, they choose Laplace mechanism to guarantee $\epsilon$-dependent differential privacy.
Meanwhile, they design arbitrage-free pricing functions based on the above property, where the noisy answer of $\mathbf{q}$ is regarded as random variables with expectation $\mathbf{w}^{T} \mathbf{x}$, and the determinacy relation is given.
As for privacy compensation, they first find the bound of the privacy loss of each data owner $i$, and design privacy compensation functions based on the bound.
In particular, the compensation can also been allocated when a total compensation is $B$, which is called a top-down design.
Numerous experiments have been conducted to demonstrate the feasibility of \textsc{Erato}.}


%as an example, it aims to trade time-series data.
%evaluates the max-influence of the state $X_t$ on a set of ¡°remote¡± states $X_M$
\textcolor[rgb]{0.00,0.00,1.00}{Niu et al.~\cite{niu2019making} also make the framework applicable on time-series private data, and propose a framework \textsc{Horae}.
First, \textsc{Horae} employs Pufferfish privacy to quantify privacy losses under temporal correlations, and compensates data owners with distinct privacy strategies in a satisfying way.
Specifically, \textsc{Horae} offers a mechanism $\mathcal{M}$ under Pufferfish privacy, and give an upper bound of the privacy loss of the data owner.
Based on the privacy loss, \textsc{Horae} provides several valid privacy compensation functions, and prices the query by the balanced and valid pricing function.
Besides, \textsc{Horae} not only guarantees good profitability at the data broker, but also ensures arbitrage freeness against cunning data consumers.
Furthermore, the experiments on real dataset proves that, \textsc{Horae} is feasible to price time-series personal data, which not only has the ability to avoid arbitrage attacks, but also can control the profit radio.}

\textcolor[rgb]{1.00,0.00,0.00}{Demo 112 2018 VPLDB}

\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Personal Data Pricing
with Market Value}}
\label{subsubsec:db-pmarket}
\textcolor[rgb]{0.00,0.00,1.00}{This kind of pricing model is different from the pricing models concerning privacy, since it models the market value of data as a function, and prices data in an online fashion.
Also, the goal of this model is to minimize the regret during the ongoing transaction, which is quite different from pricing model with privacy.}

\textcolor[rgb]{0.00,0.00,1.00}{We first introduce what the market value of product is, inspired by the existing feature based pricing work~\cite{cohen2016feature}.
In particular, the market value can be formulated as follows.}

\begin{definition}\label{defn:market-value-goods}
{\bf (Market Value of Product)}.
The market value of product in the feature based pricing setting $v_t$ is defined as:
\begin{equation}
v_t = f\left(\mathbf{x}_{t}\right)+\delta_{t}
\end{equation}
\noindent
where $\mathbf{x}_{t}$ is the feature of product, $f\left(\mathbf{x}_{t}\right)$ is the mapping function from feature vector $\mathbf{x}_{t}$ to the deterministic part in market value, and $\delta_{t}$ models the uncertainty in market value.
\end{definition}

\textcolor[rgb]{0.00,0.00,1.00}{One can find that, the price of each product relies on its feature.
Hence, the structural granularity in this model can be varied in different levels of data, which depends on the level of feature.}

\textcolor[rgb]{0.00,0.00,1.00}{Since the knowledge of market values is limited, the data broker can only passively receive each product request $\mathbf{q}_t$, and then post a price $p_t$.
When the posted price is no more than the market value, i.e., $p_{t} \leq v_{t}$, the data broker can earn a revenue.
Thus, a revenue maximization problem is produced.
Cohen et al.~\cite{cohen2016feature} translate the above problem to a regret minimization problem.
And then they approximates the polytope-shaped knowledge set with ellipsoid, and provided a worst-case regret of $O\left(n^{2} \log T\right)$, which is essentially the pure version of pricing mechanism in \cite{niu2020online}.
Furthermore, \cite{niu2020online} incorporates \cite{cohen2016feature} with personal data pricing, which models $x_{t}$ as the privacy feature of a request $\mathbf{q}$, and considers the reserve price constraint.
In the context of personal data pricing, the differentiated products $\mathbf{q}_t$ can be seen as the request of data consumer in Figure~\ref{fig:PData}, i.e., the concrete statistic and tolerable level of noise, and the features can be obtained by the privacy compensation and other technology.
Extensive experiments demonstrate that, it is feasible to apply existing online pricing technology to personal data pricing.}
\textcolor[rgb]{1.00,0.00,0.00}{Support non-linear cases}

%The market value quantify the valuation of consumers in market.
%\textbf{Online pricing for personal data.}
%\cite{niu2020online} introduces online pricing into personal data pricing.
%Specifically, it employs the idea of feature based pricing \cite{cohen2016feature}, which regards the value of products $v_{t}$ as sum of market value $f\left(\mathbf{x}_{t}\right)$ with respect feature $x_{t}$  and uncertainty $\delta_{t}$.
%In particular, $f\left(\mathbf{x}_{t}\right)$ can be modelled as a linear function, i.e., $f\left(\mathbf{x}_{t}\right)=\theta x_{t}$.
%And the revenue maximization problem is translated to be a regret minimization problem.
%\cite{cohen2016feature} approximates the polytope-shaped knowledge set with ellipsoid, and provided a worst-case regret of $O\left(n^{2} \log T\right)$, which is essentially the pure version of pricing mechanism in \cite{niu2020online}.
%Furthermore, \cite{niu2020online} incorporates \cite{cohen2016feature} with personal data pricing, which models $x_{t}$ as the privacy feature of a request $\mathbf{q}$, and considers the reserve price constraint.
%Extensive experiments demonstrate that, it is feasible to apply existing online pricing technology to personal data pricing.

%\input{sn-model}

%\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Market-oriented Pricing in Database}}
%\label{subsubsec:db-market}
%\textcolor[rgb]{0.00,0.00,1.00}{In this part, we introduce the market-oriented pricing methods in database field, including revenue maximization for query pricing, auction-based query pricing, and online pricing for personal data.
%As some basic concepts are introduced before, thus we simply summarize the main idea of each pricing scheme.}
%
%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Revenue maximization for query pricing.}
%The studies on query pricing we introduced before aim to build a framework in theory and practice, ensuring the arbitrage-freeness of pricing functions.  \cite{chawla19revenue} first identifies the revenue maximization aspect of query pricing.
%Inspired by existing work~\cite{deep2017qirana,deep2017qirana-d}, the pricing functions are based on \emph{support set} $\mathcal{S}$.
%Specifically, they conduct a hypergraph  $\mathcal{H}=(\mathcal{V}, \mathcal{E}),$ with vertex set $\mathcal{V}=\mathcal{S},$ and hyperedges $\mathcal{E}=\left\{e_{i} \mid i=1, \ldots, m\right\},$ where $e_{i}=\mathcal{C}_{S}\left(\mathbf{Q}_{i}, \mathcal{D}\right) .$ and $\mathcal{C}_{S}$ is the conflict set of $\mathbf{Q}_{i}$ with respect to $\mathcal{S}$.
%They cast the revenue maximization task as bundle pricing problem for single-minded buyers and unlimited supply, and propose several simple pricing functions, including unform bundle pricing, item pricing, and $XOS$ pricing.
%In particular, unform bundle pricing assigns same price to every hyperedge, while item pricing computes price as the weight sum of vertex in the hyperedge, and $XOS$ pricing uses the max weight of vertex in the hyperedge.
%Then they also present some approximation algorithms, in order to efficiently deriving the optimal price.}
%
%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Auction-based query pricing.}
%\cite{wang2019novel} proposes an auction-based query pricing algorithm, which is different from existing work.
%They consider the execution time and resource demands of query, and present a social welfare maximization problem under auction mechanism.
%To solve the NP-hard problem, they cast the query auction design into an integer linear programming problem, and design a primal-dual algorithm.
%Based on that, they obtain the price of each winning bids.}
%
%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Online pricing for personal data.}
%\cite{niu2020online} introduces online pricing into personal data pricing.
%Specifically, it employs the idea of feature based pricing \cite{cohen2016feature}, which regards the value of products $v_{t}$ as sum of market value $f\left(\mathbf{x}_{t}\right)$ with respect feature $x_{t}$  and uncertainty $\delta_{t}$.
%In particular, $f\left(\mathbf{x}_{t}\right)$ can be modelled as a linear function, i.e., $f\left(\mathbf{x}_{t}\right)=\theta x_{t}$.
%And the revenue maximization problem is translated to be a regret minimization problem.
%\cite{cohen2016feature} approximates the polytope-shaped knowledge set with ellipsoid, and provided a worst-case regret of $O\left(n^{2} \log T\right)$, which is essentially the pure version of pricing mechanism in \cite{niu2020online}.
%Furthermore, \cite{niu2020online} incorporates \cite{cohen2016feature} with personal data pricing, which models $x_{t}$ as the privacy feature of a request $\mathbf{q}$, and considers the reserve price constraint.
%Extensive experiments demonstrate that, it is feasible to apply existing online pricing technology to personal data pricing.}

\subsection{\textcolor[rgb]{0.00,0.00,1.00}{Quality-based Data Pricing}}
\label{subsec:db-quality}

\textcolor[rgb]{0.00,0.00,1.00}{Since the true value of data is hard to obtain, several studies aim to price data based on its intrinsic value, i.e., data quality.
Following this idea, there are two kinds of pricing models, including relational data pricing based on accuracy and XML data pricing based on  completeness.}

\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{Relational Data Pricing based on Accuracy}}
\label{subsec:db-accuracy}

\textcolor[rgb]{0.00,0.00,1.00}{This model prices data in a tuple granularity, and the price of tuple relies on data accuracy.
Different from aforementioned models, this model first receives tuple that data consumers want to purchase and the price he/she can accept.
Thus, the behind idea of this model is called ``what you pay for is what you get''.}

\textcolor[rgb]{0.00,0.00,1.00}{A theoretical and practical pricing framework~\cite{tang2013you} is proposed, in order to trade data quality (more specifically, data accuracy) for discounted prices.
In the framework, tuple value answered to data consumer is determined by the full price of tuple and the consumer bid.
The tuple provided to a data consumer is exact if he/she offers the full price for it.
Otherwise, the value of tuple is approximate when he/she offers to pay only a discounted price.
The lower the price is, the more inaccurate the answer.
In particular, the distribution of exact tuple is modelled as a degenerate distribution.
For example, if the tuple value is 1, and the possible value is ${1,2,3,4}$, then the degenerate distribution can be formed as $(1,0,0,0)$.
In the case of a discounted price, the inaccurate tuple value is randomly determined from a probability distribution.
And the distance of the distribution to the actual value (to the degenerate distribution) is measured through earth mover¡¯s distance(EMD), which is commensurate to the discount.
Meanwhile, the published value comes with a guarantee on its probability, which is also commensurate to the discount.
Ancillary pricing functions are defined to facilitate the necessary algorithms under several principles.}


%\textcolor[rgb]{0.00,0.00,1.00}{In order to trade data quality for discounted prices, a theoretical and practical pricing framework~\cite{tang2013you} is proposed.
%The answer from model is determined by the full price of tuple and the consumer bid.
%In the framework, the data provided to a data consumer is exact if she offers the full price for it. The data is approximate if she offers to pay only a discounted price. In the case of a discounted price, the value of data is randomly determined from a probability distribution.
%The distance of the distribution to the actual value (to the degenerate distribution) is commensurate to the discount. The published value comes with a guarantee on its probability. The probability is also commensurate to the discount. Ancillary pricing functions are defined to facilitate the necessary algorithms under several principles.
%(more specifically, data
%accuracy)
%The structual granu}


\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{XML Data Pricing based on  Completeness}}
\label{subsec:db-completeness}
\textcolor[rgb]{0.00,0.00,1.00}{Similar with relational data pricing model based on accuracy, this model also employs the idea of ``what you pay for is what you get''.
When consumer offers a price, this pricing model provides him an incomplete XML data.
Since XML data is formed as a tree, the granularity of pricing is the tree produced by XML data.}

\textcolor[rgb]{0.00,0.00,1.00}{Tang et al. explore a pricing framework~\cite{tang2014get} for XML data, which data quality can be traded for a discount.
It considers the case of XML documents with completeness as the quality dimension.
To be more specific, the completeness is defined as the weight ratio between the full tree and answered tree.
Thus, a sampling problem is derived, in order to find the subtree satisfies the weight, which is related to the discount price.
Then they identify the tractable cases in this problem, and provide PTIME solutions.
The situation where consumers have repeated requests is also considered.}
%
%\textcolor[rgb]{0.00,0.00,1.00}{For XML data which data quality can be traded for a discount, a pricing framework~\cite{tang2014get} is explored.
%It considers the case of XML documents with completeness as the quality dimension.
%Namely, a data provider offers an XML document, and sets both the price and weights of nodes of the document.
%The data consumer proposes a price but may get only a sample if the proposed price is lower than that of the entire document.}


\subsubsection{\textcolor[rgb]{0.00,0.00,1.00}{XML Data Pricing based on  Completeness}}
\label{subsec:db-completeness}
\textcolor[rgb]{0.00,0.00,1.00}{Similar with relational data pricing model based on accuracy, this model also employs the idea of ``what you pay for is what you get''.
When consumer offers a price, this pricing model provides him an incomplete XML data.
Since XML data is formed as a tree, the granularity of pricing is the tree produced by XML data.}

\textcolor[rgb]{0.00,0.00,1.00}{Tang et al. explore a pricing framework~\cite{tang2014get} for XML data, which data quality can be traded for a discount.
It considers the case of XML documents with completeness as the quality dimension.
To be more specific, the completeness is defined as the weight ratio between the full tree and answered tree.
Thus, a sampling problem is derived, in order to find the subtree satisfies the weight, which is related to the discount price.
Then they identify the tractable cases in this problem, and provide PTIME solutions.
The situation where consumers have repeated requests is also considered.}

\subsection{\textcolor[rgb]{0.00,0.00,1.00}{Comparison and Summarization}}
\label{subsec:db-sum}

%
%    \begin{tabular}{|p{5.5em}|p{6.8em}|p{6.8em}|p{6.8em}|p{6.8em}|p{6.8em}|p{6.8em}|}
%    \hline
%    \textbf{Category} & \multicolumn{4}{c|}{Query pricing}       & \multicolumn{2}{c|}{Personal data pricing} \bigstrut\\
%    \hline
%    \textbf{Name} & Pricing with data view & Pricing with information value & Pricing using data provenance & Pricing using query cost & Pricing personal data with privacy & Pricing personal data with market value \bigstrut\\
%    \hline
%    \textbf{Required setting} & Price points & Price points (not necessary) & Price of tuples  & None  & None  & Price feature extraction \bigstrut\\
%    \hline
%    \textbf{Pricing perspective} & Minim cover price & Data information value & Data usage & Query cost & Data privacy & Data market value \bigstrut\\
%    \hline
%    \textbf{Goal} & price any query & price any query & price any query/ revenue maximiation & social welfare maxmization & price personal data & Regret minimization \bigstrut\\
%    \hline
%    \textbf{Technology} & Intege linear programming & Support set, conflict set, etc. & Lineage set. & Intege linear programming & Differential privacy and laplace mechanism & L¡§owner-John ellipsoid \bigstrut\\
%    \hline
%    \textbf{Service} & Support SPJ query &       & Support SPJ query &       & Support aggregate statistics and optional nosie level & Support learning the market value \bigstrut\\
%    \hline
%    \textbf{Arbitrage} & No    & No    & No    & N/A   & No    & N/A \bigstrut\\
%    \hline
%    \textbf{Mechanism} & Post pricing & Post pricing & Post pricing & Auction & Post pricing & Online pricing \bigstrut\\
%    \hline
%    \textbf{Market} & No    & Yes   & No    & Yes   & No    & Yes \bigstrut\\
%    \hline
%    \end{tabular}%

\begin{table*}[tbp]
%\footnotesize
  \setlength{\tabcolsep}{3pt}
  \centering
  \caption{Comparison of Existing Data Pricing Models in Database}
    \begin{tabular}{|p{7.5em}<{\centering}|p{2em}<{\centering}|p{9em}<{\centering}|p{7em}<{\centering}|p{10.5em}<{\centering}|p{3em}<{\centering}|p{1.8em}<{\centering}|p{1.8em}<{\centering}|}
    \hline
    \textbf{Ref.} & \textbf{Cat.} & \textbf{Perspective} & \textbf{Requirements} & \textbf{Technique} & \textbf{Mech.} & \textbf{Arb.} & \textbf{Mkt.} \\
    \hline
     \cite{koutris2012querymarket,koutris2013toward,li2012pricing,koutris2015query,wang2018pricing} & QP    &  Price inference & Price points  & ILP & PP & $\times$    & $\checkmark$ \\
    \hline
     \cite{chawla19revenue,deep2017qirana,deep2017qirana-d} & QP    & Information value & Optional & Sampling & PP & $\times$    & $\checkmark$ \\
    \hline
     \cite{ruiming2014quality,tang2013price} & QP    & Data usage & Tuple price  & Query lineage & PP & $\times$    & $\times$ \\
    \hline
     \cite{wang2019novel} & QP    &  Query cost & /  & ILP & Auction & $\bigcirc$   & $\checkmark$ \\
    \hline
     \cite{li2014theory,li2017theory,niu2019making,niu2018unlocking,niu2019erato} & PDP   &  Data privacy  & /  & Differential privacy & PP & $\times$    & $\times$ \\
    \hline
    \cite{niu2020online} & PDP    & Market value & Price feature & L$\ddot{\text{o}}$wner-John ellipsoid & OP & $\bigcirc$   & $\checkmark$ \\
    \hline
     \cite{tang2013you} & QDP   & Data accuracy & Basic price & Sampling & IP & $\bigcirc$   & $\times$ \\
    \hline
     \cite{tang2014get} & QDP   & Data completeness & Basic price & Sampling & IP & $\times$   & $\times$ \\
    \hline

    \end{tabular}%
    \label{tab:pricing-dbmodels}
\end{table*}%

%    \begin{tabular}{|p{5em}|p{6em}|p{5.5em}|p{5.5em}|p{5.5em}|p{5.5em}|p{5em}|p{5em}|}
%    \hline
%    \multicolumn{2}{|c|}{\textbf{Pricing Models }} & \multicolumn{1}{c|}{\textbf{Required}} & \multicolumn{1}{c|}{\textbf{Pricing}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Technology}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Mechanism}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Arbitrage}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Market}}} \bigstrut\\
%    \cline{1-2}\multicolumn{1}{|p{5em}|}{\textbf{Category}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{setting}} & \multicolumn{1}{c|}{\textbf{perspective}} &       &       &       & \\
%    \hline
%    QP    & Pricing with data view & Price points & Minim cover price & Intege linear programming & Post pricing & No    & No \\
%    \hline
%    QP    & Pricing with information value & Price points (not necessary) & Data information value & Support set, conflict set, etc. & Post pricing & No    & Yes \bigstrut\\
%    \hline
%    QP    & Pricing using data provenance & Price of tuples  & Data usage & Lineage set. & Post pricing & No    & No \bigstrut\\
%    \hline
%    QP    & Pricing using query cost & None  & Query cost & Intege linear programming & Auction & N/A   & Yes \bigstrut\\
%    \hline
%    PDP   & Pricing personal data with privacy & None  & Data privacy & Differential privacy and laplace mechanism & Post pricing & No    & No \bigstrut\\
%    \hline
%    PDP   & Pricing personal data with market value & Price feature extraction & Data market value & L¡§owner-John ellipsoid & Online pricing & N/A   & Yes \bigstrut\\
%    \hline
%    \end{tabular}%

% Table generated by Excel2LaTeX from sheet 'Sheet6'
%\begin{table*}[tbp]
%  \centering
%  \caption{Add caption}
%    % Table generated by Excel2LaTeX from sheet 'Sheet6'
%    % Table generated by Excel2LaTeX from sheet 'Sheet6'
%    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
%    \hline
%    \multicolumn{2}{|c|}{\textbf{Pricing Models }} & \multicolumn{1}{p{4.25em}|}{\textbf{Required}} & \multicolumn{1}{p{4.815em}|}{\textbf{Pricing}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Goal}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Technology}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Service}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Arbitrage}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Mechanism}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Market}}} \bigstrut\\
%    \cline{1-2}\textbf{Category} & \textbf{Name} & \multicolumn{1}{c|}{\textbf{setting}} & \multicolumn{1}{c|}{\textbf{perspective}} &       &       &       &       &       &  \bigstrut\\
%    \hline
%    QP    & Pricing with data view & Price points & Minim cover price & price any query & Intege linear programming & Support SPJ query & No    & Post pricing & No \bigstrut\\
%    \hline
%    QP    & Pricing with information value & Price points (not necessary) & Data information value & price any query & Support set, conflict set, etc. &       & No    & Post pricing & Yes \bigstrut\\
%    \hline
%    QP    & Pricing using data provenance & Price of tuples  & Data usage & price any query/ revenue maximiation & Lineage set. & Support SPJ query & No    & Post pricing & No \bigstrut\\
%    \hline
%    QP    & Pricing using query cost & None  & Query cost & social welfare maxmization & Intege linear programming &       & N/A   & Auction & Yes \bigstrut\\
%    \hline
%    PDP   & Pricing personal data with privacy & None  & Data privacy & price personal data & Differential privacy and laplace mechanism & Support aggregate statistics and optional nosie level & No    & Post pricing & No \bigstrut\\
%    \hline
%    PDP   & Pricing personal data with market value & Price feature extraction & Data market value & Regret minimization & L¡§owner-John ellipsoid & Support learning the market value & N/A   & Online pricing & Yes \bigstrut\\
%    \hline
%    \end{tabular}%
%
%
%
%
%  \label{tab:addlabel}%
%\end{table*}%



\textcolor[rgb]{0.00,0.00,1.00}{We summarize the above pricing models in database, as shown in Table~\ref{tab:pricing-dbmodels}.
In particular, several aspects of models are compared in the following.}

\textcolor[rgb]{0.00,0.00,1.00}{
\textbf{Catagory(Cat.).} As we mentioned before, we divide the pricing models into three categories, i.e., query pricing (QP), personal data pricing (PDP), quality-based data pricing (QDP).}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Perspective.} To be more specific, we introduce eight pricing models from different pricing perspective.
The pricing model with data view can be summarized as a class of pricing models, which infer the price from price of several views. And pricing using data provenance follows the idea that prices data according to data used in query. The pricing perspective is contained in the name for other pricing models, such as pricing with information value, pricing personal data with privacy, etc.}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Requirements.} The requirements are the parts that must be determined before pricing, which can be seen as necessary preparation. In particular, the pros and cons of pricing strategies do not depend on requirements. For query pricing with data view, it requires the price points specified by data sellers. The requirements of query pricing based on information value are optional, since it is feasible when there are no price points.}

\textcolor[rgb]{0.00,0.00,1.00}{For query pricing using data provenance, it requires the price setting of tuple, in order to derive the query price.
While there are no requirements in query pricing with query cost and personal data pricing using privacy, as they price data directly according to their pricing perspective.
As personal data pricing with  market value models market value as a function of features, thus price feature extraction is necessary.
For quality-based data pricing, the models require a basic price for full and exact data, in order to quantify the discount price.}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Technology.}
In query pricing with data view and query cost, they both employ the integer linear programming (ILP) to solve the pricing problem.
For query pricing with information value and quality-based data pricing, they all use sampling methods.
However, the sampling purpose in query pricing based on information value is to reduce the number of possible databases, and improve efficiency.
While quality-based pricing aims to sample inaccurate or incomplete data for trade.}

\textcolor[rgb]{0.00,0.00,1.00}{The query pricing model using data provenance utilizes the concept of lineage set, to track data usage on query.
For personal data pricing using privacy, it involves techniques in differential privacy, such as Laplace mechanism.
As for personal data pricing with  market value, it uses L$\ddot{\text{o}}$wner-John ellipsoid technique to optimize knowledge set, for further learning market value.}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Mechanism(Mech.).} The pricing mechanisms are different. Most of the pricing models are post pricing (PP), such as query pricing with data view, personal data pricing with privacy, etc.
While the pricing model based on query cost employs the auction mechanism to maximize social welfare.
For pricing personal data using market value, it derives the price in an online fashion, thus we mark it as online pricing (OP).
It is also called ``contextual pricing'' in some literatures.
Quality-based pricing is different from others.
As it first receives the price provided by data buyers and then offers data based on the price, we mark it as inverse pricing (IP).}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Arbitrage(Arb.).} Most pricing models consider the arbitrage and can avoid arbitrage, thus there is no arbitrage among thems.
While pricing based on query cost, pricing with market value, and pricing based on data accuracy are not certain whether if they are arbitrage-free.
They do not consider the arbitrage issue in pricing, which may lead to the arbitrage.}

\textcolor[rgb]{0.00,0.00,1.00}{\textbf{Market(Mkt.).} We mark the pricing model as market-oriented if there are studies considering market factors.
For instance, \cite{chawla19revenue,syrgkanis2015pricing} takes buyers' valuation into account.
The social welfare is considered in query pricing based on query cost.
And pricing personal data with market value is obviously market-oriented.}

\textcolor[rgb]{0.00,0.00,1.00}{
To summarize, pricing models in database consider different factors in data pricing, such as information value, data usage, etc.
They utilize different techniques to remove the barrier in data pricing.
And the arbitrage property is always concerned in most pricing models.}







==> related.tex <==
\section{Pricing related issues}
\label{sec:related}

\textcolor[rgb]{0.00,0.00,1.00}{In this section, we simply overview some pricing related issues, \textcolor[rgb]{0.00,0.00,1.00}{including \textcolor[rgb]{1.00,0.00,0.00}{cloud environments, history-aware pricing, }data trade with blockchain, and price discrimination.}}




%The following example will give a brief introduction of price discrimination on physical goods trade.
%
%
%\begin{example} \textbf{Price discrimination}.
%Suppose there are two consumers, $A$ and $B$. $A$ is willing to pay \$5 for a book, but $B$ is willing to pay \$3 for the book.
%Note that the total benefits \$8 (that equals \$5 plus \$3) exceed total cost, \$7, and thus, it is socially desirable to produce the book. However, the producer cannot recover his/her costs at any uniform price: if he/she charges \$5 only one consumer will buy the book, and hence, his/her revenues will be \$5. If he/she charges \$3, both consumers will buy, but revenues will only be \$6. If the producer can employ the concept of price discriminate to sell the book to different users at different prices, it would be possible to cover the development costs of the book.
%\end{example}

\subsection{\textcolor[rgb]{0.00,0.00,1.00}{Data Acquisition}}
\label{subsec:Issues-acq}

{\color{blue}
Data acquisition is the process of sampling data from real world conditions. Modern machine learning needs sufficient data for the training process. Data can also be used for analysis and bussiness. Therefore, data acquisition is of great importance. The data acquisition problem~\cite{li2018cost} is studied for correlation analysis, in which the quality, join informativeness, and price issues of data acquisition are considered.

The paper designs a middleware service named DANCE, a Data Acquisition framework on oNline data market for CorrElation analysis, that provides cost-efficient data acquisition service for the budget-conscious search of the high-quality data on the data marketplaces that maximizes the correlation of certain attributes. DANCE consists of two phases:

\textbf{Phase 1.} During the off-line phase, it constructs a
two-layer join graph of the datasets on the data marketplace. The join graph contains the information of these datasets at both schema and instance level. To deal with the data scalability issue of the marketplaces, DANCE collects samples from the data marketplaces, and constructs the join graph from the samples;

\textbf{Phase 2.} During the online phase, it accepts
the data shoppers' correlation request as well as the constraints (budgets, data quality, and join informativeness). By leveraging the join graph, it estimates the correlation of a certain set of attributes, as well as the join informativeness and quality of the data pieces to be purchased.

Based on these estimated information, DANCE recommends the data pieces on the data marketplace that obtain the best correlation while satisfy the given constraints.


\subsection{\textcolor[rgb]{0.00,0.00,1.00}{Pricing Data in Cloud Environments}}
\label{subsec:Issues-cloud}
Over the past several years, cloud computing has emerged as an important new paradigm for building and using software systems. Multiple vendors offer cloud computing infrastructures, platforms, and software systems including Amazon~\cite{Amazon}, Google~\cite{google}, Salesforce~\cite{salesforce}, and others. Under this situation, pricing data in cloud environments becomes one of promising research lines.  In particular, a new approach for selecting and pricing shared optimizations is presented by using mechanism design~\cite{upadhyaya2012price}. 


In~\cite{upadhyaya2012price}, the author studied how a cloud data service provider should activate and price optimizations that benefit many users. The paper showed how the problem can be modeled as an instance of cost-recovery mechanism design and how the Shapley Value mechanism solves the problem of pricing a single optimization in an offline setting. Then it developed a series of mechanisms that enable the pricing of either additive or substitutive optimizations in either an offline or an online game. It also supports online scenarios where users come and go, and considers the case of substitutive optimizations.

Further, in~\cite{upadhyaya2015managing}, it proposes some new mechanisms for pricing shared cloud resources. More precisely, it provided a novel, lightweight and fast method to support optimal, history-aware pricing of data APIs. With their techniques, even if a buyer makes multiple API calls and ends up purchasing the same data item more than once, she is only charged once for the purchase. To
enable this, it proposed a framework for pricing that allows buyers to refund repeat purchases
of data. Further, the author then provided a compact, secure and tamper proof protocol that enables such
refunds and guarantees that if there is a repeat purchase, it is always possible to get refunds.
Subsequently, the paper generalized the protocol to handle updates and multiple users; and provide
performance improvements through the use of group refunds.


\subsection{\textcolor[rgb]{0.00,0.00,1.00}{History-aware Pricing}}

Typically, sellers charge buyers based on how much data they purchase. In many scenarios, buyers need to make repeated calls to the seller's API. The challenge is then for buyers to keep track of the data they purchase and avoid purchasing the same data twice. For solving the history-aware pricing of data APIs, a secure and tamper proof protocol for refund~\cite{upadhyaya2016price} is presented. 

In~\cite{upadhyaya2016price}, the author proposed lightweight modifications to data APIs to achieve optimal history-aware pricing so that buyers are only charged once for data that they have purchased and that has not been updated. The key idea behind this approach is the notion of refunds: buyers buy data as needed but have the ability to ask for refunds of data that they had already purchased before. To enable this, it proposed a framework for pricing that allows buyers to repeat purchases of data and provided a compact, secure and tamper proof protocol that enables such refunds and guarantees that if there is a repeat purchase, it is always possible to get refunds. Subsequently, it generalized the protocol to handle updates and multiple users, and provided performance improvements through the use of
group refunds.

}

\subsection{Data Trade with Blockchain}
\label{subsec:blockchain}
Blockchain has a number of attractive advantages, so it has been widely applied in many areas: cryptocurrency, finance,
and notary, etc.
The first advantage of blockchain is decentralization, which is realized by various types of consensus mechanisms.
By decentralization, the blockchain technology removes intermediaries, and hence reduces total costs.
Secondly, blockchain ensures unalterability of any information recorded on it, so it can be used to store important
information like certificates, contracts, etc.
Thirdly, blockchain with programmability can be used to realize complex digital contracts, which are called smart contracts over blockchain.
Additionally, the native cryptocurrency of blockchain provides a convenient way of peer-to-peer payment.



On the other hand, as the value of data has been recognized by organizations and individuals, data has become precious assets and been sold on trading platforms. There have emerged some data trading platforms such as {\color{blue}Microsoft Azure Marketplace~\cite{azure}, GBDEX \cite{gbdex}, Infochimps~\cite{infochimps}, etc.}
Although data trading platforms provide a way of sharing data from different sources, it suffers from drawbacks of data leakage, high cost, and unfairness \cite{guan2018secure}.
Firstly, different from physical assets, data can be easily copied with nearly zero cost. Thus, it is highly possible that, data trading platforms make a copy of the data to be sold and resell it for profit.
Secondly, data trading platforms charge very high transaction fee for data trading.
For example, GBDEX charges 40\% for each data exchange, data owners only get 60\% of the data payments.
Lastly, it is difficult to achieve fairness in data trading without a trusted third party.
If data trading platforms are removed to reduce transaction fee, fairness in data trading without any
trusted third needs to be guaranteed.
%Therefore, it is highly challenging to achieve data privacy, TTP-freeness and fairness in data trading at the same time.

To this end, based on the blockchain technology  and the hash chain micro-payment technique, two data trading schemes for data trading platforms are designed in order to achieve data privacy and   fairness in data trading \cite{guan2018secure}.
The first scheme realizes raw data trading, while the second one realizes data statistics trading.
Both systems involve three entities: a blockchain, a data owner, and a data consumer.
Both the data owner and the data consumer have access to the blockchain system to make transactions.
Let $O$ and $C$ be the data owner and data consumer, respectively.
It assumes that, $O$ and $C$ generate their own public key and private key pair respectively,
and the public key corresponds to an account address.


\textbf{Raw data trading scheme}.
The raw data trading scheme consists of six steps, namely data preparation, encrypted data publication, hash chain generation, fund deposit, (off-blockchain) data transaction, and payment settlement.
Assume that the data is generated periodically in real time, e.g., real-time medical data like blood pressure, heart rate.
%The data owner $O$ encrypts each data item with a different key, where $O$ uploads the encrypted data to the blockchain.
%By doing this, the real-time data cannot be modified later once its hash is recorded by the blockchain.
%There exists some cross-verification method of this data so that $O$ cannot forge data without detection.
The data owner $O$ and the data consumer $C$ trade data with a dedicated \emph{smart contract}, which essentially serves as a trusted third party.


The data owner $O$ first generates data encryption keys with a specially designed key generation algorithm,
then he encrypts data records with different encryption keys.
Next, the encrypted data records are processed, which along with the encrypted data records is uploaded to the smart contract.
On the other side, the data consumer $C$ uses the hash chain micro-payment technique to prepare payments for the encryption keys.
The data consumer $C$ generates a long hash chain whose length is exactly the size of the data records, and then $C$ makes a payment commitment by depositing the total payment to the smart contract.
Each hash value on the hash chain represents a piece of micro-payments for data records.
In the subsequent, $C$ and $O$ exchange an encryption key and a hash value one-by-one off-blockchain.
In the end, $O$ can send the latest hash value obtained from $C$ to the smart contract to claim his due payment.


 \textbf{Data statistics trading scheme}.
The data statistics trading scheme consists of the following process, i.e., data preparation, Merkle accumulative tree (MAT) generation,
encrypted data publication, hash chain generation, fund deposit, (off-blockchain) statistics vectors transaction,
data statistics, and payment settlement.
The main idea of encryption is to use vectors containing only $0$ and $1$ to represent scalars such as age, height, and weight, and then encrypts these vectors by multiplying a secret invertible matrix.
%This encryption method does not depend on any NP problem, and it is also additively homomorphic.
%To avoid the same data being encrypted into the same ciphertext, the vectors should be extended with $n$ random real numbers before encryption, where $n \ge 1$.
When the encrypted data is uploaded to the blockchain, the data consumer $C$ can obtain statistics of these encrypted medical data records with statistics vectors, which can be obtained from data owner $O$ through off-blockchain transaction.




\subsection{Price Discrimination}

\emph{Discriminative pricing} is widely applied to a lot of real applications. When integrating the concept of price discrimination with any aforementioned pricing model, the pricing model is able to further refine the data price, through relying on the parameters, such as time, location, demand, etc.

Price discrimination \cite{varian1995pricing} is a phenomenon based on the fact that the willingness-to-pay differs across customers, and thereby, the producer would generally find it advantageous to charge different users' prices.
In general, there are two issues one has to solve when implementing price discrimination in practice, i.e., \emph{determining the willingness} to pay of different consumers, and \emph{avoiding arbitrage} (namely, preventing consumers with high willingness to pay from purchasing the product intended for the consumers with low willingness to pay).
The following example will give a brief introduction of price discrimination on physical goods trade.

\begin{example} \textbf{Price discrimination}.
Suppose there are two consumers, $A$ and $B$. $A$ is willing to pay \$5 for a book, but $B$ is willing to pay \$3 for the book.
Note that the total benefits \$8 (that equals \$5 plus \$3) exceed total cost, \$7, and thus, it is socially desirable to produce the book. However, the producer cannot recover his/her costs at any uniform price: if he/she charges \$5 only one consumer will buy the book, and hence, his/her revenues will be \$5. If he/she charges \$3, both consumers will buy, but revenues will only be \$6. If the producer can employ the concept of price discriminate to sell the book to different users at different prices, it would be possible to cover the development costs of the book.
\end{example}

\textcolor[rgb]{0.00,0.00,1.00}{Price discrimination is a way for data owners to obtain more profit. However, it also brings some problems, which make consumers feel cheated.
It is also vary hard to derive the willingness of each consumers, thus is an interesting and open problem in data pricing.}


\textcolor[rgb]{0.00,0.00,1.00}{In summary, data trade with blockchain considers the issues of privacy, fairness, and efficiency in data trade.}


==> sn-model.tex <==


\subsection{Pricing in Social Networks}
\label{subsec:sn-model}

%Related to online Ad marketing.

%Consumers are never perfectly aware about the different purchase options they have. As pointed out by influential papers in the 60s, the access to information about the existence of a product and its characteristics is a crucial point when observing consumers decisions. This lack of information is an issue for consumers as well as for producers, that in turn need their product to be known to sell it. The traditional solution that producers opted for is advertisement in its informative view as in Nelson (1974) which, however, requires heavy sunk investments in exchange for uncertain outcome.

%In the modern economy, consumers' and producers' access to {\color{blue}information have} changed considerably and towards different directions. On the one hand, new technologies have substantially improved the possibility for consumers to acquire information, but nevertheless they are required to have more skills to use the information they have and to understand more and more sophisticated products. Namely, consumers suffer an information overload and only some of them actually have the ability to face this complexity. On the other hand, the improved knowledge of producers of the social ties among consumers have increased the interest to exploit client's social network in order to generate business. One example of pricing in social networks is that in a social network, some people with more friends usually mean that they are more popular. It also means that if they use some kind of product, more people will be likely to buy the product too. As a result, by offering the popular people rewards will help to sell the products.

%Pricing over social networks basically concern about the information. Existing pricing models  in social networks can generally be divided into two situations, i.e., the \emph{incomplete} information case and the  \emph{full} information case.


%\subsubsection{Incomplete Information Case}

%The incomplete information case suggests that, agents know a common distribution about others' private valuations, and make decisions simultaneously. The ``rational behavior'' of agents in this case is captured by the well-known Bayesian Nash equilibrium.
%{\color{blue}Consider the problem of a monopolist selling a digital product to agents in a social network \cite{arthur2009pricing}. To incorporate social influence, assume that each agent¡¯s utility of having the product is the summation of two parts: the private intrinsic valuation and the overall influence from her friends who also have the product. Given such assumption, the purchasing decision of one agent is not solely made based on her own valuation, but also on information about her friends¡¯ purchasing decisions. However, a typical agent does not have complete information about others¡¯ private valuations, and thus might make the decision based on her belief of other agents¡¯ valuations. In our case, the monopolist has no or incomplete information about the structure (and thus chooses her pricing strategy as if consumers did not interact with one another)}

%Examples include a study of linear influence on agents' utility in digital products selling under the incomplete information situation \cite{chen2011optimal} and an attempt at modeling theoretically the strategic decisions of a monopolist choosing to discriminate the price according to the ability of a consumer to induce others to buy \cite{carroni2015pricing,carroni2014pricing}.


%The  pricing strategy  \cite{arthur2009pricing} introduces \emph{non-adaptive} strategies for sellers in the context of expected revenue maximization, in which the seller chooses and commits to a discount coupon and cashback offer for each potential buyer before the cascade starts. {\color{blue}Intuitively, the seller strategy we propose is based on an influence-and-exploit idea, and it consists of categorizing each potential buyer as either an influencer or a revenue source. The influencers are offered the product for free and the revenue sources are offered the product at a pre-determined price, chosen based on the exact probability model. Briefly, the categorization is done by finding a spanning tree of the social network with as many leaves as possible, and then marking the leaves as revenue sources and the internal nodes as influencers.}



%\subsubsection{Full Information Case}


%{\color{blue}A more complex situation is the full information one. It has become more and more popular due to the great advancement in technology and Internet. Many models have been proposed under the full information case. In full information case, the auctioneer knows the demands of the agents.

%The work of Candogan, Bimpikis and Ozdaglar \cite{candogan2012optimal} considers a monopolist who sets prices for agents that are embedded in a network and exhibit positive externalities. Besides, they adopt a full-information model, whereas the agents' values are drawn from a known distribution.}

%Work in \cite{bloch2013pricing} analyzes the problem of optimal monopoly pricing in social networks in order to characterize the influence of the network topology on the pricing rule assuming that the monopoly and the customers have symmetric information.

%The use of consumers' network is an alternative solution to the informative problem, and it is more effective than advertising as consumers are usually embedded with a considerable component of trust. Moreover, the decrease in costs of communicating to a large number of subjects, brought upon by modern technologies (such as social networks, emails, messages), improves the effectiveness of this kind of programs, increasing their profitability.

%In wanting to make use of the social network, consumers that are popular and able to acquire information often become the target of company's strategies. In particular, advantageous deals in the form of a reduced price or a gift are proposed to old buyers who support the firm to extend its clients base by convincing others to buy. Old buyers are clearly aware about the existence and characteristics of the product (as they experienced it in the past)  and the more popular they are the more likely to be effective in helping firms to enlarge the demand.

%Specifically, it models the strategy of a monopolist that offers rewards to current clients in order to induce them to activate their social network and convince peers to buy from the company. In presence of heterogeneous search costs and reservation prices, this network-activation reward program may serve to expand the client base through a flow of information from informed to uninformed consumers. The offer of the monopolist affects individual incentives of aware people to share information, determining a minimal degree condition for investment. The optimal unitary reward balances the information spread effect (i.e. more receivers) and the crowding effect (i.e. less individual incentives) of an increase in the number of speakers. The monopolist always finds it profitable to use the bonus. Nevertheless, its introduction has ambiguous effects on the price and profits, depending on the process of spread of information and, in turn, on the network structure.


%Pricing in social networks is mainly about the

The effect of micro-dynamics (or interactions) between agents on macroscopic properties of a social structure  is essential to the pricing issue over social networks.
Take a viral network an example, it consists of potential buyers of a particular new product offering in the market. These buyers interact with each other and influence each other's purchase decisions through word-of-mouth and/or behaviors.

As a result, the term  of \emph{social influence} is defined to describe that, agents on their neighboring agents in the network have a significant role to play in generating a network effect on the sales of the product.
Thus, {\color{blue}the problem of ``influence maximization'' \cite{bharathi2007competitive,chen2010scalable}} is studied to determine the set of initial adopters who, through an influence process, can maximize the future adoptions of the product.
Also, the problem of ``revenue maximization'' \cite{dayama2012optimal,arthur2009pricing} is considered for viral marketing.

To enable the social influence to work, the seller has two channels through which social networks influence a consumer's demand.
The first one is called \emph{local network externalities}, where consumers benefit from the consumption of the same good by their direct neighbors. It captures situations where agents receive discounts if they call friends who subscribe to the same network, share a common software with their friends.
In the second channel of \emph{aspiration based reference pricing}, consumers construct a reference price for the good based on the price charged to their direct neighbors, and experience a positive utility if the price they receive is below their reference price.
This model is applicable to situations where firms use discriminatory pricing that lacks transparency, like airline pricing and negotiated pricing.





\subsubsection{Pricing with Local Network Externalities}

In wanting to make use of the social network, consumers that are popular and able to acquire information often become the target of companies' strategies.
In particular, advantageous deals in the form of a reduced price or a gift are proposed to old buyers who support the firm to extend its clients base by convincing others to buy.
Old buyers are clearly aware about the existence and characteristics of the product (as they experienced it in the past).
The more popular of them are more likely to be effective in helping firms to enlarge the demand.


According to the social influence of a consumer which represents the ability of a consumer to induce others to buy,  one attempts to theoretically model the strategic decisions of a monopolist choosing to discriminate the price \cite{carroni2015pricing}.
In the setup, the reduction in price takes the form of a monetary gift offered by the monopolist for each new customer brought into the clients base in a context where the population of potential buyers exhibits heterogeneous search costs.
Consider a setup where a monopolist seeks to sell a product to a large, but finite, population $N = \{1, 2, \cdots, i, \cdots, n\}$ of agents. Consumers differ according to their willingness to pay and their search costs. The utility function for an agent $i$ from buying the product at price $p$ is defined as:
$$u_i=r_i-p-s_i$$
where $r_i$ is the reservation price representing the highest price each agent can accept which is distributed according to a c.d.f. on the support $[0, 1]$, and $s_i$ is the search cost of the agent.
The search cost is interpreted as the time and skills that an agent needs to dedicate for the acquirement of information.
For instance, young people tend to have more time to spend searching for information about technological products or services than old people. Moreover, they own stronger skills to obtain and interpret information about prices and characteristics of these products. So, young people would have a lower search cost.

Consider a \emph{two-period} model where the supply side of the market is constituted by a monopolist which aims at maximizing the sum of inter-temporal profits. Defining $D_1(p)$ as the demand in the first period and assuming a marginal cost normalized to 0, the expected profit obtained charging price $p$ will be given by:
$$\pi_1=p\cdot D_1(p).$$
In the second period, the monopolist offers rewards to old customers through a ``bring a friend'' program.
The rationale of this offer is to eliminate the high search costs that prevent some of the potential consumers from buying.
This gift takes the form of a unitary amount $b$ for each referral. Since each new consumer corresponds to one reward $b$ given to some old customer, the margin in the second period is given by $(p - b)$.
Thus, defining $D_2(p, b)$ as the demand in the second period coming from new consumers, the expected profit turns out to be: $$\pi_2=(p-b)\cdot D_2(p,b).$$


The incentives created by the offer are clearly stronger.
The more one person is connected, leading to the emergence of a minimal degree (number of neighbors), above which an agent invests in communicating with peers.
This leads to the quite realistic result that, the equilibrium investors are only those with \emph{relatively high degrees}, and thus only a limited fraction of agents gets the discounts.


\subsubsection{Aspiration based Reference Pricing}


In real world, when we need to buy something from a monopoly, we may ask our friends who already bought it about the price and get our own valuation.
Accordingly, the aspiration-based price reference model is introduced.

Specifically, in this model, it assumes that, agents compare the price they receive with the prices received by their neighbors, and enjoy positive utility if they receive a lower price than the prices in their neighborhood \cite{bloch2013pricing}.
The utility of a consumer, denoted by $U_i$, is defined over the average price charged to the consumer's neighbors:$$
U_{i}=\theta_{i}-p_{i}+p_{ave},
$$
where $p_i$ is the price offered by the monopoly, $p_{ave}$ is the average of prices received by neighbors of the consumer $i$, and $\theta_{i}$ is a taste parameter uniformly distributed on $[0, 1]$. The utility represents the own valuation of the product.
A consumer located at node $i$ buys the good if and only if the valuation is positive. %As in the case of local network externalities, prices are announced before consumers learn their random valuation.

We now consider two situations, i.e., \emph{single monopoly} pricing and \emph{multi-monopolies} pricing.
For the first situation, a \emph{relevant centrality} is defined, which measures the sum of inverse degrees of a node's neighbors.
The monopoly has an incentive to charge higher prices at nodes which have higher centrality.
%, as measured by the sum of the inverse degrees of a node's neighbors.
A network of particular interest is the star, where the hub has a very high centrality measure and hence receives a higher price than the peripheral agents.
This ranking of prices in the star is very intuitive: by raising the price in the hub, the monopoly is able to increase demand at all peripheral nodes, whereas an increase in the price of the peripheral node only increases demand at the hub.
Hence, the indirect positive effect of a price increase is higher for the hub than for a peripheral agent, implying that the optimal price will be higher at the hub.

As a result, agents with many neighbors of low degree (like the hub of the star) receive a smaller surplus than agents with few neighbors of high degree (like the peripheral agents in the star).
It reflects the intuition that, agents at the hub of the star are harmed by their location in the network, as they pay a higher price than their neighbors. This result suggests that, in a model of endogenous network formation, agents would try to avoid occupying central positions, resulting in the construction of symmetric social networks.

For the situation where each node is served by different local monopolies (w.r.t. \emph{multi-monopolies} pricing), it has been proved that \cite{bloch2013pricing},
there is a unique symmetric equilibrium where all local monopolies charge the same price.
It implies that consumers at every node have the same demand, so that consumer surplus is independent of a node's centrality.
In fact, consumers have an incentive to connect to one other node in order to benefit from the positive social comparison effect, but no incentive to form any additional link.



%\subsection{Summary}
%
%So far, we have introduced the five modern pricing models for data trade.
%Table \ref{tab:Mod} summarizes these models in several aspects.
%
%
%First, among the five models, both game theory based pricing model and auction based pricing model consider the market situation, which describes the relation of demand and supply, market competitiveness, etc.
%By contrast, the other three pricing models are highly related to dataset itself.
%Indeed, the two group of pricing models, i.e., the models considering market and the ones with various data services, can combine with each other for more sophisticated trade situations.
%We can also realize that, the last three pricing models, i.e., the ones with game theory, auction, and social networks, are applicable to physical goods trade.
%Hence, these three ones have more wide application base.
%In addition, as we mentioned at the initial part of this section, all of these pricing models can cooperate with price discrimination for further market segmentation.
%
%
% \begin{table*}[t]\footnotesize
% 	\centering
% 		\caption{Summary of Different Data (Service) Pricing Models}
% 	\begin{threeparttable}
% 	\begin{tabular}
% 		{lllll}
% 		\toprule[0.7pt]
% 		\textbf{Pricing model}&\textbf{Market}&\textbf{Data} &\textbf{Physical goods}&\textbf{Price discrimination}\\
% 		\midrule[0.5pt]
% 		database based model           &$\times$  &$\checkmark$ &$\times$    &$\checkmark$\\
% 		machine learning based model   &$\times$  &$\checkmark$ &$\times$    &$\checkmark$ \\
% 		game theory based model        &$\checkmark$&$\times$
% &$\checkmark$&$\checkmark$\\
% 		auction based pricing          &$\checkmark$&$\times$ &$\checkmark$&$\checkmark$\\
% 	    pricing in social networks     &$\times$    &$\checkmark$ &$\checkmark$    &$\checkmark$\\
% 		\bottomrule[0.7pt]
% 	\end{tabular}
% 	 	\end{threeparttable}
% 	\label{tab:Mod}
% \end{table*}

%Online advertising has become the main source of revenue for many companies which provide free services over the Internet, such as Google Search, Facebook, YouTube and Flickr. Since HotWire sold the first banner ads in 1994, online advertising has evolved into many forms and techniques. Some of these techniques, such as Google's sponsored search, have benefited their developers tremendously.

%There is also a new form of advertising, which could potentially benefit social network providers such as Facebook and Twitter. We call it \emph{sponsored viral marketing}.
%It is applicable to the current situation where big social network providers such as Facebook continue to explore various different approaches for monetization. According to the research company eMarketer\footnote{http://www.emarketer.com/newsroom/index.php/ google-display-ad-leader/}, the current main source of revenue for Facebook is from the display ads market where Facebook can use the demographic information from the profiles of hundreds of millions of its users to target the ads directly to them. However, many recent data and reports (e.g. [17, 18, 33]) suggest that it is not clear how much advantage Facebook has over other internet companies which can also collect user information in many other ways, like Google, in this market. For a definitive competitive advantage that goes beyond exploiting just user information, one needs to explore new monetization schemes that better exploit the strength and distinguishing features of social networks.

%Essential is exploiting the word-of-mouth effects uniquely provided by social networks: people tend to trust their friends' recommendations more than other advertising channels. Even with all the data that social network providers have about each of their users, social influence can be even more reliable in influencing a person's online purchasing behavior.

%\subsubsection{Aspiration based Reference Pricing}
%
%
%In the aspiration-based price reference model, work in \cite{bloch2013pricing} obtain a second network irrelevance result, when every node is served by a different firm.
%This irrelevance result, which is robust to changes in the model, stems from the following observation.
%If all other firms charge the optimal monopoly price, a local monopoly cannot benefit from charging a different price. When all nodes are served by a single monopolist, this reasoning fails as the monopolist may want to increase the price at some node in order to increase demand at the neighboring nodes. For example, in a star, the monopoly has an obvious incentive to charge a high price at the hub in order to increase demand at peripheral nodes.
%
%For the single monopoly pricing, the paper define a relevant centrality which measure is the sum of inverse degrees of a node¡¯s neighbor. The monopoly has an incentive to charge higher prices at nodes which have higher centrality, as measured by the sum of the inverse degrees of a node¡¯s neighbors. A network of particular interest is the star, where the hub has a very high centrality measure and hence receives a higher price than the peripheral agents. This ranking of prices in the star is very intuitive: by raising the price in the hub, the monopoly is able to increase demand at all peripheral nodes, whereas an increase in the price of the peripheral node only increases demand at the hub. Hence the indirect positive effect of a price increase is higher for the hub than for a peripheral agent, implying that the optimal price will be higher at the hub.
%
%Hence agents with many neighbors of low degree (like the hub of the star) receive a smaller surplus than agents with few neighbors of high degree (like the peripheral agents in the star), reflecting the intuition that agents at the hub of the star are harmed by their location in the network, as they pay a higher price than their neighbors. This result suggests that in a model of endogenous network formation, agents would try to avoid occupying central positions, resulting in the construction of symmetric social networks.
%
%For the situation where each node is served by different local monopolies. The paper proves that there is
%a unique symmetric equilibrium where all local monopolies charge the same price. It implies that consumers at every node have the same demand, so that consumer surplus is independent of a node's centrality. In fact, consumers have an incentive to connect to one other node in order to benefit from the positive social comparison effect, but no incentive to form any additional link.
%
% \begin{table*}[thb]\footnotesize
% 	\centering
% 		\caption{Comparison over Different Pricing Models}
% 	\begin{threeparttable}
% 	\begin{tabular}
% 		{lllll}
% 		\toprule[0.7pt]
% 		\textbf{Pricing model}&\textbf{Wide application}&\textbf{Trasportable}&\textbf{Market situation}&\textbf{Data value}\\
% 		\midrule[0.5pt]
% 		database based model        &$\times$    &$\times$    &$\times$    &$\checkmark$\\
% 		machine learning based model&$\checkmark$&$\times$    &$\times$    &$\checkmark$\\
% 		game theory based model     &$\checkmark$&$\checkmark$&$\checkmark$&$\times$\\
% 		auction based pricing       &$\checkmark$&$\checkmark$&$\checkmark$&$\times$\\
% 	    pricing in social networks  &$\times$    &$\checkmark$&$\times$    &$\checkmark$\\
% 		\bottomrule[0.7pt]
% 	\end{tabular}
% 	 	\end{threeparttable}
% 	\label{tab:Mod}
% \end{table*}
%
%
%Table \ref{tab:Mod} summarizes the five pricing models that we've introduced in this section. Database and social networks based models are mostly applied in limited situations like viral markets, while the other three models have wide applications. Transportable means that these data pricing models can also be applied in physical goods trading. Market situation describes the competitiveness in the markets of these models. Besides, the data value represents whether or not these models are highly related to data. For instance, the database, machine learning and social networks based models are more close to data itself while auction and game theory based model are more traditional.
%
%
%
%%Online advertising has become the main source of revenue for many companies which provide free services over the Internet, such as Google Search, Facebook, YouTube and Flickr. Since HotWire sold the first banner ads in 1994, online advertising has evolved into many forms and techniques. Some of these techniques, such as Google's sponsored search, have benefited their developers tremendously.
%
%%There is also a new form of advertising, which could potentially benefit social network providers such as Facebook and Twitter. We call it \emph{sponsored viral marketing}.
%%It is applicable to the current situation where big social network providers such as Facebook continue to explore various different approaches for monetization. According to the research company eMarketer\footnote{http://www.emarketer.com/newsroom/index.php/ google-display-ad-leader/}, the current main source of revenue for Facebook is from the display ads market where Facebook can use the demographic information from the profiles of hundreds of millions of its users to target the ads directly to them. However, many recent data and reports (e.g. [17, 18, 33]) suggest that it is not clear how much advantage Facebook has over other internet companies which can also collect user information in many other ways, like Google, in this market. For a definitive competitive advantage that goes beyond exploiting just user information, one needs to explore new monetization schemes that better exploit the strength and distinguishing features of social networks.
%
%%Essential is exploiting the word-of-mouth effects uniquely provided by social networks: people tend to trust their friends' recommendations more than other advertising channels. Even with all the data that social network providers have about each of their users, social influence can be even more reliable in influencing a person's online purchasing behavior.

